Continuous and Atlas-free Analysis of Brain Structural Connectivity

Brain structural networks are often represented as discrete adjacency matrices with elements summarizing the connectivity between pairs of regions of interest (ROIs). These ROIs are typically determined a-priori using a brain atlas. The choice of atlas is often arbitrary and can lead to a loss of important connectivity information at the sub-ROI level. This work introduces an atlas-free framework that overcomes these issues by modeling brain connectivity using smooth random functions. In particular, we assume that the observed pattern of white matter fiber tract endpoints is driven by a latent random function defined over a product manifold domain. To facilitate statistical analysis of these high dimensional functional data objects, we develop a novel algorithm to construct a data-driven reduced-rank function space that offers a desirable trade-off between computational complexity and flexibility. Using real data from the Human Connectome Project, we show that our method outperforms state-of-the-art approaches that use the traditional atlas-based structural connectivity representation on a variety of connectivity analysis tasks. We further demonstrate how our method can be used to detect localized regions and connectivity patterns associated with group differences.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> manuscript_v1.tex <==
\section{Introduction}\label{sec:introduction}

 The brain connectivity is an important phenotype for understanding how the brain works in dealing with everyday challenges and in the context of mental disorder and neurodegenerative disease \citep{fornito2013, park2013}. Recent advances in brain imaging and computational neuroscience have facilitated the construction of enormous multi-subject studies such as the Human Connectome Project (HCP) \citep{glasser2013}, UK Biobank \citep{miller2016} and the Adolescent Brain Cognitive Development study \citep{karcher2021}. Along with multimodal imaging data, such studies often collect a plethora of subject level information including genetic, cognitive, psychiatric, and demographic measures. These undertakings hold great promise to bolster our understanding of the heterogeneity of brain connectivity across individuals and its relationship to various traits and mental disorders. That said, due to challenges resulting from massive data sizes and the complex nature of the connectivity data, new methods of analysis are required to fully realize their potential.
\par 
There are distinct notions of brain connectivity (or network) obtained from different brain imaging modalities. For instance, \textit{functional connectivity} (FC) is obtained from functional magnetic resonance imaging (fMRI) and determines a network using pairwise measures, e.g. correlation, in the BOLD signal. On the other hand, \textit{structural connectivity} (SC) aims to measure the strength of connectivity between regions based on the white matter (WM) fiber tracts reconstructed from diffusion MRI (dMRI). The most common approach for analyzing connectivity data is to represent it as a symmetric adjacency matrix,  $\boldsymbol{A} \in \mathbb{R}^{V \times V}$, where $V$ is the number of ROIs on the brain surface and the element $\boldsymbol{A}_{ab}$ quantifies the ``strength of connectivity'' between ROIs $a$ and $b$. To obtain $\boldsymbol{A}$, the brain is first parcellated into $V$ ROIs using some predefined atlas e.g., the Desikan-Killiany Atlas \citep{desikan2006} has $V=68$ cortical nodes, and the Destrieux Atlas \citep{destrieux2010} has $V=148$ cortical nodes. There is wide interest in understanding the variability of human brain networks \citep{durante2017nonparametric,wang2019}, and relating such variability to human traits such as cognition and personality \citep{zhang2019,arroyo2020,arroyo2021,arroyo2021b}. For an overview on the the current state of the representation and statistical analysis of connectome matrices, see \cite{chung2021}.
\par 
The discrete ROI-based framework of analyzing brain networks suffers from a major drawback - the reliance on the pre-specification of an atlas. This results in at least two major issues. First, there is no consensus as to which atlas is the best for brain connectivity analysis and therefore the selection for a given application is somewhat \textit{ad-hoc}. Second, the ROIs can be large and thus introduce information loss, since fine-grained connectivity information on the sub-ROI level is aggregated in the construction of the adjacency matrix. Recent studies indicate that connectivity information at higher resolutions capture valuable information for many traits of interest \citep{mansour2021,cole2021}. One way to mitigate these drawbacks is to increase the number of ROIs in the parcellation. We can observe this trend in more recent atlases, e.g., \cite{power2011functional} use an atlas containing $264$ nodes, and \cite{glasser2016multi} build an atlas of $360$ regions for cortical surface. However, increasing the number of ROIs introduces additional challenges in data analysis. The dimension of the network grows on the order of $V^2$, rendering statistical modeling and inference very challenging for even moderately large $V$. Moreover, alignment of smaller ROIs between subjects is difficult. When the alignment is poor, unwanted variances among the connections are introduced due to misalignment as opposed to the biological heterogeneity in which we are interested in.
\par 
Our work addresses these problems by transitioning from the discrete, ROI based representation of brain connectivity to a continuous model. Specifically, let $S_1$ and $S_2$ represent the left and right white surfaces of the brain (Figure xx shows an T1 image of the brain in panel (a) and its two white surfaces in panel (b)), we are interested in studying the connectivity pattern between any two points on $S_1$ and $S_2$. Denote $\Omega = \mathbb{S}^2_1 \cup \mathbb{S}^2_2$, where $\mathbb{S}^2_1$ and $\mathbb{S}^2_2$ are independent copies of the 2-sphere. Since each of the white surfaces is (approximately) homeomorphic to $\mathbb{S}^2$,  we propose to encode the connectivity pattern for each subject as a continuous function on $\Omega\times\Omega$ which quantifies the ``strength of connectivity'' between any pair of locations on $\Omega$. We refer to this function as the continuous connectivity (ConCon).
\par 
There are many advantages of the ConCon representation compared with the traditional discrete adjacency matrix. Crucially, it is atlas free and therefore we are able to avoid information loss resulting from ad-hoc spatial parcellations. Additionally, the continuous framework inherently captures both high and low frequency variations in the data, thus facilitating a multi-resolution representation of the connectivity. If desired, an atlas-based representation can be recovered by integrating the ConCon over the ROIs of interest. 
\par 
ConCon also presents some additional challenges over atlas-based approaches. ROI-based connectome matrices can be easily constructed by using simple statistics computed on the WM streamlines  connecting pairs of ROIs. However, ConCon is not easy to estimate from streamlines. One simple method is to impose a high-resolution mesh grid on the cortical surfaces  ($\Omega$), and estimate ConCon at each pair of vertices. For an accurate estimation, this method needs enormous amount of streamlines \cite{moyer2017,cole2021} for even moderately large grids, and generates very big adjacency matrices that are hard to store and analyze. Adding to the complexity is the data is observed in separate coordinate systems and each subjects cortical surface has different morphology, presenting additional hurdles to meaningful joint analysis.
\par 
In this work, the ConCon is modeled as a latent non-negative and symmetric \textit{random intensity function} with realizations in $L^2(\Omega\times\Omega)$. We propose an explicit generative model for the observed WM streamline endpoints using the latent ConCon, and this model reveals several paths to estimate the latent ConCon $U$ from WM streamlines obtained using tractograph algorithms. We then develop ...


%we propose an efficient methodology for the joint analysis of a sample of high resolution connectivity data under the ConCon framework. The structural connectivity data for each subject is modeled by assuming a latent non-negative and symmetric \textit{random intensity function} $U$, with realizations in $L^2(\Omega\times\Omega)$. We propose an explicit generative model for the observed WM tract endpoints for each subject and show how they can be used to learn an optimal collection of continuous basis functions for representing realizations of $U$. Under a convenient reparameterization, we show that the basis functions can be estimated by the penalized decomposition of a semi-symmetric tensor that can be computed from the high-resolution connectivity data. Crucially, the dimension of this tensor can typically be made much smaller than the raw data, allowing us to circumvent a potentially insuperable computational bottlekneck. 

We apply the proposed method to structural connectivity data computed from a sample of HCP subjects and show that our method outperforms traditional atlas-based approaches on several statistical tasks of interest. \textcolor{red}{more details to come once the real data analysis is finished ...}

\par 
The remainder of this paper is organized as follows. The statistical model for the connectivity data is given in Section ~\ref{sec:statistical_model} and the methodology for estimating the continuous connectivity is presented in Section~\ref{sec:methods}. Section~\ref{sec:simulation} shows results from simulation studies illustrating the computational performance of the proposed estimation algorithm. The real data analysis of HPC subjects is presented in Section~\ref{sec:real_data_experiments} and concluding remarks are given in Section~\ref{sec:conclusion}.


\section{Statistical Model for Continuous Connectivity}\label{sec:statistical_model}
\subsection{Relating Observed Streamline Endpoints to Latent ConCon}
%In this work, we mainly consider the structural brain connectivity (SC) derived from dMRI, although the method developed can be straightforwardly applied to functional connectivity (see brief discussion in the appendix). 

%To estimate SC, we first need to estimate local diffusion configurations, e.g., diffusion tensors or fiber orientation distribution functions \citep{descoteaux2008deterministic,smith2013sift,girard2014towards}, from the dMRI data. Then a tractography algorithm is applied to estimate the white matter fiber tracts connecting different brain regions. The output of the tractography set contains millions of streamlines in the form of 3D curves. In this paper, we adopt an state-of-the art tractography algorithm, named surface enhanced tractography (SET) \citep{st2018surface}, to reduce tractography biases and errors \citep{girard2014towards,fornito2013graph}. An important feature of SET is that it ensures the ending points of streamlines to remain on cortical surfaces (the white surfaces, the boundaries between white matter and grey matter).
%Let $\tilde{O}=\{ (\tilde{\bf p}^1_1,\tilde{\bf p}^1_2), \cdots, (\tilde{\bf p}^M_{1},\tilde{\bf p}^M_2) \}$ denote the set of all end points from streamlines connecting cortical surfaces $\Omega$. Note that $\Omega = S_1 \cup S_2$, where $S_1$ is the left cortical surface and $S_2$ is the right cortical surface, and $\tilde{\bf p}^i_j  \in \Omega$ is a point on $\Omega$. Since $S_i$ is homeomorphic to a 2-sphere, we can parameterize $S_i$ using a spherical coordinate, i.e., $S_i(\theta,\phi)$ is a point on the cortical surface parameterized by $(\theta,\phi) \in \mathbb{S}^2$. Now any point on $S_i$ has a corresponding point on $\mathbb{S}^2$. Denote $\tilde{\bf p}^i_j  \in \Omega$'s corresponding point on $\mathbb{S}^2$ as ${\bf p}^i_j$, we now have  ${O}=\{ ({\bf p}^1_1,{\bf p}^1_2), \cdots, ({\bf p}^M_{1},{\bf p}^M_2) \}$. With some abuse of notation, we let $\Omega = \mathbb{S}^2_1\cup\mathbb{S}^2_2$, and have $O \in \Omega \times \Omega$. 

%Now consider a population of subjects containing $N$ dMRI scans. After SET, we obtain a set $\{O_i\}$ for $i = 1,..., N$, where each $O_i$ is a point process on $\Omega \times \Omega$. Assuming that there is a latent function $f_i: \Omega \times \Omega \mapsto \mathbb{R}$ governing the observation $O_i$, we are interested in estimating this latent function, understanding its variation across the population and linking it to the behavior and brain function. This latent function is the continuous connectivity (ConCon) we are studying in this paper. 
%\textcolor{red}{PLOT: I'm thinking that we need a plot to illustrate cortical surface, the sphere, ending points on sphere, and connections generated by ending points.}
Let $\tilde{O}=\{ (\tilde{\bf p}^1_1,\tilde{\bf p}^1_2), \cdots, (\tilde{\bf p}^M_{1},\tilde{\bf p}^M_2) \}$ be end points of $M$ streamlines connecting cortical surfaces $\Omega = S_1 \cup S_2$ in a subject. Since $S_d$ is homeomorphic to $\mathbb{S}^2$, we can parameterize it using a spherical coordinate.  Let $({\bf p}^q_1,{\bf p}^q_1)$ be the image of $(\tilde{\bf p}^q_1,\tilde{\bf p}^q_1)$ on $\mathbb{S}^2_1 \cup \mathbb{S}^2_2$ under the homeomorphism; we define the set ${O}=\{ ({\bf p}^1_1,{\bf p}^1_2), \cdots, ({\bf p}^M_{1},{\bf p}^M_2) \}$ with $O \subset\Omega \times \Omega$. For a single subject, we can model the streamline end points $O$ as a nonhomogeneous Poisson point process on $\Omega \times \Omega$ with a unknown (deterministic) integrable intensity function $u: \Omega \times \Omega \mapsto [0,\infty)$ \citep{moyer2017}, denoted as $O \sim PP(u)$, and defined as follows. For any two distinct/non-overlapping and Borel measurable regions $E_1 \in \Omega$ and $E_2 \in \Omega$, let $A(E_1,E_2)=\int_{E_1} \int_{E_2} u(\omega_1,\omega_2)d\omega_1d\omega_2 < \infty$. Denote $N(E_1,E_2)$ as the counting process of the number of streamlines ending in $(E_1,E_2)$, the distribution of which is described as 
\begin{equation}\label{eqn:IHP}
    P(N(E_1,E_2)=n) = \frac{(A(E_1,E_2))^n}{n!}\exp(-A(E_1,E_2)),
\end{equation}
\begin{remark}
The model \eqref{eqn:IHP} subsumes the current discrete way of analyzing SC count matrices. To see this, let $\{E_1,E_2,...,E_V\}$ be the $V$ brain regions based on one of the existing brain atlases. The probability of observing an adjacency matrix ${\bf A} \in \mathbb{R}^{V \times V}$ (whose element $a_{ij}$ counts the number of streamlines connecting regions $E_i$ and $E_j$)  is given as
$$P\{N(E_i,E_j)=a_{ij},i<j;i,j = 1,..., V \} = \Pi_{i<j;i,j=1,...,V}  \frac{(A(E_i,E_j))^{a_{ij}}}{{a_{ij}}!}\exp(-a_{ij}), $$
where $A(E_i,E_j) = \int_{E_i} \int_{E_j}u(\omega_1,\omega_2)d\omega_1d\omega_2$. 
\end{remark}
\par 
In the analysis of a random sample of the structural connectivity data from $N$ subjects, $\{O_1,...,O_N\}$, two additional layers of complexity emerge. First, modeling replicated point processes with a single deterministic intensity function is likely insufficient to properly accommodate subject specific variability in connectivity patterns. In such scenarios, it is often reasonable to assume that the intensity function governing $O_i$ is itself a realization of an underlying random process. Hence, the object of interest is not a single unknown deterministic function, but rather a distribution over functions. Second, an additional source of unwanted spatial variability creeps in due to the inconsistent alignment of the cortical surface for each subject. Failure to account for such misalignment can lead to an artificial inflation in the variability of the inferred connectivity pattern. This nuisance variability can be modeled using random diffeomorphisms: $(\gamma^1,\gamma^2)$, where $ \gamma^d \in \mathbb{S}^2 \mapsto \mathbb{S}^2$. The generative model for the $i$-subject's connectivity pattern $O_i$ is given as follows:

\begin{equation}\label{eqn:generative_model}
    \begin{aligned}
    &\gamma^1_i \sim W_1 \qquad \gamma^2_i \sim W_2 \qquad U_i \sim U \qquad U \perp W_1, W_2 \\
    %&\tilde{U}_i(\omega_1,\omega_2) = U_i((\gamma^1_i)^{-1}(\omega_1),(\gamma^2_i)^{-1}(\omega_2)) \\
    %& O_i|\tilde{U}_i \sim PP(\tilde{U}_i),
    &O_i|U_i \sim PP(U_i((\gamma^1_i)^{-1}(\omega_1),(\gamma^2_i)^{-1}(\omega_2))), \\
    \end{aligned}
\end{equation}
where $(\gamma)^{-1}$ indicates the inverse of $\gamma$,
$W_d$ for $d=1,2$ are distributions on the space of diffeomorphisms of $\mathbb{S}^2$ and $U$ is the random intensity function. We assume that the realizations of $U$ are twice continuously differentiable on $\Omega\times\Omega$. 

%Next, we consider two subjects and their streamline ending points $O_1$ and $O_2$. To study the difference of their ConCons, another layer of complexity starts to kick in - we have to align to find the spatial correspondence between the two subjects. Failure to account for such variability can be detrimental when computing descriptive summaries, and for subsequent inferential tasks. Let $\gamma$ be a diffeomorphism: $\gamma: \mathbb{S}^2 \mapsto \mathbb{S}^2$, the alignment between two ConCons is the process of finding a pair of diffeomorphisms $(\gamma^1, \gamma^2)$ that minimizes certain cost function between $f_1(x,y)$ and $f_2(\gamma^1(x),\gamma^2(y))$. It is often important to regularize the two diffeomorphisms to avoid a degenerated result which is also referred as pinching effect in functional data alignment, see e.g., \cite{zhang2015elastic} and \cite{ramsay2005}.

%Now let's consider multiple subjects with multiple observations $\{O_1,...,O_N\}$. Assume their ConCons are $\{f_1,...,f_N\}$, respectively. To compare these ConCons, we first need to have a template ConCon and then align individual ConCons $\{f_1,...,f_N\}$ to this template. Let $f_\mu$ denote this template, and let $f^*_i$ be the aligned ConCon, where $f^*_i = f_i(\gamma^1_i,\gamma^2_i)$ with $(\gamma^1_i,\gamma^2_i)$ being the diffeomorphisms aligning $f_i$ to $f_\mu$. Inspired by existing work on Bayesian registration of functional data \citep{cheng2016bayesian,bharath2020distribution}, we write the following generative model for multiple ConCons: 

%\begin{equation}\label{eqn:generative_model}
%    \begin{aligned}
%    &\gamma^1_i \sim W_1 \qquad \gamma^2_i \sim W_2 \\
%    &f^*_i|(\gamma^1_i,\gamma^2_i) \sim GP(f_\mu,\Sigma) \\
%    &f_i = f_i^*((\gamma^1_i)^{-1},(\gamma^2_i)^{-1}) \\
%    & O_i|f_i \sim PP(f_i),
%    \end{aligned}
%\end{equation}
%where $W_i$ for $i=1,2$ are distributions on the space of  diffeomorphisms of $\mathbb{S}^2$, $f_i^* = f_i(\gamma^1_i,\gamma^2_i)$, and $GP(,)$ represents a Gaussian Process model. 
\subsection{A Reduced Rank Model for ConCon}\label{ssec:rr_model_cc}
Fundamentally, we are interested in inference and prediction of $U$. Due to it's infinite dimensionality, we propose a reduced rank modeling solution, which permits the translation of the statistical analysis of interest into a function subspace with finite dimension. In this section, we formulate a data adaptive reduced rank space that avoids the curse of dimensionality.
\par 
Let $\mathcal{H} = \{u \in L^2(\Omega\times\Omega): u(\omega_1,\omega_2)=u(\omega_2,\omega_1)\}$ be the space of symmetric $L^2$ functions over the product domain $\Omega\times\Omega$. Notice that under the log transformation, we have $\text{log}(U) \in\mathcal{H}$. We proceed to model $\text{log}(U)$ in order to avoid the non-negativity constraint on $U$, a common approach in the literature \citep{moller1998}. With slight abuse of notation, from here on we denote $U := \text{log}(U)$. We assume $U$ to be a mean square continuous random function with realizations in $\mathcal{H}$ and associated measure $\mathbb{P}$ such that $\mathbb{E}_{\mathbb{P}}[U] = \mu\in \mathcal{H}$ and mean square integrable covariance function $C = \mathbb{E}_{\mathbb{P}}[(U-\mu)(U-\mu)]$. The spectral data of $C$ are defined by the integral equation 
\begin{equation}\label{eqn:integral_form_spectrum}
    \int_{\Omega\times\Omega}C(\omega_1,\omega_2, \omega_1^*,\omega_2^*)\psi_k( \omega_1^*,\omega_2^*)d\omega_1^*d\omega_2^* = \rho_k\psi_k(\omega_1,\omega_2) \quad k=1,2,...,
\end{equation}
and by Mercer's theorem, the covariance function can be written as 
$C(\omega_1,\omega_2, \omega_1^*,\omega_2^*) = \overset{\infty}{\underset{k=1}{\sum}}\rho_k \psi_k(\omega_1,\omega_2)\psi_k( \omega_1^*,\omega_2^*)$. By the Karhunen-Lo\`{e}ve theorem, we have the decomposition $U(\omega_1, \omega_2) = \mu(\omega_1,\omega_2) + \sum_{k=1}^\infty Z_k\psi_k(\omega_1, \omega_2)$, where $Z_k = \langle U - \mu, \psi_k\rangle_{L^2(\Omega\times\Omega)}$ are independent, mean zero random variables with $\mathbb{E}_{\mathbb{P}}[Z_k^2] = \rho_k$. 
\par 
The eigenfunctions possess another desirable property, namely, the first $K$ form the best rank $K$ basis for representing realizations of $U$. In practice, this makes them very useful for forming finite rank approximations to infinite dimensional random functions. Of course, the eigenfunctions are unknown and must be estimated from the data using a procedure known as functional principal components analysis (FPCA). A common approach to FPCA is to form a smoothed estimate $\widehat{C}$ and then perform a spectral decomposition over some finite dimensional basis system or discretization of the domain. However, both of these approaches are infeasible in the current situation due to the curse of dimensionality, as $C$ is a symmetric PSD function defined over an $8$-D manifold domain. This prompt us to look for an alternative reduced rank solution, which we outline next. 
\par 
Invoking the best rank $K$ property of the eigenfunctions, an alternative definition to \eqref{eqn:integral_form_spectrum} is given by the (unique) solutions to 
\begin{equation}\label{eqn:theoretical_fpca}
    \begin{aligned}
        \{\psi_k\}_{k=1}^K = \underset{\{e_k\in \mathcal{H}\}_{k=1}^K}{\text{argmin}} \quad & \mathbb{E}_{\mathbb{P}}\Big\|U - \mu - \overset{K}{\underset{k=1}{\sum}} Z_ke_k\Big\|^2_{L^2(\Omega\times\Omega)} \\
        \textrm{s.t.} \quad & \langle e_k, e_j\rangle_{L^2(\Omega\times\Omega)} = \delta_{k,j},
    \end{aligned}
\end{equation}
where $\delta_{k,j}$ is the Kronecker delta. This formulation does not explicitly require the pre-estimation of the $C$, and thus avoids the associated dimension doubling effect. However, it still requires solving an optimization problem over $\mathcal{H}$, the space of symmetric functions on $\Omega\times\Omega$, itself a product space of two 2D submanifolds of $\mathbb{R}^3$, so the curse of dimensionality is still problematic. In order to circumvent this issue, we look for multiplicatively separable solutions to \eqref{eqn:theoretical_fpca}, that is, we assume $e_k(\omega_1,\omega_2) = e_{k1}(\omega_1)e_{k2}(\omega_2):=e_{k1}\cdot e_{k2}$. Coupled with the symmetry of the $\mathcal{H}$, it follows that $e_{k1}\equiv e_{k2}:=e_k$. 
\par 
It is also desirable that the solutions have local support. Basis systems with local support are widely used, e.g. splines/wavelets, owing to several advantageous properties. In the context of the current work, the local support property allows the association of the basis function coefficients to localized regions on the cortical surface. In turn, this permits efficient spatially localized inference by performing inference directly on the coefficients, which can be done with existing multivariate techniques. With this in mind, we define the optimal collection of $K$ separable locally supported basis functions as the solutions to
\begin{equation}\label{eqn:theoretical_separable_fpca}
    \begin{aligned}
        \{\xi_k\}_{k=1}^K = \underset{\{e_k\in L^{2}(\Omega)\}_{k=1}^{K}}{\text{argmin}}\quad & \mathbb{E}_{\mathbb{P}}\Big\|U - \mu - \overset{K}{\underset{k=1}{\sum}} S_ke_k\cdot e_k\Big\|^2_{L^2(\Omega\times\Omega)} \\
        \textrm{s.t.} \quad & \langle e_k, e_j\rangle_{L^2(\Omega)} = \delta_{k,j}\\
        & \text{Con}_{SP}(e_k) := \int_{\Omega}\mathbb{I}\{e_k(\omega)\neq 0\}d\omega \le \alpha_2 \text{ for }k=1,...,K
    \end{aligned}
\end{equation}
where $S_k = \langle U - \mu, e_k\cdot e_k\rangle_{L^2(\Omega\times\Omega)}$. $\text{Con}_{SP}$ measures the total area of the support of the $\xi_k$ and is incorporated in order to mandate that the basis functions have the local support property. 
\par 
In general, $\psi_k \neq \xi_k\cdot\xi_k$, so while $\text{span}\left(\{\xi_k\cdot\xi_k\}_{k=1}^K\right)$ is not the optimal rank $K$ space for representing realizations of $U$, it does offer a desirable trade-off between flexibility and computational complexity. In regard to the latter, notice that \eqref{eqn:theoretical_separable_fpca} is an optimization problem over $L^2(\Omega)$, while \eqref{eqn:theoretical_fpca} is an optimization problem over $\mathcal{H}\subset L^{2}(\Omega\times\Omega)$, thus we obtain both dimensionality reduction and avoid a symmetry constraint on our search space. In regard to the former, it can be shown that $\{\xi_k\cdot\xi_k\}_{k=1}^K$ is a complete basis system for $\mathcal{H}$ as $K\rightarrow\infty$, and thus are universal approximators for our function space of interest. For a more detailed analysis of the approximation properties of the theoretically optimal separable basis system including converge rate analysis and a quantification of the cost associated with the separable assumption, see \cite{consagra2021}.

%With model (\ref{eqn:generative_model}) and the observed $\{O_i\}$, we are ready to estimate the aligned ConCons $f^*_i$. One possibility is a complete likelihood based approach; however it is problematic for several reasons. First, likelihood estimation is often computationally demanding for inference in doubly stochastic Poisson process models for spatial point patterns \citep{diggle2013}. Other important challenges in the current set-up include the massive sizes of the point patterns (each can contain more than 1 million streamlines/endpoints), the exotic product manifold domain $\Omega\times\Omega$, the infinite dimensional nuisance diffeomorphism $\gamma$ and the large sample size $N$ (e.g., $N \approx 1000$ in the HCP data we considered). Due to these issues, we avoid exact likelihood based inference of \eqref{eqn:generative_model} and instead we propose a faster and multi-step method: first estimate $f_i$ according to $O_i$, and then estimate $(\gamma_i^1,\gamma_i^2)$ so that we can get $f^*_i$. 

%From the observed point process $O_i$, there are many ways to estimate $f_i$, including some parametric methods \citep{baddeley2007spatial} and non-parametric ones \citep{helmers2003consistent,ellison2014kernel,moyer2017,cole2021}. We follow the procedure in \cite{moyer2017} and \cite{cole2021} to use a kernel density estimation method to estimate $f_i$, where a heat kernel on sphere is extended to the space of $\Omega \times \Omega$. To represent $f_i$, we impose a mesh grid on $\Omega$ and sample values between any pair of vertices.   \textcolor{red}{Figure xx panel (a) shows the method grid, panel (b) shows the heat kernel we used to estimated $f_i$ from $O_i$, and panel (c) shows an example of $f_i$ sampled on the mesh grid.} To align between subjects, we simply take the alignment produced by freesurfer, and apply it to obtained $f^*_i$. Note that the alignment is produced according to geometric features such as the folding patterns \citep{fischl1999high} instead of the connectome feature $f_i$. A direct alignment between subjects based on $f_i$ is still unavailable, and we do not handle this problem given its complexity in this paper. 

%\subsection{High Resolution Structural Connectivity}\label{ssec:high_resolution_connectivitiy}

%Due to the massive size of the point sets, we can confidently apply smoothing techniques to form estimates of the intensity function $u_i$ from $Y_i = (\gamma_i\times\gamma_i)^{-1}\circ(O_i)$, for each subject independently. We can then model the stochastic structure of $U$ by formulating a functional principal components analysis on the smoothed estimates. Clearly this requires an initial estimate of $\gamma_i$, which can be constructed from $\Omega_i$ using a spherical registration algorithm. In practice, the SCBI described in \citep{cole2021}, which implements both the registration \citep{robinson2014} and smoothing \citep{moyer2017} steps, can be applied to each subject to obtain estimates $\hat{u}_i$ at each point on a user defined grid
%$
%\boldsymbol{V} := (\boldsymbol{v}_{11}, \boldsymbol{v}_{12}, ..., \boldsymbol{v}_{1n_{1}}, \boldsymbol{v}_{21}, \boldsymbol{v}_{22}, ..., \boldsymbol{v}_{2n_{2}})^\prime
%$
%where each vector of marginal points $\boldsymbol{V}_d := (\boldsymbol{v}_{d1}, \boldsymbol{v}_{d2}, ..., \boldsymbol{v}_{dn_{d}})\in \mathbb{S}^2_d$, $d=1,2$. That is, for each of the $i=1,..,N$ subjects, we can construct the data matrix 
%$$
%    \boldsymbol{Y}^{(i)} =\begin{bmatrix}
%                            \boldsymbol{Y}_{11}^{(i)}  & \boldsymbol{Y}_{12}^{(i)}  \\
%                            \boldsymbol{Y}_{12}^{(i)\prime}& \boldsymbol{Y}_{22}^{(i)}
%                        \end{bmatrix};  
%$$
%where $,\boldsymbol{Y}_{d_{1}d_{2}}^{(i)} \in \mathbb{R}^{n_{d_{1}}\times n_{d_{2}}}$ whose $l,j$ elements is given by $\hat{u}_i(\boldsymbol{v}_{d_{1}l}, \boldsymbol{v}_{d_{2}j})$, for $d_{1},d_{2}\in\{1,2\}$ where $\boldsymbol{v}_l \in \boldsymbol{V}_{d_{1}}$, $\boldsymbol{v}_j \in \boldsymbol{V}_{d_{2}}$. 

 
%The grid is user specified and can be made arbitrarily dense and therefore $\boldsymbol{Y}^{(i)}$ can be considered as the high-resolution analogues of the traditional Atlas-based structural connectome matrices and therefore in theory can be modeled using the existing latent graph embedding mentioned in Section~\ref{sec:introduction}. In practice, the super-high dimensionality of data renders many of the standard algorithms computationally infeasible, see Section~\ref{sec:simulation}. In the following section we propose a methodology for modeling the high-resolution connectivity which represents the data into a collection of continuous, symmetric spatial functions. We show that under mild structural assumptions, we are able to derive a tractable estimation algorithm that can handle arbitrarily dense $\boldsymbol{V}$.   

\section{Methods}\label{sec:methods}

\subsection{Smoothed Empirical Optimization Problem}
We would like to form estimates $\{\hat{\xi}_k, \widehat{S}_{ik}\}$ for $i=1,...,N$, $k=1,...,K$ from a sample of streamline endpoints $\{O_1, ..., O_N\}$. One possibility is a full likelihood based approach under model \eqref{eqn:generative_model}; however this is problematic for several reasons. First, likelihood estimation is often computationally demanding for inference in doubly stochastic Poisson process models for spatial point patterns \citep{diggle2013}. Further exacerbating problems in the current set-up are the massive sizes of the point patterns (each can contain more than 1 million streamlines), the exotic product manifold domain $\Omega\times\Omega$, the infinite dimensional nuisance $W_d$ and the large sample size $N$. Due to these issues, we avoid exact likelihood based inference of \eqref{eqn:generative_model} and instead we adopt a strategy common in the functional data analysis literature and propose a ``smooth first, then estimate'' approach \citep{zhang2007}.
\par 
Let $H_{h}:\Omega\times\Omega\mapsto \mathbb{R}^{+} \cup \{0\}$ be a kernel function with bandwidth $h > 0$. At any pair of locations, we can form the point-wise estimate for the $i$'th subject 
\begin{equation}\label{eqn:KDE_cc}
    \widehat{U}_i(\omega_1,\omega_2) = \text{log}\left(\sum_{({\bf p}^{ij}_1,{\bf p}^{ij}_2)\in O_i} H_{h}((\omega_1,\omega_2)|(\gamma_i^1({\bf p}^{ij}_1),\gamma_i^2({\bf p}^{ij}_2)) + 1\right).
\end{equation}
Due to the massive sizes of the point sets,  $|O_i|$ can be on the order of millions, we can be confident that the local estimates from \eqref{eqn:KDE_cc} will be accurate. Denote $\boldsymbol{\xi}_{K} := (\xi_1, ..., \xi_K)^\prime$, let $\boldsymbol{S}\in\mathbb{R}^{N\times K}$ be the matrix of subject specific coefficients and let $\boldsymbol{S}_{i}:= \text{diag}(S_{i1}, ..., S_{iK})$ be the diagonal coefficient matrix for the $i$th sample. We propose to form estimates $\hat{\xi}_k$ and associated $\widehat{S}_{ik}$ by solving the smoothed, regularized empirical counterpart of \eqref{eqn:theoretical_separable_fpca}, given by
\begin{equation}\label{eqn:empirical_separable_fpca}
\begin{aligned}
        (\{\hat{\xi}_k\}_{k=1}^K, \widehat{\boldsymbol{S}}) = &\underset{\underset{ \boldsymbol{S}\in\mathbb{R}^{N\times K}}{\xi_k\in L^2(\Omega)}}{\text{argmin}} \quad  \frac{1}{N}\sum_{i=1}^N\left\| \widehat{U}_{i} - \widehat{\mu} - \boldsymbol{\xi}_{K}^\prime\boldsymbol{S}_i\boldsymbol{\xi}_{K} \right\|_{L^2(\Omega\times\Omega)}^2 + \sum_{k=1}^K\alpha_{1}\text{Pen}_{R}(\xi_k) \\ 
        & \text{Pen}_{R}(\xi_k) := \int_{\Omega} |\nabla_{\Omega} \xi_k(\omega)|^2d\omega \\ 
        & \qquad \textrm{s.t.} \quad  \langle \xi_k, \xi_j\rangle_{L^2(\Omega)} = \delta_{k,j}\\
        & \qquad\qquad\text{Con}_{SP}(\xi_k) := \int_{\Omega}\mathbb{I}\{\xi_k(\omega)\neq 0\}d\omega \le \alpha_2 \text{ for }k=1,...,K
\end{aligned}
\end{equation}
where $\widehat{\mu}$ is the empirical mean of the $\widehat{U}_i$'s and $\alpha_{1},\alpha_{2} > 0$. $\text{Pen}_{R}$ is a ``roughness'' penalty, defined using the integrated quadratic variation of the candidate solution. The incorporation of roughness penalties in functional estimators is a standard practice, done in order to ameliorate the effect of the error in estimates $\widehat{U}_i$ and promote smooth solutions. 

\subsection{Marginal Spherical Spline Representation}\label{ssec:marg_splines}
Let $\{\phi_{j}\}_{j=1}^\infty$ be a complete basis system for $L^2(\mathbb{S}^2)$, which can be trivially extended to the domain of interest since $L^2(\Omega) := \text{span}(\{\phi_{j}\})\cup \text{span}(\{\phi_{j}\})$. Denote the $M_d$-dimensional truncation $\boldsymbol{\phi}_{M_{d}} = (\phi_1, ..., \phi_{M_{d}})^\prime$ and the corresponding extension of over $\Omega$ as $\mathcal{H}_{M_{1},M_{2}} := \text{span}(\boldsymbol{\phi}_{M_{d}})\cup\text{span}(\boldsymbol{\phi}_{M_{2}})$. 
Recalling that \eqref{eqn:empirical_separable_fpca} is an optimization problem over an infinite dimension space, to facilitate tractable estimation of the functional parameter $\xi_k$, we model $\xi_k\in\mathcal{H}_{M_{1},M_{2}}$, that is, we assume the optimal separable basis functions can be expressed
\begin{equation}\label{eqn:basis_expansion}
 \xi_{k}(\omega) = \boldsymbol{c}_{1,k}^\prime\boldsymbol{\phi}_{M_{1}}(\omega)\mathbb{I}\{\omega\in\mathbb{S}^2_1\} + \mathbb{I}\{\omega\in\mathbb{S}^2_2\}\boldsymbol{c}_{2,k}^\prime\boldsymbol{\phi}_{M_{2}}(\omega),
\end{equation}
where the $\boldsymbol{c}_{d,k} \in \mathbb{R}^{M_{d}}$ are the vectors of coefficients with respect to the basis $\boldsymbol{\phi}_{M_{d}}$. In theory, $\boldsymbol{\phi}$ can be taken as any complete basis system for $L^2(\mathbb{S}^2)$. In practice, we use spherical splines basis of degree 1, i.e. piecewise linear basis functions defined over a spherical triangulation. Linear spherical splines have many appealing properties, including local support, which, as we will see, is paramount for efficiently incorporating the local support constraint on the $\xi_k$ into our estimation algorithm. For completeness, we give a brief overview of the construction of linear spherical splines. We refer the interested reader to \cite{lai2007} for a more thorough treatment.
\par 
Define a spherical triangle $T$ with vertices $\boldsymbol{v}_1, \boldsymbol{v}_2, \boldsymbol{v}_3$, as the set of points in $\mathbb{S}^2$ that are bounded by the great circle arcs connecting $(\boldsymbol{v}_{i}, \boldsymbol{v}_{i+1})$, $i=1,2,3$ and $\boldsymbol{v}_4\equiv \boldsymbol{v}_1$. A collection of spherical triangles $\mathcal{T} = \{T_j\}_{j=1}^J$ is a spherical triangulation of $\mathbb{S}^2$, provided that the intersection between any two elements in $\mathcal{T}$ is empty, a common vertex or a common edge and $\mathbb{S}^2 = \bigcup_{T_j\in\mathcal{T}} T_j$. The \textit{spherical Delaunay triangulation} is the unique triangulation over a set of points $\{\boldsymbol{v}_m\}_{m=1}^M$ such that the minimum angle in the triangulation is as large as possible.
\par 
For each spherical triangle $T_j$, we can define a local coordinate system called the \textit{spherical barycentric coordinates}, defined for $\boldsymbol{v}\in T_i$ to be the nonnegative real numbers satisfying 
$$
    \boldsymbol{v} = b_1(\boldsymbol{v})\boldsymbol{v}_1 + b_2(\boldsymbol{v})\boldsymbol{v}_3 + b_3(\boldsymbol{v})\boldsymbol{v}_3.
$$
We can define the linear spherical Bernstein basis on $T_j$ as the span of the three nodal basis functions $\mathcal{B} := \text{span}\left(\{b_1(\boldsymbol{v}), b_2(\boldsymbol{v}), b_3(\boldsymbol{v})\}\right)$. That is, for any $s(\boldsymbol{v}) \in \mathcal{B}$, there exists coefficients $c_1,c_2,c_3$ such that $s(\boldsymbol{v}) = \sum_{j=1}^3c_jb_j(\boldsymbol{v})$.
The local basis functions defined for each spherical triangle can be ``glued together'' to form a piecewise continuous linear spline space over $\mathbb{S}^2$. Following \cite{lai2007}, we define 
$$
    \mathcal{S}_1^0(\mathcal{T}) = \{s\in C^0(\mathbb{S}^2):s|_{T_{j}}\in \mathcal{B},\quad\text{for}\quad j=1,...,J\}.
$$
An explicit basis for $ \mathcal{S}_1^0(\mathcal{T})$ can be constructed as follows: for each vertices $\boldsymbol{v}_m$ in tessellation $\mathcal{T}$, let $\phi_j\in\mathcal{S}_1^0(\mathcal{T})$ such that
$$
    \phi_j(\boldsymbol{v}_m) = \begin{cases}
      1 & \text{ if } j=m\\
      0 & \text{ otherwise}
    \end{cases}.
$$
It can be shown that $\phi_j$ is unique and that $\{\phi_j\}_{j=1}^M$ forms a basis for $\mathcal{S}_1^0(\mathcal{T})$ \citep{lai2007}.
%\par 
%The $\{\phi_j\}$ have several attractive properties. Efficient algorithms exist for evaluating and computing their directional derivative using the local basis functions \citep{schumaker2015}. For scattered data approximation, the $L^2$ rate of convergence of the least squares minimizer in $\mathcal{S}_d^0(\mathcal{T})$ for $g$ with $\beta+1$ continuous derivatives is $\mathcal{O}(|\mathcal{T}|^{\beta})$, where $|\mathcal{T}| = \max_{T\in\mathcal{T}}|T|$ with $|T|$ being the length of the longest arc in $T$ and any degree $d$. Although the rate depends on the smoothness of the unknown function, it is independent of the degree $d$ and hence in the ``fine grid'' regime, we do not gain approximation power by considering any spline basis of order larger than 1. 
\par 
Under the spherical spline model for the $\xi_k$'s, the optimization problem \eqref{eqn:empirical_separable_fpca} can be reformulated with respect to the finite dimensional parameters $\{\boldsymbol{c}_{d,k}\}$. Define $\boldsymbol{C}_d = \left[ \boldsymbol{c}_{d,1}, ..., \boldsymbol{c}_{d, K}\right]$, $\boldsymbol{C} = \left[\boldsymbol{C}_1,\boldsymbol{C}_2\right]^\prime$, $\boldsymbol{\phi}_M = (\boldsymbol{\phi}_{M_{1}}^\prime,\boldsymbol{\phi}_{M_{2}}^\prime)^\prime$, where $M = M_{1}+M_{2}$, and let $\mathcal{T}_d$ be the spherical triangulation defining $\boldsymbol{\phi}_{M_{d}}$. Define $\boldsymbol{F}_d(\boldsymbol{v})\in\mathbb{R}^{M_{d}\times 3}$ to be the Jacobian of $\boldsymbol{\phi}_{M_{d}}$ and denote the inner product matrices 
$$
\boldsymbol{R}_{\boldsymbol{\phi}} = 
\begin{bmatrix}
\boldsymbol{R}_1 & \boldsymbol{0} \\
\boldsymbol{0} & \boldsymbol{R}_2 
\end{bmatrix} = \begin{bmatrix} \int_{\mathbb{S}^2}\boldsymbol{F}_{1}\boldsymbol{F}^\prime_{1} & \boldsymbol{0} \\ \boldsymbol{0} & \int_{\mathbb{S}^2}\boldsymbol{F}_{2}\boldsymbol{F}^\prime_{2} \end{bmatrix}; \quad 
\boldsymbol{J}_{\phi} = \begin{bmatrix} 
\int_{\mathbb{S}^2}\boldsymbol{\phi}_{M_{1}}\boldsymbol{\phi}_{M_{1}}^\prime & \boldsymbol{0} \\
\boldsymbol{0} &  \int_{\mathbb{S}^2}\boldsymbol{\phi}_{M_{2}}\boldsymbol{\phi}_{M_{2}}^\prime
\end{bmatrix}.
$$
Then optimization problem \eqref{eqn:empirical_separable_fpca} can be written as 
\begin{equation}\label{eqn:SSSB_empirical_optm}
\begin{aligned}
        (\widehat{\boldsymbol{C}}, \widehat{\boldsymbol{S}}) = &\underset{\underset{\boldsymbol{S}\in\mathbb{R}^{N\times K}}{\boldsymbol{C}\in\mathbb{R}^{M\times K}}}{\text{argmin}} \quad  \frac{1}{N}\sum_{i=1}^N\left\| \widehat{U}_{i} - \widehat{\mu} -  \boldsymbol{\phi}_M^\prime\boldsymbol{C}\boldsymbol{S}_i\boldsymbol{C}^\prime\boldsymbol{\phi}_M \right\|_{L^2(\Omega\times\Omega)}^2 + \alpha_1\text{trace}(\boldsymbol{C}^\prime\boldsymbol{R}_{\boldsymbol{\phi}}\boldsymbol{C}) \\ 
        & \qquad \textrm{s.t.} \quad \boldsymbol{C}^\prime\boldsymbol{J}_{\boldsymbol{\phi}}\boldsymbol{C} = \boldsymbol{I} \\
        & \sum_{d=1}^2\sum_{T_{dj}\in \mathcal{T}_d}\text{area}(T_{dj})\mathbb{I}\{\boldsymbol{C}_{d,j_{d},k}\neq 0, \text{ for some } j_{d} \in \text{vertex}(T_{dj})\} \le \alpha_2,\text{ for }k=1,...,K \\
\end{aligned}
\end{equation}
where $\text{area}(T_{dj})$ is the surface area measure, $\text{vertex}(T_{dj})$ is a function that returns the indices of the vertices of spherical triangle $T_{dj}$, and $\boldsymbol{I}$ is the identity matrix. Efficient algorithms exist for evaluating spherical splines, computing their directional derivatives as well as performing integration. As a result the matrices $\boldsymbol{J}_{\boldsymbol{\phi}}$ and $\boldsymbol{R}_{\boldsymbol{\phi}}$ can be constructed cheaply. For more information on how to compute the required gradients and integrals, see the Supplementary Materials or \cite{schumaker2015} for a more thorough treatment. 
\begin{remark}
The number of unknown parameters to estimate in a rank $K$ separable basis under the marginal representation \eqref{eqn:basis_expansion} is given by $K(M+N)$, compared to $NM^2/2$ in the corresponding (symmetric) tensor product basis. Since the global rank $K$ can typically be made much smaller than either of the marginal ranks $M_1,M_2$, this can amount to a dramatic reduction in the number of unknown parameters.
\end{remark}

\subsection{A Relaxed Discretization}\label{ssec:relaxed_disc}

Notice that, under the spine representation of the marginal basis, $\text{Pen}_{R}$ is translated into a simple convex function of the unknown coefficient matrix $\boldsymbol{C}$. On the other hand, while the local support property of the splines does allow for some simplification, $\text{Con}_{SP}$ is a highly non-trivial function of $\boldsymbol{C}$. In order to facilitate the development of a computationally feasible optimization algorithm, we relax the the local support constraint to be the $\|\cdot\|_{0}$ of the $k$'th column of $\boldsymbol{C}$. This is justifiable due to choosing $\boldsymbol{\phi}_M$ to be locally supported itself. If we assume that $\max\left\{\text{area}(T_{dj})\right\}_{d,j} - \min\left\{\text{area}(T_{dj})\right\}_{d,j}$ is relatively small, then the number of non-zero coefficients provides a good proxy for a quantity proportional to $\text{Con}_{SP}$. 
\par 
Employing a standard approach in estimation for functional data, we discretize the loss function of \eqref{eqn:SSSB_empirical_optm} over a dense grid on $\Omega\times\Omega$. Define the mesh $\boldsymbol{X} := (\boldsymbol{x}_{11}, ..., \boldsymbol{x}_{1n_{1}}, \boldsymbol{x}_{22}, ..., \boldsymbol{x}_{2n_{2}})^\prime\subset\Omega$,
where each vector of marginal points $\boldsymbol{X}_d := (\boldsymbol{x}_{d1}, \boldsymbol{x}_{d2}, ..., \boldsymbol{x}_{dn_{d}})\in \mathbb{S}^2_d$, $d=1,2$. For each of the $i=1,..,N$ subjects, define the matrix:
$\boldsymbol{Y}_{i} =\begin{bmatrix}
                            \boldsymbol{Y}_{i,11} & \boldsymbol{Y}_{i,12}  \\
                            \boldsymbol{Y}_{i,12}^{\prime}& \boldsymbol{Y}_{i,22}
                        \end{bmatrix}$,
where $\boldsymbol{Y}_{i,d_{1}d_{2}} \in \mathbb{R}^{n_{d_{1}}\times n_{d_{2}}}$ whose $l,j$ elements is given by $\widehat{U}_i(\boldsymbol{x}_{d_{1}l}, \boldsymbol{x}_{d_{2}j})$, formed according to \eqref{eqn:KDE_cc}, where $\boldsymbol{x}_{d_{1}l} \in \boldsymbol{X}_{d_{1}}$, $\boldsymbol{x}_{d_{2}j} \in \boldsymbol{X}_{d_{2}}$. Define $\boldsymbol{\Phi}_d\in\mathbb{R}^{n_d \times M_{d}}$ to be the matrix of evaluations of $\boldsymbol{\phi}_{M_{d}}$ over $\boldsymbol{X}_d$ and define the block matrix $\boldsymbol{\Phi} = \begin{bmatrix} 
                       \boldsymbol{\Phi}_1 & \boldsymbol{0} \\
                        \boldsymbol{0} &\boldsymbol{\Phi}_2
                \end{bmatrix}$. The discretized, relaxed formulation of \eqref{eqn:SSSB_empirical_optm}
is given by 
\begin{equation}\label{eqn:SSSB_empirical_optm_relaxed_discrete}
\begin{aligned}
    (\widehat{\boldsymbol{C}}, \widehat{\boldsymbol{S}}) = \underset{\underset{\boldsymbol{S}\in\mathbb{R}^{N\times K}}{\boldsymbol{C}\in\mathbb{R}^{M\times K}}}{\text{argmin}} & \quad  \frac{1}{Nn_1n_2}\sum_{i=1}^N\left\| \boldsymbol{Y}_i^c  - \boldsymbol{\Phi}\boldsymbol{C}\boldsymbol{S}_i\boldsymbol{C}^\prime\boldsymbol{\Phi}^\prime \right\|_{F}^2 + \alpha_1\text{trace}(\boldsymbol{C}^\prime\boldsymbol{R}_{\boldsymbol{\phi}}\boldsymbol{C}) \\ 
    \textrm{s.t} \quad &  \boldsymbol{C}^\prime\boldsymbol{J}_{\phi}\boldsymbol{C} = \boldsymbol{I}, \qquad \left\|\boldsymbol{C}_{:,k}\right\|_0 \le n_{\alpha_{2}} \text{ for }k=1,...,K
\end{aligned}
\end{equation}
where $\boldsymbol{Y}_i^{c} = \boldsymbol{Y}_i  - \bar{\boldsymbol{Y}}$, $\bar{\boldsymbol{Y}}$ is the mean of the $\boldsymbol{Y}^{(i)}$'s, $\boldsymbol{C}_{:,k}$ indicates the $k$'th column of $\boldsymbol{C}$ and $n_{\alpha_{2}}$ is an integer depending on $\alpha_2$.
\subsection{Algorithm}\label{ssec:algorithm} 
The practical requirement to estimate models with relatively large $M_1,M_2$ and $K$ demands a scalable and efficient procedure to solve problem \eqref{eqn:SSSB_empirical_optm_relaxed_discrete}. However, an exact solution to \eqref{eqn:SSSB_empirical_optm_relaxed_discrete} is, in general,  computationally infeasible, as it is both non-convex and NP-hard \citep{hillar2013}. Therefore, we propose a novel greedy algorithm which forms an approximation by solving a sequence of rank-1 problems. Denote $\mathcal{Y}$ as the $(n_1 + n_2) \times (n_1 + n_2) \times N$-dimensional semi-symmetric tensor obtained from a mode-3 stacking of the $\boldsymbol{Y}_i^{c}$. Using properties of the Frobenius tensor norm, it is straight forward to show that the rank-1 formulation of \eqref{eqn:SSSB_empirical_optm_relaxed_discrete} is given by:
\begin{equation}\label{eqn:SSSB_empirical_optm_relaxed_discrete_rank1}
\begin{aligned}
    \min_{\boldsymbol{c}, \boldsymbol{s}} \quad & \frac{1}{Nn_1n_2}\left\| \mathcal{Y}^{(k)} - \boldsymbol{\Phi}\boldsymbol{c} \otimes \boldsymbol{\Phi}\boldsymbol{c}\otimes(s \boldsymbol{s}) \right\|_{F}^2 + \alpha_1 \boldsymbol{c}^\prime\boldsymbol{R}_{\boldsymbol{\phi}}\boldsymbol{c}\\
    \textrm{s.t.} \quad & \|\boldsymbol{s}\|_{2}=1; \quad s>0\\
  & \boldsymbol{c}^\prime\boldsymbol{J}_{\boldsymbol{\phi}}\boldsymbol{c_j} = 0\text{ for }j=1,...,k-1; \quad \boldsymbol{c}^\prime\boldsymbol{J}_{\boldsymbol{\phi}}\boldsymbol{c} =1 \\
  & \left\|\boldsymbol{c}\right\|_{0} \le n_{\alpha_{2}}
\end{aligned}
\end{equation}
for ranks $k=1,...,K$, where $\mathcal{Y}^{(k)}  = \mathcal{Y} - \sum_{j=1}^{k-1}\boldsymbol{\Phi}\boldsymbol{c}^{*}_j \otimes \boldsymbol{\Phi}\boldsymbol{c}^{*}_j\otimes (s_j \boldsymbol{s}^{*}_j)$ is the residual tensor,  $(\boldsymbol{c}^{*}_j, \boldsymbol{s}^{*}_j)$ are the rank-1 solutions from the $j$th iteration and $s_j = \mathcal{Y}^{(j)}  \times_1 \boldsymbol{\Phi}\boldsymbol{c}^{*}_j \times_2 \boldsymbol{\Phi}\boldsymbol{c}^{*}_j \times_3 \boldsymbol{s}^{*}_j$ is the scale. Note that $\times_d$ and $\otimes$ denote the $d$-mode multiplication and outer product, respectively. The rank-1 problem \eqref{eqn:SSSB_empirical_optm_relaxed_discrete_rank1} is still non-convex and NP-hard, hence an approximation is formed using an alternating optimization method with variable blocks $\boldsymbol{c}$ and $\boldsymbol{s}$. This procedure is described in the following. 
\par 
Denote the the singular value decomposition $\boldsymbol{\Phi}_d = \boldsymbol{U}_d\boldsymbol{D}_d\boldsymbol{V}_d^\prime$, define the block matrices 
$$
\boldsymbol{V} = \begin{bmatrix} 
                        \boldsymbol{V}_1 & \boldsymbol{0} \\
                        \boldsymbol{0} & \boldsymbol{V}_2
                \end{bmatrix}, \qquad 
                 \boldsymbol{D} = \begin{bmatrix} 
                        \boldsymbol{D}_1 & \boldsymbol{0} \\
                        \boldsymbol{0} & \boldsymbol{D}_2
                \end{bmatrix}, \qquad \boldsymbol{U} = \begin{bmatrix} 
                        \boldsymbol{U}_1 & \boldsymbol{0} \\
                        \boldsymbol{0} & \boldsymbol{U}_2
                \end{bmatrix},
$$
and define the transformed tensor $\mathcal{G}^{(k)} := \mathcal{Y}^{(k)}\times_1\boldsymbol{U}^\prime\times\boldsymbol{U}^\prime$.
The update for block variable $\boldsymbol{c}$ at the $t+1$ iteration is given by 
\begin{equation}\label{eqn:ctilde_update}
\begin{aligned}
    \boldsymbol{c}^{(t+1)} = \text{max} &\quad \boldsymbol{b}^\prime\left[\boldsymbol{V}\boldsymbol{D}\left(\boldsymbol{I} - \boldsymbol{P}_{k-1}\right)\left[2\mathcal{G}^{(k)}\times_3\boldsymbol{s}^{(t)} - \alpha_1\boldsymbol{R}\right]\left(\boldsymbol{I} - \boldsymbol{P}_{k-1}^{\prime}\right)\boldsymbol{D}\boldsymbol{V}^\prime\right]\boldsymbol{b} \\
    & \textrm{s.t.} \quad \left\|\boldsymbol{b}\right\|_{\boldsymbol{J}_{\boldsymbol{\phi}}} = 1, \quad \left\|\boldsymbol{b}\right\|_{0} \le n_{\alpha_{2}}, \\
\end{aligned}
\end{equation}
where 
\begin{equation}\label{eqn:update_P}
        \boldsymbol{P}_{k-1} = \boldsymbol{D}\boldsymbol{V}^\prime\boldsymbol{C}_{k-1}^{*}\left[\boldsymbol{C}_{k-1}^{*\prime}\boldsymbol{J}_{\boldsymbol{\phi}}\boldsymbol{C}_{k-1}^{*}\right]^{-1}\boldsymbol{C}_{k-1}^{*\prime}\boldsymbol{J}_{\boldsymbol{\phi}}\boldsymbol{V}\boldsymbol{D}^{-1}  \quad \boldsymbol{C}_{k-1}^{*} := \left[\boldsymbol{c}^{*}_1, ..., \boldsymbol{c}^{*}_{k-1}\right].
\end{equation}
For block variable $\boldsymbol{s}$, the update at the $t+1$ iteration is given in closed form by 
\begin{equation}\label{eqn:s_update}
       \boldsymbol{s}^{(t+1)} = \frac{\mathcal{G}^{(k)}  \times_1 \left(\boldsymbol{D}\boldsymbol{V}^\prime\boldsymbol{c}^{(t+1)}\right)
          \times_2 \left(\boldsymbol{D}\boldsymbol{V}^\prime\boldsymbol{c}^{(t+1)}\right)}{\left\|\mathcal{G}^{(k)}  \times_1 \left(\boldsymbol{D}\boldsymbol{V}^\prime\boldsymbol{c}^{(t+1)}\right)
          \times_2 \left(\boldsymbol{D}\boldsymbol{V}^\prime\boldsymbol{c}^{(t+1)}\right)\right\|_2}.
\end{equation}
For detailed derivation of the updates \eqref{eqn:ctilde_update} and \eqref{eqn:s_update}, please visit the Supplementary Materials.
\par 
All of the matrices involved in the matrix product in \eqref{eqn:ctilde_update} can be precomputed, save the mode-3 product term, which costs $O(NM^2)$. An approximation to $\boldsymbol{c}^{(t+1)}$ can be obtained using the truncated power iterations method from \cite{yuan2011}, outlined by Algorithm~\ref{alg:ttpm} for completeness, at a computational cost of $O\left(n_{\alpha_{2}}M\right)$ per iteration. The $d$-mode multiplications needed to form \eqref{eqn:s_update} can be computed at a computational cost of $O\left(N\left(1+ M + M^2\right) + M^2\right)$, where $O\left(NM^2\right)$ and $O\left(NM\right)$ come from the first $1$-mode and $2$-mode products, the $O(M^2)$ comes from the matrix transformation of the $\boldsymbol{c}^{(t+1)}$ and the $O(N)$ comes from the normalization. Notice that, since $\mathcal{G}^{(k)}$ can be precomputed, the complexity of the updates are independent of the number of grid points used in the discretization $(n_1+n_2)$. Since typically $M \ll n_1+n_2$, this can amount to an enormous savings in computation when compared to an alternative approach of performing tensor decomposition directly on $\mathcal{Y}$.
\par 
Algorithm~\ref{alg:rank_1_ssb} provides pseudocode for the proposed scheme. 
The block update \eqref{eqn:ctilde_update} requires an initialization for $\boldsymbol{c}^{(0)}$ and $\boldsymbol{s}^{(0)}$. Consider the rank-1 model of $\mathcal{Y}$, whose mode-1 and mode-3 matricization have the form 
\begin{equation}\label{eqn:krp_prop}
         \left(\boldsymbol{\Phi}\boldsymbol{c} \otimes \boldsymbol{\Phi}\boldsymbol{c}  \otimes(s \boldsymbol{s}) \right)_{(1)} = \boldsymbol{\Phi}\boldsymbol{c}\left(\boldsymbol{\Phi}\boldsymbol{c} \odot (s\boldsymbol{s})\right)^\prime, \quad 
         \left(\boldsymbol{\Phi}\boldsymbol{c} \otimes \boldsymbol{\Phi}\boldsymbol{c}  \otimes(s \boldsymbol{s}) \right)_{(3)} = s\boldsymbol{s}\left(\boldsymbol{\Phi}\boldsymbol{c} \odot \boldsymbol{\Phi}\boldsymbol{c}\right)^\prime
\end{equation}
where $\odot$ denotes the Krocker product and the $_{(d)}$ notation indicates the $d$-mode matricization. Therefore, for the $k$'th rank-1 factor, the leading left singular vectors of $\mathcal{Y}^{(k)}_{(1)}$ and $\mathcal{Y}^{(k)}_{(3)}$ are a reasonable initialization for the block variables $\boldsymbol{c}^{(0)}$ and $\boldsymbol{s}^{(0)}$, respectively. That said, we would like to limit any computations that scale with $n_1+n_2$. Alternatively, notice that under the same rank-1 model for $\mathcal{Y}^{(k)}$ we have
$$
\begin{aligned}
    \mathcal{G} &= \mathcal{Y}\times_1 \boldsymbol{U}^\prime\times_2\boldsymbol{U}^\prime \\
    &= \left(\boldsymbol{\Phi}\boldsymbol{c} \otimes \boldsymbol{\Phi}\boldsymbol{c}  \otimes(s \boldsymbol{s}) \right)\times_1 \boldsymbol{U}^\prime\times_2\boldsymbol{U}^\prime \\
    &=  \left(\boldsymbol{D}\boldsymbol{V}^\prime\boldsymbol{c} \otimes \boldsymbol{D}\boldsymbol{V}^\prime\boldsymbol{c}  \otimes(s \boldsymbol{s}) \right).
\end{aligned}
$$
The property of the Kronecker property used in \eqref{eqn:krp_prop} indicates that we may equivalently use the leading left singular vectors of $\mathcal{G}^{(k)}_{(1)}$ and  $\mathcal{G}^{(k)}_{(3)}$, thus avoiding a computation that scales with the grid. In practice, these can be computed efficiently using power iterations on the symmetric matrices $\mathcal{G}^{(k)}_{(1)}\mathcal{G}^{(k)^\prime}_{(1)}$ and $\mathcal{G}^{(k)}_{(3)}\mathcal{G}^{(k)^\prime}_{(3)}$. We conclude the section with a couple remarks. 

\begin{remark}
By proposition 3 in \cite{yuan2011}, the iterates produced by Algorithm~\ref{alg:ttpm} are guaranteed to monotonically increase the objective function for positive semi-definite (PSD) matrices. The matrix $$
\left[\boldsymbol{V}\boldsymbol{D}\left(\boldsymbol{I} - \boldsymbol{P}_{k-1}\right)\left[2\mathcal{G}^{(k)}\times_3\boldsymbol{s} - \alpha_1\boldsymbol{R}\right]\left(\boldsymbol{I} - \boldsymbol{P}_{k-1}^{\prime}\right)\boldsymbol{D}\boldsymbol{V}^\prime\right]$$
is not guaranteed to be PSD, but can easily be forced to be by adding a small ridge penalty. Establishing global convergence of alternating optimization algorithms, of which Algorithm~\ref{alg:rank_1_ssb} is an example of,to a fixed point of the objective typically requires establishing the existence and uniqueness (EU) of the solutions for all the block updates \cite{bezdek2003}. While the EU for \eqref{eqn:s_update} is trivial, the EU for the sparse eigenvector problem in \eqref{eqn:ctilde_update} ... 
\end{remark}

\begin{remark}
In practice,  Algorithm~\ref{alg:rank_1_ssb} will estimate $\xi_k$'s that are \textit{nearly} orthogonal. This is an artifact of post-estimate theresholding operation in the truncated power method.  
\end{remark}

\begin{algorithm}
\caption{Truncated Power Iterations from \cite{yuan2011} to solve \eqref{eqn:ctilde_update}}
\label{alg:ttpm}
\begin{algorithmic}[1]
\State \textbf{Input}: symmetric matrix $\boldsymbol{M}$, initial guess $\boldsymbol{x}^{(0)}$, number of non-zero components $n_{\alpha_{2}}$
\State \textbf{Output}: $\boldsymbol{x}^{(t+1)}$
\While{\text{Not Converged}}
\State $\boldsymbol{x}^{(t+1)} \gets \boldsymbol{M}\boldsymbol{x}^{(t)}/\left\|\boldsymbol{M}\boldsymbol{x}^{(t)}\right\|$
\State Set all but $n_{\alpha_{2}}$ largest (in absolute magnitude) components of $\boldsymbol{x}^{(t+1)}$ to zero
\State $\boldsymbol{x}^{(t+1)} \gets \boldsymbol{x}^{(t+1)}/\left\|\boldsymbol{x}^{(t+1)}\right\|$
\EndWhile
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Algorithm to approximate \eqref{eqn:SSSB_empirical_optm_relaxed_discrete_rank1}}\label{alg:rank_1_ssb}
\begin{algorithmic}[1]
\State \textbf{Input}: $\text{Tensor }\mathcal{Y}; \text{ matrices }\boldsymbol{J}_{\boldsymbol{\phi}}, \boldsymbol{R}_{\boldsymbol{\phi}}, \boldsymbol{U},\boldsymbol{V},\boldsymbol{D};  \text{ rank }K; \text{ hyperparameters } \alpha_1, n_{\alpha_{2}}$
\State \textbf{Output}: $\boldsymbol{C}, \boldsymbol{S}$
\State \textbf{Initialize}: $\mathcal{G}^{(1)} \gets  \mathcal{G} := \mathcal{Y}\times_1\boldsymbol{U}^\prime\times_2\boldsymbol{U}^\prime$; $\boldsymbol{C} \gets \emptyset$; $\boldsymbol{S}\gets \emptyset$; $\boldsymbol{P}_0\gets \boldsymbol{0}_{M\times M}$
\For{$k=1,...K$}
    \State \textbf{Initialize} $\boldsymbol{s}_k^{(0)}$ and  $\boldsymbol{c}_k^{(1)}$ using the left singular vectors of $\mathcal{G}^{(k)}_{(3)}$ and $\mathcal{G}^{(k)}_{(1)}$, respectively
    \While{\text{Not Converged}}
        \State 
        \State \textbf{Update} $\boldsymbol{c}_k^{(t+1)}$ according to \eqref{eqn:ctilde_update} using initial guess $\boldsymbol{c}_k^{(t)}$
        \State \textbf{Update} $\boldsymbol{s}_k^{(t+1)}$ according to \eqref{eqn:s_update}
    \EndWhile
    \State Compute $\boldsymbol{P}_k$ using \eqref{eqn:update_P}
    \State $s_k \gets \mathcal{G}^{(k)} \times_1 \left(\boldsymbol{D}\boldsymbol{V}^\prime\boldsymbol{c}_k^{(t+1)}\right) \times_2 \left(\boldsymbol{D}\boldsymbol{V}^\prime\boldsymbol{c}_k^{(t+1)}\right) \times_3 \boldsymbol{s}_k^{(t+1)}$
    \State $\mathcal{G}^{(k+1)} \gets \mathcal{G}^{(k)}- \left(\boldsymbol{D}\boldsymbol{V}^\prime\boldsymbol{c}_k^{(t+1)}\right) \otimes \left(\boldsymbol{D}\boldsymbol{V}^\prime\boldsymbol{c}_k^{(t+1)}\right) \otimes (s_k \boldsymbol{s}_k^{(t+1)})$
    \State $\boldsymbol{C} \gets \left[\boldsymbol{C};\boldsymbol{c}_k^{(t+1)}\right]$
    \State $\boldsymbol{S} \gets \left[\boldsymbol{S}; (s_k\boldsymbol{s}_k^{(t+1)})\right]$
\EndFor

\end{algorithmic}
\end{algorithm}

\subsection{Hyperparameter Selection}\label{sssec:hyper_param_select}

\noindent{\bf Spherical Triangulation}
\par\bigskip
For piecewise linear spherical splines, there is a 1-1 correspondence between the approximation properties of span$(\boldsymbol{\phi}_{M_{d}})$ and the tessellation $\mathcal{T}_d$. It is known that the accuracy of this approximation is highly dependent on both the the geometric properties of $T_{dj}\in \mathcal{T}_{d}$, the spatial distribution of vertices and the properties of the unknown function \citep{shewchuk2002,chen2004}. It is therefore likely that, for a fixed $M_d$, adapting $\mathcal{T}_d$ based on the distributional properties of $U$ would result in basis systems that have strong performance. In this work, we use a simple heuristic to design $\mathcal{T}_d$, independently for each copy of $\mathbb{S}^2$, using a crude estimate of the marginal functional variance, and leave a more principled method as an interesting direction for future work. Our technique consists of the following the steps: i) initiate a dense set of (nearly) equispaced vertices over $\mathbb{S}^2$ ii) assign a positive weight to each vertex using the variance of the row vector of the $\boldsymbol{Y}^{c}_i$'s corresponding to the closest mesh point iii) retain the top $M_d$ vertices sorted by weight iv) define $T_d$ to be the spherical Delaunay tessellation over this refined vertex set. This rather simple procedure can clearly be improved, but it was observed to consistently result in better $L^2$ reconstruction performance than the (nearly) equispaced vertex strategy for the same $M_d$.
\par\bigskip
\noindent{\bf Penalty Parameters and Ranks}
\par\bigskip
Algorithm~\ref{alg:rank_1_ssb} requires a specification of the penalty strength parameter $\alpha_1$, which dictates the degree of smoothness in the solution, as well as the $n_{\alpha_{2}}$, which determines the size of the support of the $\xi_k$'s. In practice, $\alpha_1$ can be selected through cross validation or through experimentation. In our analysis, we found small values were preferable, likely due to the fact that the functional data is already relatively smooth. The local support parameter $n_{\alpha_{2}}$ was chosen based on a quantile threshold.
\par 
It is also important to select both the marginal and global ranks, $M_1, M_2$ and $K$, respectively. The global rank can be selected using a threshold criteria on the estimated proportion of variance explained, estimated using the transformed tensor by $\left\|\mathcal{G}^{(K)}\right\|_{F}^2/\left\|\mathcal{G}\right\|_{F}^2$. Obtaining a simple criteria for selecting the marginal ranks is less straightforward. As this is intimately related the the spherical triangulation selection problem, we leave a principled marginal rank selection procedure as an interesting direction for future work. In this work, they were selected using experimentation. 
\par\bigskip
\noindent{\bf Kernel Smoothing}
\par\bigskip
The estimator \eqref{eqn:KDE_cc} depends on the choice of kernel function $H$, the bandwidth $h$ as well as the diffeomorphisms $(\gamma_i^1,\gamma_i^2)$, the latter of which are unobserved and therefore must be estimated. Given the assumption $U\perp W_1, W_2$ in \eqref{eqn:generative_model}, the diffeomorphisms can be estimated independently of the connectivity data using standard techniques and then plugged into  \eqref{eqn:KDE_cc}. Briefly, the cortical surfaces $S_d$ and corresponding homeomorphism are estimated from the T1 images, e.g. using freesurfer. Estimates $(\hat{\gamma}_i^1,\hat{\gamma}_i^2)$ are then obtained by applying a spherical registration algorithm \citep{yeo2010} to the $\mathbb{S}^2$ inflated representation of $S_d$. We take $H$ to be the product heat kernel from \cite{moyer2017}. The bandwidth $h$ can be selected per-subject using the leave-one-out procedure from the same reference. 

\subsection{Inference for Continuous Connectivity}\label{ssec:inference}

We are often interested in making comparisons between the structural connectivity of two groups. That is, in the most general sense, given a sample $\{U_{11}, U_{21}, ..., U_{N_{1}1},  U_{12},  U_{21}, ..., U_{N_{2}2}\}$ with $U_{i1} \sim U_1$ and $U_{i2} \sim U_2$, we are interested in testing $U_1 \overset{\text{dist}}{=} U_2$, where $U_j$ is the random ConCon for group $j=1,2$. Moreover, we are typically not only interested in whether the connectivity is different between the groups but \textit{where} this difference manifests on $\Omega\times\Omega$. This is known as local inference in the context of functional data. A common approach for local inference is to first represent the data using some basis system with local support and then perform testing on the coefficients of the expansion, since the coefficients effect can be localized on the domain. Since we explicitly formulate the $\xi_k$'s to have the local support property, we can adopt the same tactic to perform inference on the cortical surface. In particular, the inference procedure can be conducted in the following three steps: i) represent each $U_{ij}$ using the $\xi_k$'s (either pre-trained or estimated from the sample), ii) apply a univariate permutation test on each of the coefficients iii) adjust the p-values using an appropriate multiple testing correction.

%\section{Simulation Studies}\label{sec:simulation}
%\subsection{Computational Efficiency Comparisons}
%\subsection{Convergence Under Separability}
%\subsection{Selection of Marginal and Global Ranks}

\section{Application}\label{sec:real_data_experiments}

In this section, we ...

\subsection{Dataset and Preprocessing}
We apply our method to a datasets consisting of subjects from both the HCP scan-rescan dataset and the HCP 1200 subjects release. For each subject, we used both the dMRI and the structural T1-weighted images. The imaging acquisition protocol as well as the minimal preprocessing pipeline applied to the dMRI data are given in \cite{glasser2013}, which includes susceptibility induced distortion correction and motion correction using FSL \citep{smith2004}. After preprocessing, the \texttt{scilpy} pipeline was applied to the dMRI data to perform surface enhanced tractography. The tractography results were used to construct both continuous and atlas based representations. In particular, continuous SC estimates for each subject were computed on a $4,121 \times 4,121$ grid on $\Omega\times\Omega$ using the techniques outline in \cite{cole2021}. Binary and streamline count based adjacency matrices were constructed using both the Desikan \citep{desikan2006} and Destriex \citep{destrieux2010} atlases for comparison. 
\par 
For CC estimation, the marginal basis system $\phi_1$ and $\phi_2$ were set as spherical spline basis with $M_1=M_2=410$ piecewise linear basis functions. The spherical tessellation was formed using the sequential vertex removal procedure outlined in the Supplemental Material. 

\subsection{Reproducibility}
In this section we analyze the reproducibility of the continuous representations using the HPC scan-rescan data. This data consists of a subset of HCP subjects for whom two scans were collected during different sessions several months apart. In absence of disease, we expect the brain organization of a healthy adult to be relatively constant over the span of several months and therefore the scans can be considered as independent samples of the same connectome, making this data appealing for evaluating the reproducibility of a method. 
\par 
We used the subjects scan-1 data to form estimates $\hat{\xi}_k$ according to the procedure in Section~\ref{sec:methods}. For several $K$, the basis functions $\{\hat{\xi}_1, ...,\hat{\xi}_K\}$ were fixed and used to represent the scan-2 high resolution connectivity data by standard basis expansion under the least squares principle. The pairwise $L^2(\Omega\times\Omega)$ distances between the continuous representations of all the scan-1 and scan-2 data were computed. A quantitative assessment of the reproducibility was obtained using the leave-one-out cross validated (LOOCV) accuracy of a simple nearest neighbor classifier applied to the distances: for each representation $i$, we compute $j = \text{argmin}_{l\neq i} \text{dist}(i,l)$, where $\text{dist}(i,l)$ is shorthand for the $L^2(\Omega\times\Omega)$ distance between continuous representation $i$ and $l$. The LOOCV accuracy is computed as the fraction of examples where $i$ and $j$ are two scans corresponding to the same individual. Figure~\ref{fig:reproducibility_analysis} displays the resulting pairwise distance matrices and LOOCV accuracy results. The two scans corresponding to the same subject were put next to one another in order to form the observed block diagonal pattern. We note that the block diagonal pattern is prominent displayed even when using only $K=8$ basis functions. The data driven function space resulting from the first $K=22$ basis functions fully separates the data under the standard $L^2(\Omega\times\Omega)$ metric. 

\begin{figure}
    \centering
   \includegraphics[scale=0.7]{Figures/reproducibility.pdf}
    \caption{Pairwise $L^2(\Omega\times\Omega)$ distance matrices with elements being distances between the scan-1 and scan-2 continuous connectivity representations for several $K$'s. The LOOCV accuracy of the nearest neighbor classier applied to the distances is also recorded.}
    \label{fig:reproducibility_analysis}
\end{figure}

\subsection{Trait Prediction}

Associated with each HCP subject are a set of 175 measurements related to various cognitive, physical, socioeconomic and psychiatric factors. The measurements are hierarchically grouped into \textit{assessment} and \textit{category}. For instance, the score on the \textit{NIH Toolbox Sadness Survey} (measurement) is measuring \textit{Negative Affect} (assessment) which is an \textit{Emotion} (category). Many of the measurements under the same assessment were found to be highly correlated with one another. Therefore, to decorrelate and reduce the number of measures, we constructed a set of \textit{derived measures} using PCA. In particular, we first grouped the measurements at the assessment level, discarding any that were binary or categorical. The assessments considered were: fluid intelligence, processing speed, self regulation and impulse control, sustained attention, executive function, psychiatric, taste, emotional recognition, anger and hostility and finally BMI and weight. This resulted in 81 total outcomes. A PCA was performed on each of the assessement level groupings and the first $n$ PCs that explained $\ge 90\%$ of the variance were selected. Each subjects measurements were then projected onto each of the principal directions, which were used as outcomes for the trait prediction task. In all, there were 31 of these. 
\par 
We compare the predictive power of the SC-embeddings constructed from the proposed framework, i.e. the coefficients $\boldsymbol{S}$, to those obtained from several alternative state-of-the-art network embedding methods, namely Tensor-Network PCA (TN-PCA) \citep{zhang2019}, Multiple Random Dot-Product Graph model (MRDPG) \citep{nielsen2018} and Multiple Adjacency Spectral Embedding method (MASE) \citep{arroyo2021b}. Each method was applied to connectome matrices constructed from both the Desikan and Destriex atlas-based streamline count representation of the SC data. TN-PCA can be applied directly to the count data, while MRDPG and MASE require a binarization of the connectome matrices. $K=100$ embedding dimensions were used for all methods, except MRDPG applied to the Desikan atlas, since this method requires $K\le V$, and hence we let $K=68$. For the CC representations, we again use a spherical spline basis with $M_1=M_2=410$ piecewise linear basis functions as the marginal basis system on both copies of $\mathbb{S}^2$. TN-PCA, MRDPG and MASE all have publicly available implementations that were utilized for this study. 
\par 
We now describe the predictive modeling framework. The embeddings were used as features in a predictive model for the various outcomes of interest. Specifically, a LASSO regression model was used as a predictor. For each outcome of interest, we performed 100 random 80-20 train-test splits of the data. The LASSO regularization paths were computed using the training data and the model associated with the penalty parameter resulting in the minimum mean cross validated error was chosen, unless this resulted in the null model, in which case the model consisting of the first 5 features included in the regularization paths was selected. The selected model was then applied to the test set and both the resulting Pearson correlation and mean squared error were recorded. Any outcome whose predictions were not deemed significantly associated ($\rho > 0.1$) with \textit{any} of the embedding framework were discarded from analysis. In all, 15 out of the original 31 outcomes were deemed significant.
\par 
Table~\ref{tab:concon_vs_atlas} records the Pearson correlation averaged over the random train-test splits for the significant outcomes from all embedding techniques. The outcomes are labeled with the convention \textit{assessment}-PC number. Comparing CC to the results of the best predictions from the competitor network embeddings from either atlas, (Destriex atlas shown in Table~\ref{tab:concon_vs_atlas}(a) and Desikan atlas shown in Table~\ref{tab:concon_vs_atlas}(b)), our method improves on the field in 11 out of 15 outcomes. In several cases, the improvement is quite dramatic, e.g. Anger and Hostility-2, BMI and Weight-1,  Executive Function-2. This suggests potentially large gains in the predictive capability when using connectivity data at much higher resolutions than are commonly being pursued currently. Furthermore, comparing the results from Table~\ref{tab:concon_vs_atlas}(a) and (b), we see that in many cases, the results are highly sensitive to the choice of atlas. This highlights another important advantage of the proposed framework, namely, we avoid any confounding introduced by choice of parcellation scheme. Any prediction or inference based on the CC framework will be inherently be atlas-free. 

\begin{table}
\centering
\small
\caption{Pearson correlation averaged over the 100 random train-test splits for outcomes significantly correlated with predictions using any of the embedding models. Standard deviations are shown in parentheses. The embedding technique whose associated predictions were most highly correlated with the outcome is embolden.}
\subcaption*{(a) Results for CC along with TN-PCA, MASE, and MRDPG using the Destriex atlas.}
\begin{tabular}{r|rrrrr}
\toprule
 &  \multicolumn{4}{c}{\textbf{Embedding}} \\
 Outcome & CC & TN-PCA & MASE & MRDPG \\
\midrule
Fluid Intelligence-1  &   0.1530 (0.0853) &      0.1122 (0.0692) &     0.1321 (0.0765) &     0.1235 (0.0839) \\
Self Regulation-1     &   \textbf{0.2079} (0.0932) &     -0.0460 (0.0902) &     0.1280 (0.0810) &     0.1410 (0.0856) \\
Self Regulation-3     &   0.0329 (0.0838) &      0.0464 (0.1026) &    -0.0117 (0.0811) &     0.1289 (0.0966) \\
Sustained Attention-2 &   \textbf{0.1228} (0.0922) &     -0.0412 (0.0844) &    -0.0343 (0.0830) &    -0.0031 (0.0924) \\
Executive Function-1  &   \textbf{0.1085} (0.1033) &      0.1072 (0.0790) &     0.0415  (0.0788) &     0.0881 (0.0753) \\
Executive Function-2  &   \textbf{0.1441} (0.0757) &     -0.0116 (0.0918) &    -0.0631 (0.0859) &     0.0521 (0.1016) \\
Psychiatric-3         &   \textbf{0.1128} (0.0884) &     -0.0470 (0.0797) &    -0.0107 (0.1025) &    -0.0274 (0.0791) \\
Psychiatric-6         &  -0.0376 (0.0872) &      \textbf{0.1277} (0.0862) &     0.1001 (0.0852) &     0.1239 (0.0957) \\
Taste-1               &   \textbf{0.1236} (0.0815) &      0.0164 (0.0873) &     0.0466 (0.0800) &     0.0214 (0.0868) \\
Emotion Recognition-1 &   \textbf{0.1058} (0.0834) &      0.0895 (0.0910) &     0.0896 (0.0802) &     0.0160 (0.0826) \\
Emotion Recognition-2 &   0.0100 (0.0880) &      0.0489 (0.0887) &     \textbf{0.1145} (0.0827) &    -0.0436 (0.0921) \\
Emotion Recognition-4 &   \textbf{0.1591} (0.0873) &     -0.0329 (0.0840) &    -0.0659 (0.0895) &    -0.0349 (0.1017) \\
Anger and Hostility-2 &   \textbf{0.2216} (0.0871) &      0.0011 (0.0957) &    -0.0369 (0.0950) &    -0.0379 (0.0809) \\
Anger and Hostility-3 &   \textbf{0.2190} (0.0898) &     -0.0078 (0.0918) &     0.1850 (0.0904) &     0.0576 (0.0815) \\
BMI and Weight-1      &   \textbf{0.3046} (0.0858) &      0.2365 (0.0899) &     0.0866 (0.0855) &     0.1519 (0.0922) \\
\bottomrule
\end{tabular}
\bigskip
\subcaption*{(b) Results for TN-PCA, MASE, and MRDPG using the Desikan atlas.}
\begin{tabular}{r|rrrr}
\toprule
 &   \multicolumn{3}{c}{\textbf{Embedding}}  \\
 Outcome & TN-PCA & MASE & MRDPG \\
\midrule
Fluid Intelligence-1  &  \textbf{0.1752} (0.0865) &    -0.0873 (0.0792) & -0.0151  (0.0743) \\
Self Regulation-1     &  0.0975 (0.0866) &    -0.0172 (0.0939) &   -0.0027  (0.0949) \\
Self Regulation-3     &   \textbf{0.1334}  (0.1103) &     0.0006 (0.0952) &     -0.0811  (0.0855) \\
Sustained Attention-2 &   0.0183 (0.0975) &    -0.0605 (0.0904) &    -0.0890  (0.0720) \\
Executive Function-1  &    -0.0154 (0.0887) &     0.0455 (0.0869) &   0.0787  (0.0823) \\
Executive Function-2  &     -0.0481 (0.0849) &     0.0068 (0.0955) & 0.0008  (0.0774) \\
Psychiatric-3         &   0.0594 (0.0942) &    -0.0573 (0.0929) &  0.0091  (0.0862) \\
Psychiatric-6         &    -0.0323 (0.0730) &     0.0971 (0.0794) &  -0.0175  (0.0962) \\
Taste-1               &   -0.0943 (0.0869) &     0.0974 (0.0985) &  0.0368  (0.0817) \\
Emotion Recognition-1 &     0.0127 (0.0792) &     0.0826 (0.1017) &   0.0127  (0.0904) \\
Emotion Recognition-2 &      0.0343 (0.0864) &    -0.0519 (0.0798) &  -0.0064  (0.0925) \\
Emotion Recognition-4 &      0.1170 (0.1032) &    -0.0633 (0.0841) &  -0.0194  (0.0961) \\
Anger and Hostility-2 &     -0.0328 (0.0919) &    -0.0731 (0.0885) &   -0.0390  (0.0894) \\
Anger and Hostility-3 &       -0.0513 (0.0820) &     0.0505 (0.0832) &     0.1187 (0.0815) \\
BMI and Weight-1      &  0.2054 (0.0827) &     0.0493 (0.0896) &   0.0600  (0.0841)\\
\bottomrule
\end{tabular}
\label{tab:concon_vs_atlas}
\end{table}
%\begin{figure}
%    \centering
%    \includegraphics[scale=0.55]{Figures/SC_prediction_comparison.pdf}
%    \caption{Violin plots displaying the Pearson correlations computed over 100 random 80-20 train-test splits of the data.}
%    \label{fig:prediction_comparison}
%\end{figure}
%\par 
%For each outcome, we can define the relative importance of a feature by the fraction of times it was selected for inclusion in the final LASSO model. There are strong theoretic foundations for using such a measure of importance \citep{meinshausen2010}. Figure \ref{fig:SC_important_eigenfunctions} shows the spatial basis function associated with the most selected feature for \textit{fluid intelligence-1}, \textit{processing speed-1} and \textit{executive function-2}. For the executive function outcome, the leading basis function is active within areas of the lateral prefrontal cortex, an area known to be crucial to executive function tasks such as  inhibitory control and working memory \citep{yusuke2013}. The leading spatial functions associated with the fluid intelligence and processing speed measures are located within the temporal lobe, an area known to be related to general intelligence \citep{yoon2017}.

%\begin{figure}
%    \centering
%    \includegraphics{Figures/SC_important_eigenfunctions_cropped.pdf}
%    \caption{Marginal SC eigenfunctions associated with the most informative coefficients as quantified by inclusion rate in the predictive modeling task for several significant outcomes of interest.}
%    \label{fig:SC_important_eigenfunctions}
%\end{figure}

\subsection{Case Study: Self Regulation and Impulse Control}
Delay discounting refers to the subjective decline in the value of a reward when it's arrival is delayed in time. It is known that steep discounting is associated with a variety of psychiatric conditions, including antisocial personality disorders, drug abuse and pathological gambling \citep{odum2011}. The HCP collects several measures of delay discounting on each participant as a part of a self-regulation/impulsivity assessment. In this study we focus on one of the measures, namely, the subjective value of $\$200$ at 6 months. For this measure, a series of trials are performed in which the subject's are made to choose between two alternatives: $\$200$ in 6 months or a smaller amount today. For each trial, reward amounts are adjusted based on the subject's choices to iteratively determine an indifference amount that identifies the participants subjective value of $\$200$ at 6 months. For more information, we refer the interested reader to \cite{estle2006} or the \textit{WU-Minn HCP Quarter 1 (Q1) Data Release: Reference Manual}.
\par 
In this case study, we analyze the relationship between delay discounting and structural connectivity using the CC framework using the inference procedure discussed in Section~\ref{ssec:inference}. 

\iffalse 
In particular, we consider the univarite function-on-scalar regression model of the form:
$$
    U_{Li}(\omega_1,\omega_2) = \mu_L(\omega_1,\omega_2) + A_{i}\beta(\omega_1,\omega_2) + \theta_{i}(\omega_1,\omega_2)
$$
for $i = 1,...,N$, where $A_{i}$ is the subjective value of $\$200$ at 6 months for the $i'th$ subject,  $\beta$ is the fixed effect function and $\theta_{i}$ a mean zero stochastic process with covariance function $C$. We are interested in testing hypothesis of the form
$$
\begin{aligned}
   H_0:\beta(\omega_1,\omega_2)  &= 0 \text{ } \forall (\omega_1,\omega_2) \in \Omega\times\Omega  \\
   H_1:\beta(\omega_1,\omega_2) &\neq 0 \text{ for some } (\omega_1,\omega_2) \in \Omega\times\Omega
\end{aligned}
$$
A standard approach estimates the unknown functional parameter $\hat{\beta}$ by minimizing a least squares criterion over a sufficiently expressive basis system \citep{ramsay2005}, which we take to be $\{\hat{\xi}_1, ..., \hat{\xi}_K\}$. That is, we look for solutions $\hat{\beta} = \sum_{k=1}^K\hat{b}_k\hat{\xi}_k\hat{\xi}_k$, where 
$$
    \hat{\boldsymbol{b}} = \underset{\boldsymbol{b}\in\mathbb{R}^K}{\text{argmin}}\sum_{i}\left\|\sum_{k=1}^K \widehat{\boldsymbol{S}}_{ik}\hat{\xi}_k\hat{\xi}_k - A_i\sum_{k=1}^Kb_k\hat{\xi}_k\hat{\xi}_k\right\|_{\mathcal{H}}^2.
$$
Denoting $\boldsymbol{a} = (A_1, ..., A_N)$, the integrated model sum squared error (ISSE) is given by
$$
\begin{aligned}
    \text{ISSE} & := \int_{\Omega\times\Omega}\sum_{i}\left(\widehat{U}_{Li}(\omega_1,\omega_2) - \left[\hat{\mu}_{L}(\omega_1,\omega_2) + A_i\hat{\beta}(\omega_1,\omega_2)\right]\right)^2  \\
 &= \left\|\widehat{\boldsymbol{S}} - \boldsymbol{a}\hat{\boldsymbol{b}}^\prime\right\|_{F}^2.
\end{aligned}
$$
Notice that, under $H_0$, the distribution of ISSE is invariant to the reordering of $\boldsymbol{a}$ and thus the global significance of the testing problem can be assessed using a permutations. 
\par 
A p-value of $0.00195$ was computed using the empirical null distribution formed from 20,000 permutations, indicating an overall global significance. In order to evaluate the local effect, we examine the brain regions where $\hat{\beta}$ is extreme; which we define as cortical locations associated with the $99.5\%$ quantile of $|\hat{\beta}|$. The extreme values were coarsened using the Desikan atlas in order to display the connectivity information in Figure~\ref{fig:circle_graph}. The surviving connectivity pattern is within and between areas in the left and right frontal lobe as well within the left and right occipital lobe. Connectivity differences in a variety of areas in the frontal lobe has been shown to be related to delayed discounting. In particular, the left and right supramarginal gyrus (region 31) appears to be one of the most affected regions with multiple connections to in the frontal lobe. This is consistent with previous DTI studies finding significant differences in white matter integrity measures in this area \citep{olson2009}. In particular, strong connections with both the lingual gyrus (region 13) and supramarginal gyrus are present in both left and right hemispheres. These regions have also been implicated in delayed discounting \citep{owens2017}. Another area strong connection is between the caudal middle frontal gyrus and pars triangularis, areas which are known to be involved in both reasoning processes, modulating emotional responses and executive control of behavior \textcolor{blue}{http://www.fmriconsulting.com/brodmann/}. Additional areas in the frontal lobe whose connectivity is altered such as the rostral anterior cingulate cortex have also been shown to be related to impulse control in general and delay discounting in particular \citep{sebastian2014}. A fMRI studies have demonstrated increased activation in the left hemisphere of frontal lobe in delayed discounting tasks, a pattern reproduced here in the structural connectivity results \citep{wesley2014}. 

%Some studies have also found increased functional activity in the occipital lobe during delayed discounting tasks \citep{hinvest2011,luo2009}, lending credibility towards the structural findings. 
\par 
As $\hat{\beta}$ is represented using a linear combination of the optimal symmetric basis functions, the coefficient of this representation can be used to assess the importance or informativeness of continuous spatial pattern with in predicting delayed discounting. The estimated basis functions were observed to be sparse, in the sense that their values outsize a small localized region were near zero. This area, referred to as the ``active region'', can be obtained using simple thresholding. Each of the six color patches in Figure~\ref{fig:informative_eigenfunctions} indicate the active regions on the cortical surface for each of the six most informative basis functions.   
\begin{figure}
    \centering
    \includegraphics[scale=0.6]{Figures/impulse_control_13.pdf}
    \caption{Connectivity fixed effect function $\hat{\beta}$ discretized using the Desikan atlas. Only the regions where $|\hat{\beta}|$ exceeded it's 99.5\% percentile were incorporated.}
    \label{fig:circle_graph}
\end{figure}
Figure~\ref{fig:informative_eigenfunctions}
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Figures/delayed_discounting_MIEF.pdf}
    \caption{The most informative marginal basis functions as quantified by the magnitude of the associated regression coefficient in the estimate $\hat{\beta}$. Each color corresponds to the regions where $|\hat{\xi}_k|$ exceeded it's .99 quantile.}
    \label{fig:informative_eigenfunctions}
\end{figure}

\fi 

\section{Discussion and Future Directions}\label{sec:conclusion}

From a methodological point of view, there are several avenues along which I would like to extend the method. A principled way of adapting the spherical tessellation, hence the spline approximation space, to the properties of the distribution of $U$ would likely result in the ability to fit accurate models with far smaller marginal ranks than the current approach. It can be shown that the optimal tessellation for piecewise linear spline approximation of realizations from a random function is governed by the variance of the Hessian. In particular, the optimal tessellation elements should a) have vertices distributed according to a density function proportional to the determinant of the variance of the Hessian b) be equilateral under the Riemannian metric induced by the variance of the Hessian. We notice that this is closely related to the optimal meshing techniques found in the numerical partial differential equations literature, which seek meshes that are adapted to the properties of the dynamic system to produce solvers with greatly reduced approximation error \citep{du2003,du2005,xu2006}. Therefore, it seems likely that the algorithms used for optimal mesh adaptation can be re-purposed for our application. As a special case, formulating the optimal spherical triangulations under a piecewise constant estimator can be used to construct a data driven atlas for traditional connectome analysis. I am also interested in the possibility of scrapping the current pre-smoothing based estimation approach for a unified, likelihood based treatment of the generative model in Equation~\eqref{eqn:generative_model}, e.g. exploring GP-based priors on the random functions similar to the methods from \cite{john2018}.

\pagebreak
\begin{center}
\textbf{\LARGE Supplemental Materials}
\end{center}
\setcounter{equation}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{section}{0}
%\setcounter{page}{1}
\makeatletter
\renewcommand{\theequation}{S\arabic{equation}}
\renewcommand{\thefigure}{S\arabic{figure}}
\renewcommand{\thetable}{S\arabic{table}}
\renewcommand{\thesection}{S\arabic{section}}
\renewcommand{\bibnumfmt}[1]{[S#1]}
\renewcommand{\citenumfont}[1]{S#1}

\section{Theory}

\subsection{Functional Greedy Algorithm}\label{ssec:ff_greedy}

We begin with describing relevant notations. Denote $U^{c} := U - \mu$, define 
$$\mathcal{V} = \{\xi_k\cdot\xi_k: \xi_k \in L^2(\Omega), \langle \xi_k \xi_j\rangle_{L^{2}} = \delta_{kj},\text{ for }k = 1,2,...\}.$$
For $k=1,...,K$,
the fully functional greedy algorithm is defined by repeating the following steps 
\begin{equation}\label{eqn:greedy_algorithm}
\begin{aligned}
        \xi_k &= \mathbb{E}\left[\sup_{\xi\in\mathcal{V}} |\left\langle R_{k-1}, \xi\cdot\xi\right\rangle|^2\right] \\
    \quad R_{k} &= U^c - P_{k}(U^c) \\ 
\end{aligned}
\end{equation}
where $P_{k}$ is the orthogonal projection operator onto $\text{span}\left(\{\xi_1\cdot\xi_1, ..., \xi_k\cdot\xi_k\}\right)$. The procedure is initialized with $R_{0} = U^{c}$.
\begin{proposition}[Universal Approximation Property]\label{prop:uap}
$\mathcal{V}$ has the universal approximation property for $u\in \mathcal{H}$. That is, $\exists$ a countable index set $I$ such that
$$
\left\| u - \sum_{k \in I} c_k\xi_j\cdot\xi_j\right\|_{L^{2}} = 0.
$$
where $c_k \in\mathbb{R}$.
\end{proposition}
\begin{proof}
Let $\Gamma := \{\gamma_j: j=1,2,...\}$ be a complete orthogonal basis system for $L^2(\Omega)$. For instance, $\Gamma$ may be constructed using the spherical wavelet basis functions defined in \cite{lessig2008}, which form a complete orthogonal basis for $L^2(\mathbb{S}^2)$, and then trivially be extended to a basis for $L^2(\Omega)$ using the technique discussed previously. Then by definition, for $u \in \mathcal{H}\subset L^2(\Omega\times\Omega)$, we have that $u(\omega_1, \omega_2) = \sum_{j=1}^\infty\sum_{l=1}^\infty a_{jl}\gamma_{j}(\omega_1)\gamma_{l}(\omega_2)$, where $a_{jl} = a_{lj}$, due to symmetry. Denote the infinite symmetric matrix 
$$
A = \begin{bmatrix} a_{11} & a_{12} & a_{13} & \cdots \\
a_{21} & a_{22} &  a_{23} & \cdots\\
a_{31} & a_{32} &  a_{33} & \cdots\\
\vdots & \vdots &  \vdots & \vdots\\
\end{bmatrix}.
$$
Since $u \in L^2(\Omega\times\Omega)$, it follows that $\sum_{j=1}^\infty\sum_{l=1}^\infty a_{jl}^2 < \infty$ and therefore $A$ is a Hilbert–Schmidt operator on the space $l^2(\mathbb{N})$ and thus is compact. Then by the spectral theorem, there exists real eigenvalues $\{\lambda_k\}_{k=1}^\infty$ and orthogonal eigenvectors $\{e_k\}_{k=1}^\infty$ such that 
$$
A = \sum_{k=1}^\infty \lambda_ke_k\otimes e_k,
$$
\citep{Hsing2015TheoreticalFO}. Let $\xi_k = \sum_{j=1}^\infty e_{kj}\gamma_j(\omega)$, it follows that both 
$$
\begin{aligned}
    u(\omega_1, \omega_2) &= \sum_{j=1}^\infty\sum_{l=1}^\infty a_{jl}\gamma_{j}(\omega_1)\gamma_{l}(\omega_2) \\
    &= \sum_{j=1}^\infty\sum_{l=1}^\infty\sum_{k=1}^\infty \lambda_ke_{kj} e_{kl}\gamma_{j}(\omega_1)\gamma_{l}(\omega_2) \\ 
    &= \sum_{k=1}^\infty\lambda_k\left(\sum_{j=1}^\infty e_{kj}\gamma_{j}(\omega_1)\right)\left(\sum_{l=l}^\infty e_{kl}\gamma_{l}(\omega_1)\right) \\ 
    &= \sum_{k=1}^\infty \lambda_k \xi_k(\omega_1)\xi_k(\omega_2)
\end{aligned}
$$
and 
$$
\begin{aligned}
\langle\xi_k,\xi_m\rangle_{L^{2}} &= \int_{\Omega}\left(\sum_{j=1}^\infty e_{kj}\gamma_{j}(\omega)\right)\left(\sum_{l=l}^\infty e_{jl}\gamma_{l}(\omega)\right)d\omega \\
&= \sum_{j=1}^\infty\sum_{l=l}^\infty e_{kj}e_{jl}\int_{\Omega}\gamma_{j}(\omega)\gamma_{l}(\omega)d\omega \\
&= \sum_{j=1}^\infty e_{kj}e_{mj} = \delta_{km},
\end{aligned}
$$
completing the proof. 
\end{proof}
From here on for clarity, denote $S_{\xi_{j}} := \langle U^c, \xi_j\cdot \xi_j\rangle_{L^{2}}$.
By Proposition~\ref{prop:uap}, we have that, with probability 1, $U^{c} = \sum_{j\in I} S_{\xi_{j}} \xi_j\cdot\xi_j$. Since the $L^2$ norm is invariant to basis representation, it must be the case that 
$$\mathbb{E}\left[\|U^{c}\|_{L^{2}}^2\right] =  \sum_{j\in I} \mathbb{E}\left[S_{\xi_{j}}^2\right] = \sum_{k=1}^\infty\mathbb{E}\left[Z_k^2\right] = \sum_{k=1}^\infty\rho_k < \infty.
$$
On top of the second order moment condition that we essentially get ``for free'', in order to proceed we will make a stronger assumption on the function space which the $U$ inhabit. We begin by defining this space.
\begin{definition}\label{defn:smoothness_class}
Let $0 < B < \infty $ be a generic constant. Denote the class of functions $$
L_{1,B}(\mathcal{V}) := \{u \in \mathcal{H}: u = \sum_{\xi\in\mathcal{V}} S_{\xi}\xi\cdot\xi, \sum_{\xi\in\mathcal{V}} |S_{\xi}| \le B\},$$ 
and the associated norm 
$$
\left\|u\right\|_{L_{1,B}} := \sum_{\xi\in\mathcal{V}} |S_{\xi}|
$$
\end{definition}
\begin{assumption}\label{assm:smoothness_class}
There exists some $0 < B < \infty$ such that $U \in L_{1,B}(\mathcal{V})$, almost surely.
\end{assumption}

\begin{remark}
Assumption~\ref{assm:smoothness_class} can almost certainly be weekend, e.g. by defining $U$ as almost surely in the ``interpolation space'' between $\mathcal{H}$ and $L_{1,B}(\mathcal{V})$, as was the tactic in \cite{barron2008}. We leave an extension of our results for random functions in this more general space as a direction of future work.
\end{remark}

%\begin{assumption}\label{assm:moment_decay}
%Let $0 < B < \infty $ be a generic constant. We assume
%$$
%\sum_{j\in I}\mathbb{E}\left[S_{\xi_{j}}^2\right]^{1/2} = \sqrt{B}
%$$
%\end{assumption}
%\begin{remark}
%Assumption~\ref{assm:moment_decay} can be equivalently formulated as the following bound on moments of the tail coefficients.
%\begin{assumption}\label{assm:moment_bound}
%Let $\mathcal{V}_k$ be the collections of $\xi_k$ after $k$ iterations of the algorithm defined in equation~\eqref{eqn:greedy_algorithm}. We assume that $\exists K \in \mathbb{N}$ such that $\forall \xi \in \mathcal{V}\setminus \mathcal{V}_K$, we have 
%$$
%    \left\|\sum_{\xi \notin \mathcal{V}_k} \langle U_c, \xi \cdot\xi\rangle_{L^{2}}\xi\cdot\xi \right\|_{L^{2}} = O(k^{-r})
%$$
%for some $r > 0$.
%\end{assumption}
%\end{remark}

We are now ready to state our result on the convergence rate of the fully functional greedy algorithm.
\begin{theorem}[Convergence Rate of Fully Functional Greedy Algorithm]\label{thm:population_convergence_rate}
Under Assumption~\ref{assm:smoothness_class}, we have the following expected approximation error rate resulting from the greedy algorithm defined in equation~\eqref{eqn:greedy_algorithm}
$$
\mathbb{E}\left[\left\|R_{k}\right\|_{L^{2}}^2\right] = O(k^{-1})
$$
\end{theorem}
\begin{proof}
Notice that we can write
\begin{equation}\label{eqn:reccurence}
\begin{aligned}
    \left\|R_{k}\right\|_{L^{2}}^2 &= \left\| U^c - P_{k}(U^c)\right\|_{L^{2}}^2 \\
    &= \left\| U^c - P_{k-1}(U^c) - \langle U^c - P_{k-1}(U^c), \xi_k\cdot\xi_k\rangle \xi_k\cdot\xi_k\right\|_{L^{2}}^2  \\
    &= \left\| U^c - P_{k-1}(U^c)\right\|_{L^{2}}^2 - |\left\langle U^c - P_{k-1}(U^c), \xi_k\cdot\xi_k\right\rangle_{L^{2}}|^2 \\
    & \equiv \left\| R_{k-1}\right\|_{L^{2}}^2 - |\left\langle R_{k-1}, \xi_k\cdot\xi_k\right\rangle_{L^{2}}|^2 
\end{aligned}
\end{equation}
Furthermore,  
\begin{equation}\label{eqn:bound_prev_reccurence}
\begin{aligned}
    \left\| R_{k-1}\right\|_{L^{2}}^2 &=  \left\langle R_{k-1}, R_{k-1}\right\rangle_{L^{2}} \\ 
    &= \left\langle R_{k-1}, U^{c}\right\rangle_{L^{2}} \\
    &= \left\langle R_{k-1}, \sum_{j \in I} S_{\xi_{j}}\xi_{j}\cdot\xi_{j}\right\rangle_{L^{2}} \\
    &= \sum_{j \in I}S_{\xi_{j}}\left\langle R_{k-1},  \xi_{j}\cdot\xi_{j}\right\rangle_{L^{2}}\\ 
    &\le \sum_{j \in I}|S_{\xi_{j}}||\left\langle R_{k-1},  \xi_{j}\cdot\xi_{j}\right\rangle_{L^{2}}|\\
    &\le \sum_{j \in I}|S_{\xi_{j}}|\sup_{\xi\in\mathcal{V}}|\left\langle R_{k-1},  \xi\cdot\xi\right\rangle_{L^{2}}|
\end{aligned}
\end{equation}
Now, taking the expected value of \eqref{eqn:bound_prev_reccurence} and using Cauchy-Schwarz, we have that 
$$
\begin{aligned}
     \mathbb{E}\left[\sum_{j \in I}|S_{\xi_{j}}|\sup_{\xi\in\mathcal{V}}|\left\langle R_{k-1},  \xi\cdot\xi\right\rangle_{L^{2}}|\right] \le  \mathbb{E}\left[\left(\sum_{j \in I}|S_{\xi_{j}}|\right)^2\right]^{1/2}\mathbb{E}\left[\sup_{\xi\in\mathcal{V}}|\left\langle R_{k-1},  \xi\cdot\xi\right\rangle_{L^{2}}|^2\right]^{1/2} \\ 
\end{aligned}
$$
which gives the bound 
$$
 \mathbb{E}\left[ \left\| R_{k-1}\right\|_{L^{2}}^2\right]^2 \le \mathbb{E}\left[\left(\sum_{j \in I}|S_{\xi_{j}}|\right)^2\right]\mathbb{E}\left[\sup_{\xi\in\mathbb{D}}|\left\langle R_{k-1},  \xi\cdot\xi\right\rangle_{L^{2}}|^2\right].
$$
By the definition of our greedy selection algorithm, we have that
$$
\mathbb{E}\left[\sup_{\xi\in\mathcal{V}}|\left\langle R_{k-1},  \xi\cdot\xi\right\rangle_{L^{2}}|^2\right] = \mathbb{E}\left[|\left\langle R_{k-1},  \xi_k\cdot\xi_k\right\rangle_{L^{2}}|^2\right].
$$
Taking the expectation of \eqref{eqn:reccurence} and plugging in our results, we have that 
$$
\begin{aligned}
\mathbb{E}\left[\left\|R_{k}\right\|_{L^{2}}^2\right] &=  \mathbb{E}\left[\left\| R_{k-1}\right\|_{L^{2}}^2\right] - \mathbb{E}\left[|\left\langle R_{k-1}, \xi_k\cdot\xi_k\right\rangle_{L^{2}}|^2\right] \\
&\le \mathbb{E}\left[\left\| R_{k-1}\right\|_{L^{2}}^2\right]\left(1 - \frac{\mathbb{E}\left[\left\| R_{k-1}\right\|_{L^{2}}^2\right]}{\mathbb{E}\left[\left(\sum_{j \in I}|S_{\xi_{j}}|\right)^2\right]}\right) \\
& \le \mathbb{E}\left[\left\| R_{k-1}\right\|_{L^{2}}^2\right]\left(1 - \frac{\mathbb{E}\left[\left\| R_{k-1}\right\|_{L^{2}}^2\right]}{B^2}\right),
\end{aligned}
$$
where the final inequality comes from the fact that, under Assumption~\ref{assm:smoothness_class},
$$
\mathbb{E}\left[\left(\sum_{j \in I}|S_{\xi_{j}}|\right)^2\right] = \mathbb{E}\left[\left\|U\right\|_{L_{1,B}}^2 \right] \le B^2
$$
Furthermore, we have that 
$$
\begin{aligned}
    \mathbb{E}\left[\left\|R_{0}\right\|_{L^{2}}^2\right] &= \sum_{k=1}^\infty\mathbb{E}\left[Z_k^2\right] = \mathbb{E}\left[\sum_{j\in I}|S_{\xi_{j}}||S_{\xi_{j}}|\right] \\
    &\le \mathbb{E}\left[\left(\sum_{j\in I}|S_{\xi_{j}}|\right)\left(\sum_{k\in I}|S_{\xi_{k}}|\right)\right] \\
    &= \mathbb{E}\left[\left\|U\right\|_{L_{1,B}}^2 \right] \le B^2
\end{aligned}
$$
Hence the sequence $\{\mathbb{E}\left[\left\|R_{k}\right\|_{L^{2}}^2\right]\}_{k}$ is decreasing.
\par 
For clarity, denote $r_k := \mathbb{E}\left[\left\|R_{k}\right\|_{L^{2}}^2\right]$. Assume that $r_{k-1}\le \frac{B^2}{k}$ for any $k$. Then if $r_{k-1} \le \frac{B^2}{k+1}$, clearly $r_{k} \le \frac{B^2}{k+1}$ since it is a decreasing sequence. If $r_{k-1} \ge \frac{B^2}{k+1}$, then 
$r_k \le \frac{B^2}{k}\left(1 - B^{-2}\frac{B^2}{k+1}\right)= \frac{B^2}{k+1}$. Hence, by induction we have established that 
$$
\mathbb{E}\left[\left\|R_{k}\right\|_{L^{2}}^2\right] \le \frac{B^2}{k+1} = O(k^{-1}).
$$
\end{proof}

\subsection{An Empirical Formulation}

In practice, we do not know the true distribution $\mathbb{P}$, rather, that we have access to a sample of $N$ realizations of $U$. Hence, we must work with an empirical formulation of the greedy algorithm discussed in \eqref{eqn:greedy_algorithm}. Denote $R_{k,i} := U_i^{c} - P_k(U_i^{c})$, then the empirical algorithm is 
\begin{equation}\label{eqn:empirical_greedy_algorithm}
\begin{aligned}
        \xi_k &= \mathbb{E}_{N}\left[\sup_{\xi\in\mathcal{V}} |\left\langle R_{k-1,i}, \xi\cdot\xi\right\rangle|^2\right] \\
    \quad R_{k,i} &= U^c_i - P_{k}(U_i^c) \\ 
\end{aligned}
\end{equation}
For clarity, denote $S_{i,\xi_{j}} = \langle U^{c}_i, \xi_j\cdot\xi_j\rangle_{L^{2}}$.
The following result gives a probabilistic rate for the empirical residual.
\begin{theorem}\label{thrm:sample_convergence_rate}
Let $U_1, ..., U_N$ be i.i.d. with $U_i \sim U$ and let $t > 0$. Under Assumption~\ref{assm:smoothness_class}, with probability greater than $1 - 2\text{exp}\left(-2Nt^2/B^4\right)$, we have that the in-sample residual error rate resulting from the empirical greedy algorithm defined in equation~\eqref{eqn:empirical_greedy_algorithm}, is  
$$
N^{-1}\sum_{i=1}^N \left\|R_{k,i}\right\|_{L^{2}}^2 = O(k^{-1})
$$
\end{theorem}
\begin{proof}
Using the same logic as \eqref{eqn:reccurence} and \eqref{eqn:bound_prev_reccurence} we have that 
$$
\left\|R_{k,i}\right\|_{L^{2}}^2 = \left\|R_{k-1,i}\right\|_{L^{2}}^2 -  |\left\langle R_{k-1,i}, \xi_k\cdot\xi_k\right\rangle_{L^{2}}|^2 
$$
and 
$$
\left\|R_{k-1,i}\right\|_{L^{2}}^2 \le \sum_{j \in I}|S_{i,\xi_{j}}|\sup_{\xi\in\mathcal{V}}|\left\langle R_{k-1,i},  \xi\cdot\xi\right\rangle_{L^{2}}|.
$$
Furthermore, applying Cauchy-Schwarz to the empirical inner product, we have that 
$$
\begin{aligned}
N^{-1}\sum_{i=1}^N\sum_{j \in I}|S_{i,\xi_{j}}|\sup_{\xi\in\mathcal{V}}|\left\langle R_{k-1,i},  \xi\cdot\xi\right\rangle_{L^{2}}| &\le \left(N^{-1}\sum_{i=1}^N\left(\sum_{j \in I}|S_{i,\xi_{j}}|\right)^2\right)^{1/2}\times \\
&\left(N^{-1}\sum_{i=1}^N\sup_{\xi\in\mathcal{V}}|\left\langle R_{k-1,i},  \xi\cdot\xi\right\rangle_{L^{2}}|^2\right)^{1/2}.
\end{aligned}
$$
Combining these results, we obtain the relation 
\begin{equation}\label{eqn:empirical_recurrence}
    R^{(N)}_k \le R^{(N)}_{k-1}\left(1 - \frac{R^{(N)}_{k-1}}{U^{(N)}_{L_{1}}}\right).
\end{equation}
where
$$
    R^{(N)}_k := N^{-1}\sum_{i=1}^N\left\|R_{k,i}\right\|_{L^{2}}^2 \text{ and } U^{(N)}_{L_{1}} := N^{-1}\sum_{i=1}^N\left\|U_i\right\|_{L_{1,B}}^2
$$
for clarity. 
\par 
By Hoeffding's Inequality, for any $t>0$ we have that 
$$
\mathbb{P}\left(|N^{-1}\sum_{i=1}^N\left\|U_i\right\|_{L_{1,B}}^2 - \mathbb{E}\left[\left\|U\right\|_{L_{1,B}}^2\right]| \ge t\right)\le 2\text{exp}(-\frac{2Nt^2}{B^4}). 
$$
So with probability at least  $1 - 2\text{exp}(-\frac{2Nt^2}{B^4})$, we have 
$$
\begin{aligned}
N^{-1}\sum_{i=1}^N\left\|U_i\right\|_{L_{1,B}}^2 &= |N^{-1}\sum_{i=1}^N\left\|U_i\right\|_{L_{1,B}}^2 - \mathbb{E}\left[\left\|U\right\|_{L_{1,B}}^2\right] + \mathbb{E}\left[\left\|U\right\|_{L_{1,B}}^2\right]| \\ 
&\le |N^{-1}\sum_{i=1}^N\left\|U_i\right\|_{L_{1,B}}^2 - \mathbb{E}\left[\left\|U\right\|_{L_{1,B}}^2\right]| + \mathbb{E}\left[\left\|U\right\|_{L_{1,B}}^2\right] \\
&\le t + B^2.
\end{aligned}
$$
and 
\begin{equation}\label{eqn:empirical_recurrence_prop_bound}
    R^{(N)}_k \le R^{(N)}_{k-1} \left(1 - \frac{R^{(N)}_{k-1}}{t + B^2}\right).
\end{equation}
Finally we note that, with probability 1, $R^{(N)}_k\le B^2 + t$. The final result can be obtained by applying the same recursion argument as in the proof to Theorem~\ref{thm:population_convergence_rate}.
\end{proof}

\section{Empirical Optimization}

\subsection{Regularization and Sparsity}
In practice, the functional sample is discretely observed over a mesh. Therefore to promote smoother solutions we consider a regularized augmentation of the greedy update in \eqref{eqn:empirical_greedy_algorithm} given by 
\begin{equation}\label{eqn:regularized_sparse_empirical_update}
    \mathbb{E}_{N}\left[\sup_{\xi\in\mathcal{V}} |\left\langle R_{k-1,i}, \xi\cdot\xi\right\rangle|^2\right] - \alpha_1 \int_{\Omega}|\nabla_{\Omega}\xi(\omega)|^2d\omega 
\end{equation}

\subsection{Optimization Procedure}
In practice, the maximization defining the greedy update in \eqref{eqn:empirical_greedy_algorithm} is computationally intractable. Instead, we consider maximizing the empirical form of the lower bound given by
\begin{equation}\label{eqn:objective_lower_bound}
    \sup_{\xi\in\mathcal{V}}\mathbb{E}\left[\left|\langle R_{k-1}, \xi\cdot\xi\right\rangle_{L^{2}}|^2\right] \le \mathbb{E}\left[\sup_{\xi\in\mathcal{V}}|\left\langle R_{k-1}, \xi\cdot\xi\right\rangle_{L^{2}}|^2\right].
\end{equation}
Notice that
\begin{equation}\label{eqn:empirical_objective_function}
\begin{aligned}
    \sup_{\xi\in\mathcal{V}}\mathbb{E}_{N}\left[\left\langle R_{k-1}, \xi\cdot\xi\right\rangle_{L^{2}}^2\right] &= \sup_{\xi\in\mathcal{V}}N^{-1}\sum_{i=1}^N\left\langle R_{k-1, i}, \xi\cdot\xi\right\rangle_{L^{2}}^2 \\ 
    &= \sup_{\xi\in\mathcal{V}} N^{-1}\sum_{i=1}^N S_{i,\xi}^2 \\
    &= \sup_{\xi\in\mathcal{V}} N^{-1}\sum_{i=1}^N S_{i,\xi}\left\langle R_{k-1, i}, \xi\cdot\xi\right\rangle_{L^{2}}
\end{aligned}
\end{equation}
In practice, we work with the discretized formulation of the $L^2$ norm and represent the $\xi$
using the truncated basis system $\{\phi_j\}_{j=1}^M$. We see that the corresponding discretized residual for the $i$'th subject is defined as follows:
$$
\boldsymbol{R}_{k,D,i} = \boldsymbol{Y}^{c}_i - \sum_{j=1}^k S_{ij}\left(\boldsymbol{\Phi}\boldsymbol{c}_j\right)\otimes\left(\boldsymbol{\Phi}\boldsymbol{c}_j\right).
$$
\par 
Denote the the singular value decomposition $\boldsymbol{\Phi}_d = \boldsymbol{U}_d\boldsymbol{D}_d\boldsymbol{V}_d^\prime$, define the block matrices 
$$
\boldsymbol{V} = \begin{bmatrix} 
                        \boldsymbol{V}_1 & \boldsymbol{0} \\
                        \boldsymbol{0} & \boldsymbol{V}_2
                \end{bmatrix}, \qquad 
                 \boldsymbol{D} = \begin{bmatrix} 
                        \boldsymbol{D}_1 & \boldsymbol{0} \\
                        \boldsymbol{0} & \boldsymbol{D}_2
                \end{bmatrix}, \qquad \boldsymbol{U} = \begin{bmatrix} 
                        \boldsymbol{U}_1 & \boldsymbol{0} \\
                        \boldsymbol{0} & \boldsymbol{U}_2
                \end{bmatrix},
$$
and define the reparameterization $\tilde{\boldsymbol{c}} = \boldsymbol{D}\boldsymbol{V}^\prime\boldsymbol{c}$.
Using the form from Equation~\eqref{eqn:empirical_objective_function}, we have that 
$$
\begin{aligned}
\left\langle R_{k-1, i}, \xi\cdot\xi\right\rangle_{L^{2}}^2 &\approx (n_1n_2)^{-1}\langle s_{i}(\boldsymbol{c})\boldsymbol{R}_{k-1,D,i}, \left(\boldsymbol{\Phi}\boldsymbol{c}\right)\otimes\left(\boldsymbol{\Phi}\boldsymbol{c}\right)\rangle_{F}\\ 
&= (n_1n_2)^{-1}s_{i}(\tilde{\boldsymbol{c}})\left(\tilde{\boldsymbol{c}}^\prime\boldsymbol{G}_{k-1,i}\tilde{\boldsymbol{c}}\right)  \\
&= (n_1n_2)^{-1}\left(\tilde{\boldsymbol{c}}^\prime s_{i}(\tilde{\boldsymbol{c}})\boldsymbol{G}_{k-1,i}\tilde{\boldsymbol{c}}\right)
\end{aligned}
$$
where $\boldsymbol{G}_{k-1,i} = \boldsymbol{U}^\prime\boldsymbol{R}_{k-1,D,i}\boldsymbol{U}$. It is easy to show that $s_i(\tilde{\boldsymbol{c}}) = \tilde{\boldsymbol{c}}^\prime\boldsymbol{G}_{k-1,i}\tilde{\boldsymbol{c}}$. The reparameterized form of the ob



The discretized empirical objective function can be written as 
$$
\mathcal{O}(\tilde{\boldsymbol{c}}) = (n_1n_2)^{-1}N^{-1}\sum_{i=1}^N\left(\tilde{\boldsymbol{c}}^\prime s_{i}(\tilde{\boldsymbol{c}})\boldsymbol{G}_{k-1,i}\tilde{\boldsymbol{c}}\right)
$$
\par 
To facilitate an efficient solution, we introduce the auxiliary variable $\tilde{\boldsymbol{s}}$ and consider the following optimization equivalent optimization problem

we adopt an alternating optimization (AO) scheme and optimize $\tilde{\boldsymbol{c}}$ and $\boldsymbol{s}$ in blocks. That is, we apply AO to 
$$
\mathcal{O}(\tilde{\boldsymbol{c}}, \boldsymbol{s}) = (n_1n_2)^{-1}N^{-1}\sum_{i=1}^N\left(\tilde{\boldsymbol{c}}^\prime\boldsymbol{s}_{i}\boldsymbol{G}^{(k-1)}_i\tilde{\boldsymbol{c}}\right)
$$


we adopt an alternating optimization (AO) scheme and optimize $\tilde{\boldsymbol{c}}$ and $\boldsymbol{s}$ in blocks. That is, we apply AO to 
The derivation of the block updates can be obtained by simple refactoring of the arguments in the following Section~\ref{ssec:algoImp}.

\section{Algorithm Implementation}\label{ssec:algoImp}

\subsection{Penalty Matrix Computation}

Define  $\psi:\Theta\subset\mathbb{R}^2\rightarrow\mathbb{R}^3$ be a local parameterization around $\boldsymbol{x}\in\mathbb{S}^2$ that is smooth and bijective. The following choice of local parameterization 
$$
    \psi(\theta_1, \theta_2) = (\text{sin}(\theta_1)\text{cos}(\theta_2), \text{sin}(\theta_1)\text{sin}(\theta_2), \text{cos}(\theta_1))^\prime \equiv \boldsymbol{x}^\prime
$$
is valid (invertible) for all points on $\mathbb{S}^2$ except $(0,0,\pm 1)$, i.e. outside of the poles. By definition, the vectors 
$$
    \{\frac{\partial \psi}{\partial\theta_1}(\theta_1,\theta_2), \frac{\partial \psi}{\partial\theta_2}(\theta_1,\theta_2)\}
$$
form a basis for the tangent space $T_{\boldsymbol{x}}(\mathbb{S}^2)$. We may equip $T_{\boldsymbol{x}}(\mathbb{S}^2)$ with an inner product defined by matrix $\boldsymbol{G}\in\mathbb{R}^{2\times 2}$
where 
$$
\langle \boldsymbol{u}, \boldsymbol{v} \rangle_{T_{\omega}(\mathbb{S}^2)} = \boldsymbol{u}^\prime\boldsymbol{G}\boldsymbol{v}
$$
where $\boldsymbol{u},\boldsymbol{v}\in\mathbb{R}^2$ are coordinates w.r.t. to basis vectors of $T_{\omega}(\mathbb{S}^2)$. We let $\boldsymbol{G}$ be the first fundamental form, i.e. the inner product induced by the Euclidean embedding space $\mathbb{R}^3$, that is for $\theta = \psi^{-1}(\omega)$, we have the element-wise definition 
$$
    \boldsymbol{G}_{ij}(\theta) = \langle\frac{\partial \psi}{\partial\theta_i}(\theta_1,\theta_2), \frac{\partial \psi}{\partial\theta_j}(\theta_1,\theta_2)\rangle_{\mathbb{R}^3}.
$$
\par 
We can now define the gradient for $\phi_k:\mathbb{S}^2\rightarrow\mathbb{R}$ 
$$
    \nabla_{\mathbb{S}^2}\phi_k(\boldsymbol{x}) = \sum_{i,j}^2 [\boldsymbol{G}(\boldsymbol{\theta})]^{-1}_{ij}\frac{\partial (\phi_k\circ\psi)}{\partial \theta_j}(\boldsymbol{\theta})\frac{\partial \psi}{\partial \theta_j}(\boldsymbol{\theta}).   
$$
Using basic trigonometric identities it easy to show
$$
\boldsymbol{G}^{-1}(\boldsymbol{\theta}) = \begin{pmatrix}  
            1 & 0 \\
            0 & 1/\text{sin}^2(\theta_1)  
\end{pmatrix}.
$$
The basis vectors are 
$$
   \frac{\partial \psi}{\partial\theta_1}(\theta_1,\theta_2) = (\text{cos}(\theta_1)\text{cos}(\theta_2), \text{cos}(\theta_1)\text{sin}(\theta_2), -\text{sin}(\theta_1))^\prime
$$
and 
$$
    \frac{\partial \psi}{\partial\theta_2}(\theta_1,\theta_2) = (-\text{sin}(\theta_1)\text{sin}(\theta_2), \text{sin}(\theta_1)\text{cos}(\theta_2), 0)^\prime
$$
Finally, we must compute the partial derivative of the basis $\phi_j$ with respect to the local coordinates. We have 
$$
\begin{aligned}
    \frac{\partial \phi_k \circ \psi}{\partial \theta_j}(\theta) &= \sum_{l=1}^3 \frac{\partial\phi_k}{\partial x_l}\frac{\partial x_l}{\partial\theta_j} \\
\end{aligned}
$$
Now, we have already computed $\frac{\partial x_l}{\partial\theta_j}$ and thus we must find  $\frac{\partial\phi_k}{\partial x_l}$ to complete the computation, for which fast algorithms exists \cite{lai2007}. The final form of the penalty matrix is given in the following proposition. 
\begin{proposition}\label{prop:penalty_formulation}
Under the basis expansion in Equation~\eqref{eqn:basis_expansion}, the quadratic variation penalty has the representation 
$$
\text{trace}\left( \begin{pmatrix} \boldsymbol{C}_{1} \\ \boldsymbol{C}_{2}  \end{pmatrix}^\prime \begin{bmatrix} \int_{\mathbb{S}^2}\boldsymbol{F}_{1}\boldsymbol{F}^\prime_{1} & \boldsymbol{0} \\ \boldsymbol{0} & \int_{\mathbb{S}^2}\boldsymbol{F}_{2}\boldsymbol{F}^\prime_{2} \end{bmatrix} \begin{pmatrix} \boldsymbol{C}_{1} \\ \boldsymbol{C}_{2}  \end{pmatrix}\right),
$$
where $\boldsymbol{F}_d(\boldsymbol{x})\in\mathbb{R}^{M_{d}\times 3}$ be the Jacobian of $\boldsymbol{\phi}_{M_{d}}$, 
which is a quadratic function of $\left(\boldsymbol{C}_1, \boldsymbol{C}_2\right)$.
\end{proposition}
\begin{proof}
Since $\Omega = \mathbb{S}_1^2 \cup \mathbb{S}_2^2$, the gradient separates as 
$$
    \nabla_{\Omega}(\xi_k(\boldsymbol{x})) = \nabla_{\mathbb{S}^2}(\boldsymbol{c}^\prime_{1,k}\boldsymbol{\phi}_{M_{1}}(\boldsymbol{x}))\mathbb{I}\{\boldsymbol{x}\in\mathbb{S}_1^2\} + \nabla_{\mathbb{S}^2}(\boldsymbol{c}^\prime_{2,k}\boldsymbol{\phi}_{M_{2}}(\boldsymbol{x}))\mathbb{I}\{\boldsymbol{x}\in\mathbb{S}_2^2\}.
$$
We have 
$$
\begin{aligned}
    \text{Pen}(\xi_k) &=  \sum_{k=1}^K\int_{\Omega}\left[ \boldsymbol{c}^\prime_{1,k}\boldsymbol{F}_{1}(\boldsymbol{x})\boldsymbol{F}^\prime_{1}(\boldsymbol{x})\boldsymbol{c}_{1,k}1\{\boldsymbol{x}\in\mathbb{S}_1^2\} + \boldsymbol{c}^\prime_{2,k}\boldsymbol{F}_{2}(\boldsymbol{x})\boldsymbol{F}^\prime_{2}(\boldsymbol{x})\boldsymbol{c}_{2,k}1\{\boldsymbol{x}\in\mathbb{S}_2^2\}\right] d\boldsymbol{x} \\
    &=  \sum_{k=1}^K\begin{pmatrix} \boldsymbol{c}_{1,k} \\ \boldsymbol{c}_{2,k} \end{pmatrix}^\prime \begin{bmatrix} \int_{\mathbb{S}^2}\boldsymbol{F}_{1}\boldsymbol{F}^\prime_{1} & \boldsymbol{0} \\ \boldsymbol{0} & \int_{\mathbb{S}^2}\boldsymbol{F}_{2}\boldsymbol{F}^\prime_{2} \end{bmatrix} \begin{pmatrix} \boldsymbol{c}_{1,k} \\ \boldsymbol{c}_{2,k} \end{pmatrix} \\ 
    &= \text{trace}\left( \begin{pmatrix} \boldsymbol{C}_{1} \\ \boldsymbol{C}_{2}  \end{pmatrix}^\prime \begin{bmatrix} \int_{\mathbb{S}^2}\boldsymbol{F}_{1}\boldsymbol{F}^\prime_{1} & \boldsymbol{0} \\ \boldsymbol{0} & \int_{\mathbb{S}^2}\boldsymbol{F}_{2}\boldsymbol{F}^\prime_{2} \end{bmatrix} \begin{pmatrix} \boldsymbol{C}_{1} \\ \boldsymbol{C}_{2}  \end{pmatrix}\right)
\end{aligned}
$$
\end{proof}
The required integrals can be computed using Lebedev quadrature rules or using exact rules for the local planar triangle approximation to the spherical triangle. 


\subsection{Derivation of Block Updates}

In this section we derive the forms of the updates for the block coordinate descent algorithm. We begin by proving a couple propositions that we will make repeated used of. First, to facilitate the derivations in this section, we make use of a convenient reparameterization based on the singular value decomposition, given in the following proposition.
\begin{proposition}\label{thrm:coorindate_transformation}
Denote the the singular value decomposition $\boldsymbol{\Phi}_d = \boldsymbol{U}_d\boldsymbol{D}_d\boldsymbol{V}_d^\prime$ and define the block matrices 
$$
\boldsymbol{V} = \begin{bmatrix} 
                        \boldsymbol{V}_1 & \boldsymbol{0} \\
                        \boldsymbol{0} & \boldsymbol{V}_2
                \end{bmatrix}, \qquad 
                 \boldsymbol{D} = \begin{bmatrix} 
                        \boldsymbol{D}_1 & \boldsymbol{0} \\
                        \boldsymbol{0} & \boldsymbol{D}_2
                \end{bmatrix}, \qquad \boldsymbol{U} = \begin{bmatrix} 
                        \boldsymbol{U}_1 & \boldsymbol{0} \\
                        \boldsymbol{0} & \boldsymbol{U}_2
                \end{bmatrix}.
$$
The optimization problem \eqref{eqn:SSSB_empirical_optm} can be equibelently formulated using the transformed parameters $\boldsymbol{\tilde{C}} = \boldsymbol{D}\boldsymbol{V}^\prime \boldsymbol{C}$ as 
\begin{equation}\label{eqn:SSSB_empirical_optm_transformed}
\begin{aligned}
    \widehat{\boldsymbol{\tilde{C}}}, \widehat{\boldsymbol{S}} = \underset{\boldsymbol{\tilde{C}}, \boldsymbol{S}}{\text{argmin}} \quad & \sum_{i=1}^N\left\|\boldsymbol{G}_i - \boldsymbol{\tilde{C}}\boldsymbol{S}_i\boldsymbol{\tilde{C}}^\prime\right\|_{F}^2 + \alpha_1 \text{trace}\left(\boldsymbol{\tilde{C}}^\prime\boldsymbol{\tilde{R}}_{\boldsymbol{\phi}}\boldsymbol{\tilde{C}}\right) \\
    \textrm{s.t} \quad &  \boldsymbol{\tilde{C}}^\prime\boldsymbol{\tilde{J}}_{\phi}\boldsymbol{\tilde{C}} = \boldsymbol{I} \\
    & \left\|\boldsymbol{V}\boldsymbol{D}^{-1}\boldsymbol{\tilde{C}}_{:,k}\right\|_0 \le n_{\alpha_{2}} \text{ for }k=1,...,K
\end{aligned}
\end{equation}
where $$\boldsymbol{G}_i = \boldsymbol{U}^\prime(\boldsymbol{Y}_i -\bar{\boldsymbol{Y}})\boldsymbol{U}, \qquad \boldsymbol{\tilde{J}}_{\boldsymbol{\phi}} = \boldsymbol{D}^{-1}\boldsymbol{V}^\prime\boldsymbol{J}_{\boldsymbol{\phi}}\boldsymbol{V}\boldsymbol{D}^{-1}, \qquad \boldsymbol{\tilde{R}}_{\boldsymbol{\phi}} = \boldsymbol{D}^{-1}\boldsymbol{V}^\prime\boldsymbol{R}_{\boldsymbol{\phi}}\boldsymbol{V}\boldsymbol{D}^{-1}.
$$ 
\end{proposition}
\begin{proof}
The Frobenuis norm is invariant to multiplication by semi-orthogonal matrices. The result follows trivially after noting that $\boldsymbol{U}$ is a semi-orthogonal matrix. 
\end{proof}
The parameter estimate of interest is obtained by transforming the solutions according to $\widehat{\boldsymbol{C}} = \boldsymbol{V}\boldsymbol{D}^{-1}\widehat{\boldsymbol{\tilde{C}}}$.

\begin{proposition}\label{prop:reformulate_objective}
Denote the objective function in \eqref{eqn:SSSB_empirical_optm_relaxed_discrete_rank1}
as 
$$\mathcal{L}(\boldsymbol{c}, \boldsymbol{s}) &:= \left\| \mathcal{Y}^{(k)} - \boldsymbol{\Phi}\boldsymbol{c} \otimes \boldsymbol{\Phi}\boldsymbol{c}\otimes(s \boldsymbol{s}) \right\|_{F}^2 + \alpha_1 \boldsymbol{c}^\prime\boldsymbol{R}_{\boldsymbol{\phi}}\boldsymbol{c},
$$
then 
$$
\begin{aligned}
    \mathcal{L}(\boldsymbol{c}, \boldsymbol{s}) =
\mathcal{L}(\boldsymbol{\tilde{c}}, \boldsymbol{s})  &:= \left\| \mathcal{G}^{(k)} - s \boldsymbol{\tilde{c}} \otimes \boldsymbol{\tilde{c}} \otimes \boldsymbol{s} \right\|_{F}^2 + \alpha_1 \boldsymbol{\tilde{c}}^\prime\boldsymbol{R}_{\xi}\boldsymbol{\tilde{c}} \\
 &= \|\mathcal{G}^{(k)}\|_{F}^2 - 2\boldsymbol{\tilde{c}}^\prime[\mathcal{G}^{(k)}\times_3\boldsymbol{s}]\boldsymbol{\tilde{c}} + \alpha_1\boldsymbol{\tilde{c}}^\prime\boldsymbol{R}_{\xi}\boldsymbol{\tilde{c}} + (\boldsymbol{\tilde{c}}^\prime\boldsymbol{\tilde{c}})^2
\end{aligned}
$$
\end{proposition}
\begin{proof}
    This follows directly for the reparameterization established in Proposition~\ref{eqn:SSSB_empirical_optm_transformed} along with simple algebra.
\end{proof}



\subsubsection{$\boldsymbol{\tilde{c}}$ Subproblem}

Parameterize $\boldsymbol{\tilde{c}} = c\boldsymbol{v}$, where $c\in\mathbb{R}$ and $\boldsymbol{v}$ is a unit vector. Then using proposition \ref{prop:reformulate_objective}, we can re-parmeterize the loss function as 
$$
\begin{aligned}
        \mathcal{L}(c, \boldsymbol{v}) &= \|\mathcal{G}^{(k)}\|_{F}^2 - 2\boldsymbol{v}^\prime[\mathcal{G}^{(k)}\times_3\boldsymbol{s}]\boldsymbol{v} + \alpha c^2 \boldsymbol{v}^\prime\boldsymbol{R}\boldsymbol{v} + c^4 \\
        &=  \|\mathcal{G}^{(k)}\|_{F}^2 - c^2\boldsymbol{v}^\prime[2\mathcal{G}^{(k)}\times_3\boldsymbol{s} - \alpha\boldsymbol{R}]\boldsymbol{v} + c^4 
\end{aligned}
$$
Now, the fist order gradient conditions of $\mathcal{L}$ with respect to c implies that 
$$
     c^2 = \frac{1}{2}\boldsymbol{v}^\prime[2\mathcal{G}^{(k)}\times_3\boldsymbol{s} - \alpha\boldsymbol{R}]\boldsymbol{v}
$$
or $c=0$. Plugging this back into $\mathcal{L}$, we obtain 
$$
    \begin{aligned}
        \mathcal{L}(\boldsymbol{v}) &=  \|\mathcal{G}^{(k)}\|_{F}^2 - (\frac{1}{2}\boldsymbol{v}^\prime[2\mathcal{G}^{(k)}\times_3\boldsymbol{s} - \alpha\boldsymbol{R}]\boldsymbol{v})(\boldsymbol{v}^\prime[2\mathcal{G}^{(k)}\times_3\boldsymbol{s} - \alpha\boldsymbol{R}]\boldsymbol{v}) + (\frac{1}{2}\boldsymbol{v}^\prime[2\mathcal{G}^{(k)}\times_3\boldsymbol{s} - \alpha\boldsymbol{R}]\boldsymbol{v})^2 \\
        &=  \|\mathcal{G}^{(k)}\|_{F}^2 - \frac{1}{4}(\boldsymbol{v}^\prime[2\mathcal{G}^{(k)}\times_3\boldsymbol{s} - \alpha\boldsymbol{R}]\boldsymbol{v})^2
\end{aligned}
$$
Clearly, the loss is minimized when 
\begin{equation}\label{eqn:max_eigenvalue_subproblem}
    \boldsymbol{v}^\prime[2\mathcal{G}^{(k)}\times_3\boldsymbol{s} - \alpha\boldsymbol{R}]\boldsymbol{v}
\end{equation}
is maximized, which occurs when $\boldsymbol{v}$ is the eigenvector associated with the largest positive eigenvalue. 
\par 
We now incorporate the constraints. The following proposition characterizes the space of allowable solutions under the orthogonality constraint.
\begin{proposition}\label{prop:orthogonal_constraint}
Let $\boldsymbol{\tilde{C}}_{k-1} = [\boldsymbol{\tilde{c}}_1, ..., \boldsymbol{\tilde{c}}_{k-1}]$. Then the orthogonality constraint $\boldsymbol{\tilde{c}}^\prime\boldsymbol{\tilde{J}}_{\boldsymbol{\phi}}\boldsymbol{\tilde{c}_j} = 0\text{ for }j=1,...,k-1$ is equivalent the condition that 
$$
    (\boldsymbol{I} - \boldsymbol{\tilde{P}}_{k-1})\boldsymbol{\tilde{c}} = \boldsymbol{\tilde{c}}
$$
where 
$$
    \boldsymbol{\tilde{P}}_{k-1} = \boldsymbol{\tilde{C}}_{k-1}[\boldsymbol{\tilde{C}}_{k-1}^\prime\boldsymbol{\tilde{J}}_{\boldsymbol{\phi}}\boldsymbol{\tilde{C}}_{k-1}]^{-1}\boldsymbol{\tilde{C}}_{k-1}^\prime\boldsymbol{\tilde{J}}_{\boldsymbol{\phi}}
$$
\end{proposition}
\begin{proof}
Note that the matrix $\boldsymbol{\tilde{J}}$ is symmetric and positive definite and therefore defines an inner product on $\mathbb{R}^{M_{1}+M_{2}}$. The result then follows trivially from standard results in linear algebra. 
\end{proof}
Proposition~\ref{prop:orthogonal_constraint} allows us to incorporate the orthogonality constraint directly into the objective, i.e. the update of $\boldsymbol{\tilde{c}}$ solves.
$$
\begin{aligned}
    \text{max} &\quad \boldsymbol{\tilde{c}}^\prime(\boldsymbol{I} - \boldsymbol{\tilde{P}}_{k-1})[2\mathcal{G}^{(k)}\times_3\boldsymbol{s} - \alpha\boldsymbol{R}](\boldsymbol{I} - \boldsymbol{\tilde{P}}_{k-1}^\prime)\boldsymbol{\tilde{c}} \\
    & \textrm{s.t.} \quad \left\|\boldsymbol{V}\boldsymbol{D}^{-1} \boldsymbol{\tilde{c}}\right\|_{\boldsymbol{J}_{\boldsymbol{\phi}}} = 1, \quad  \left\|\boldsymbol{V}\boldsymbol{D}^{-1} \boldsymbol{\tilde{c}}\right\|_{0} \le n_{\alpha_{2}}
\end{aligned}
$$
We now transform the problem back to the original coordinate space using the inverse transfom $\boldsymbol{c} = \boldsymbol{V}\boldsymbol{D}^{-1}\boldsymbol{\tilde{c}}$, resulting in 
$$
\begin{aligned}
    \text{max} &\quad \boldsymbol{c}^\prime\boldsymbol{V}\boldsymbol{D}(\boldsymbol{I} - \boldsymbol{\tilde{P}}_{k-1})[2\mathcal{G}^{(k)}\times_3\boldsymbol{s} - \alpha\boldsymbol{R}](\boldsymbol{I} - \boldsymbol{\tilde{P}}_{k-1})\boldsymbol{D}\boldsymbol{V}^\prime\boldsymbol{c} \\
    & \textrm{s.t.} \quad \left\|\boldsymbol{c}\right\|_{\boldsymbol{J}_{\boldsymbol{\phi}}} = 1, \quad \left\|\boldsymbol{c}\right\|_{0} \le n_{\alpha_{2}}. \\
\end{aligned}
$$
Using the definition of $\tilde{\boldsymbol{c}}$, it is easy to see that $\boldsymbol{\tilde{P}}_{k-1} = \boldsymbol{P}_{k-1}$ as defined by \eqref{eqn:update_P}.
\subsubsection{$\boldsymbol{s}$ Subproblem}

Considering proposition \eqref{prop:reformulate_objective}, notice that we can re-write the component of the objective function that depends on $\boldsymbol{s}$ as 
$$
\begin{aligned}
    \mathcal{G}^{(k)}\times_1 \boldsymbol{\tilde{c}}
      \times_2 \boldsymbol{\tilde{c}} \times_3 \boldsymbol{s} &= (\mathcal{G}^{(k)} \times_1 \boldsymbol{\tilde{c}}
      \times_2 \boldsymbol{\tilde{c}}) \times_3 \boldsymbol{s} \\
      &= \boldsymbol{s}^\prime \boldsymbol{g}_{\boldsymbol{\tilde{c}}}; \qquad  \boldsymbol{g}_{\boldsymbol{\tilde{c}}} := \mathcal{G}^{(k)} \times_1 \boldsymbol{\tilde{c}}
      \times_2 \boldsymbol{\tilde{c}} \in\mathbb{R}^{N}
\end{aligned}
$$
and therefore the block update for $\boldsymbol{s}$ is given by the solution to 
\begin{equation}\label{eqn:conditional_optim_s}
    \boldsymbol{s}^{*} = \max_{\boldsymbol{s}^\prime\boldsymbol{s}=1} \boldsymbol{s}^\prime\boldsymbol{g}_{\boldsymbol{\tilde{c}}}
\end{equation}
It is easy to show that $\boldsymbol{g}_{\boldsymbol{\tilde{c}}}\ge 0$ and hence \eqref{eqn:conditional_optim_s} has the analytic solution $\boldsymbol{s}^{*} = \boldsymbol{g}_{\boldsymbol{\tilde{c}}}/\|\boldsymbol{g}_{\boldsymbol{\tilde{c}}}\|_2$, which results from the Cauchy-Schwartz inequality.


==> manuscript_v2.tex <==
\section{Introduction}\label{sec:introduction}
Brain connectivity is an important phenotype for understanding how the brain works in dealing with everyday challenges and in the context of mental disorder and neurodegenerative disease \citep{fornito2013, park2013}. There are distinct notions of brain connectivity (or network) obtained from different brain imaging modalities. For instance, \textit{functional connectivity} (FC) is obtained from functional magnetic resonance imaging (fMRI) and determines a network using pairwise correlation measures in the BOLD signal. \textit{Structural connectivity} (SC) aims to measure the strength of connectivity between regions based on the white matter (WM) fiber tracts reconstructed from diffusion MRI (dMRI), the collection of which is referred to as the \textit{structural connectome}. In this work, we focus on the latter. The most common approach for analyzing connectivity data is to represent it as a symmetric adjacency matrix, denoted $\boldsymbol{A} \in \mathbb{R}^{V \times V}$,  where $V$ is the number of regions of interest (ROIs) on the brain surface and the element $\boldsymbol{A}_{ab}$ quantifies the strength of connectivity between ROIs $a$ and $b$. To obtain $\boldsymbol{A}$, the brain surface is discretized into $V$ disjoint regions using some predefined parcellation, referred to as a brain atlas (see e.g., \cite{desikan2006} and \cite{destrieux2010}). There is a great interest in understanding the variability of these networks \citep{durante2017nonparametric,wang2019} and relating this variability to human traits such as cognition and personality \citep{zhang2019,arroyo2021,arroyo2021b}. For an overview on the current state of representation and statistical analysis of connectome matrices, see \cite{chung2021}.
\par 
The reliance on the pre-specification of an atlas in the discrete ROI-based analysis framework is problematic for at least two major reasons. First, there is no consensus as to which atlas is best for brain connectivity analysis, and therefore the selection for a given application is somewhat \textit{ad-hoc}. Analyses can be sensitive to the choice of atlas \citep{zalesky2010}, resulting in different conclusions for different parcellation schemes of the same data. Second, this approach can introduce information loss, since fine-grained connectivity information on the sub-ROI level is aggregated in the construction of the adjacency matrix. Recent studies indicate that connectivity information at high resolutions is predictive for many behavioral traits of interest \citep{mansour2021}. One way to mitigate these drawbacks is to increase the number of ROIs in the parcellation. This trend can be observed in more recent atlases, e.g., \cite{power2011functional} use an atlas containing $264$ nodes, and \cite{glasser2016multi} build an atlas of $360$ regions for the cortical surfaces. However, increasing the number of ROIs introduces additional challenges in data analysis. The dimension of the network grows on the order of $V^2$, rendering statistical modeling and inference very challenging for even moderately large $V$. 
%Moreover, alignment of smaller ROIs between subjects is difficult. When the alignment is poor, unwanted variance among the connections is introduced due to misalignment as opposed to the biological heterogeneity in which we are interested in.
\par 
Our work addresses these problems by transitioning from the discrete, ROI based representation of brain connectivity to a fully continuous model. Specifically, let $S_1$ and $S_2$ denote the left and right white surfaces of the brain. The white surface, denoted as $S_1\cup S_2$, refers to the interface between the cortical grey matter and white matter regions. Figure~\ref{fig:t1_and_surface} shows an image of the structural connectome of a randomly selected Human Connectome Project (HCP) \citep{glasser2013} subject embedded within the white surface of the brain. The endpoints of the WM streamlines (colored curves) are points on $\left(S_1\cup S_2\right)\times\left(S_1\cup S_2\right)$. We assume the spatial pattern of these points is related to an unobserved continuous function on $\left(S_1\cup S_2\right)\times\left(S_1\cup S_2\right)$, which governs the strength of connectivity between any pair of points on $S_1\cup S_2$. This unobserved intensity function is referred to as the continuous (structural) connectivity, a concept first explored in \cite{moyer2017}. 
%Since each of $S_1$ and $S_2$ are homeomorphic to an independent copy of  $\mathbb{S}^2$, we can use the product 2-sphere as a domain for modeling the continuous connectivity and leverage its nice properties to simplify computations.
\par 
Crucially, the continuous model of connectivity does not depend on the pre-specification of an atlas and therefore avoids the previously outlined issues which plague traditional discrete network-based approaches. Moreover, the continuous framework inherently captures both high and low frequency variations in the data, thus facilitating a flexible representation of the connectivity. The top left image in Figure~\ref{fig:connectome_representations} shows the continuous connectivity of a randomly selected HCP subject evaluated over all pairs of points in a dense grid on $S_1\cup S_2$. Compared to the corresponding discrete atlas-based connectivity matrix shown in the top right of Figure~\ref{fig:connectome_representations}, the continuous representation is both smoother and able to represent more complex patterns in the connectome. For any point or region on $S_1\cup S_2$, the continuous connectivity can be marginalized to obtain the strength of connectivity with all other points on the surface, as shown in the bottom panel of Figure~\ref{fig:connectome_representations}.
\par 
Despite the outlined advantages, the continuous approach also presents some additional challenges compared to atlas-based methods. Atlas-based connectivity matrices can be easily constructed using simple statistics computed on the WM streamlines connecting pairs of ROIs. In comparison, estimating a continuous model of connectivity from the sample of streamlines is non trivial. The approach developed by \cite{moyer2017}, and utilized in \cite{cole2021}, proposes a point-wise estimator via a kernel smoothing technique. A high-resolution mesh grid on $S_1\cup S_2$ is defined and the continuous connectivity is then represented using a symmetric matrix, where each element of the matrix is the smoother applied to a pair of points in the grid. Unfortunately, for even moderately large grids, this generates enormous matrices and therefore results in major computational hurdles for anything beyond simple subject-level analysis.
\par 
In this work, we extend the current frameworks for continuous connectomics \citep{gutman2014,moyer2017,cole2021,mansour2022} by considering the per-subject continuous connectivity as a realization of a latent random intensity function which governs observed WM streamline endpoints through a doubly stochastic point process model. As a result, the continuous connectome matrices can be considered as a sample of functional data. Existing functional data analysis (FDA) approaches to point-process modeling have mainly been concerned with the 1-D case \citep{bouzas2006,muller2013,panaretos2016,wrobel2019}. These approaches involve estimating the eigenvalues and eigenfunctions of the covariance function of the latent intensity process using functional principal components analysis (FPCA). In our case, the covariance function is a functional object on an 8-dimensional manifold domain and therefore typical methods for FPCA, and by extension the aforementioned approaches, are not feasible for our problem due to the curse of dimensionality. The literature on methods for multidimensional replicated point processes is relatively sparse, though some have recently been developed under the framework of a doubly stochastic Poisson process model. \cite{gervini2019} uses penalized likelihood estimation and basis expansion to estimate spatiotemporal intensity functions on $\mathbb{R}\times\mathbb{R}^2$ under time-space separability, while \cite{john2018} introduce a Gaussian process assumption on the latent intensity function and develop a scalable variational Bayesian approach for estimation and inference. In our set-up, the symmetry of the intensity function and the exotic product manifold domain render these likelihood-based approaches computationally prohibitive, mainly due to the presence of a normalization term which requires repeated integration over $\left(S_1\cup S_2\right)\times\left(S_1\cup S_2\right)$.
\par 
Due to these issues, we propose a novel methodology to construct a data-adaptive reduced-rank function space for continuous connectivity representation and analysis that avoids the curse of dimensionality while simultaneously possessing a universal approximation property with a favorable convergence rate. To estimate a basis for this space, we derive a novel estimation algorithm, the dimension of which is user controlled and can typically be made much smaller than the raw connectivity data. Our framework also allows for the incorporation of penalties to both promote smoothness and local support of the solutions. We apply the proposed method to a subset of HCP subjects and show that it outperforms traditional atlas-based approaches on several prediction and hypothesis testing tasks of interest. We also demonstrate the application of our method for detecting local connectivity differences between groups, equivalent to the significant sub-network detection problem in the literature \citep{wang2021classification,wang2021learning}, extended to the infinite dimensional case.
\par 
This paper is an extension of a brief conference paper \citep{Consagra2022}, in which we include several key additions. Discussion of the methodological framework, including the construction of the reduced-rank representation space, procedure for statistical inference for a sample of continuous connectivity objects and the derivation of the novel estimation algorithm are all extended considerably. Furthermore, the experimental evaluation is far more comprehensive, including additional real data analysis demonstrating the superiority of our method over several state-of-the-art competitors, as well as a simulation study investigating convergence and computational complexity.
%\par 
%The remainder of this paper is organized as follows. Descriptions of the datasets and the SC estimation pipeline are provided in Section~\ref{sec:data}. Section~\ref{sec:statistical_framework} provides an explicit statistical model for the observed connectivity data. Section~\ref{sec:reduced_rank_model} proposes a framework for constructing reduced-rank representations of the continuous connectivity and shows how to utilize these representations to facilitate statistical tasks of interest.  Relevant theoretical properties are also discussed. Our novel estimation algorithm is presented in Section~\ref{sec:methods} and it's performance is evaluated on simulated data in Section~\ref{sec:simulation}. Section~\ref{sec:real_data_experiments} presents several real data analyses using HCP data and concluding remarks are given in Section~\ref{sec:conclusion}.

\begin{figure}[t]
    \centering
     \includegraphics[scale=0.5]{Figures/S1_S2_andT1w_3tile.pdf}
    \caption{(A) 3D view of the cortical white surface extracted from the T1 image and the structural connectome of a randomly selected HCP subject. (B) Local surface magnification showing white matter streamlines (colored curves) ending on the surface. (C) The endpoint distribution of streamlines from the region in (B).}
    \label{fig:t1_and_surface}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.6]{Figures/continuous_vs_discrete_connectivity_update-1.pdf}
    \caption{The top left image shows the continuous connectivity of a randomly selected HCP subject evaluated over each pair of points in a dense grid on $S_1\cup S_2$. The top right image shows the corresponding discrete connectivity matrix, under the Desikan brain atlas. The bottom panel shows the mean marginal continuous connectivity in the indicated region on the left cortical surface.}
    \label{fig:connectome_representations}
\end{figure}

\section{Structural Connectivity Data}\label{sec:data}

\subsection{Human Connectome Project}
In this work, we consider a sample of 437 female subjects from the HCP young adult cohort (\textit{https://db.humanconnectome.org}). In addition to multimodal imaging data, associated with each subject are a set of measurements related to various cognitive, physical, socioeconomic and psychiatric factors, or \textit{traits}. Many of these traits are defined and measured using tests from the NIH Toolbox for Assessment of Neurological and Behavioral Function \citep{gershon2013}, though some additional tests for measuring cognitive and emotional processing were also performed.  To understand the association between brain structural connectivity and human traits, we collected 175 traits spanning eight categories: cognition, motor, substance use, psychiatry, sense, emotion, personality and health. We also utilized the HCP test-retest data in our analysis. This data consists of a subset of HCP subjects for whom two scans were collected during different sessions several months apart. This dataset contains 37 subjects and a total of 74 scans.  
\subsection{Data Description, Image Acquisition and Processing}
Diffusion MRI measures the local anisotropy of water molecule diffusion to infer white matter microstructure. In particular, the local geometry of the white matter induces an anisotropy in the local water molecule diffusion, in which water tends to diffuse faster along the direction of the underlying neural fiber tracts. Diffusion MRI exploits this relationship and collects measurements of spatially localized diffusion signals along many different directions, called b-vectors, to obtain a 3-dimensional picture of diffusion through each location (voxel) on a regular grid over the brain volume. Smooth local models of diffusion are fit to these measurements, e.g. the diffusion tensor \citep{Basser_diffusion} or the orientation distribution function (ODF) \citep{tuch_2004}, and are subsequently used to trace out the large-scale white matter fibers using a process called tractography \citep{basser2000}.
\par 
For each subject, we use both the dMRI and the structural T1-weighted images. The T1 provides images with high contrast between WM and GM regions and is therefore useful for estimating the white surface. The full imaging acquisition protocol as well as the minimal preprocessing pipeline applied to the dMRI data are given in \cite{glasser2013}, which includes susceptibility induced distortion correction and motion correction using FSL \citep{smith2004}. The diffusion images were collected at 1.25 mm isotropic resolution on a 3T Siemens Connectom scanner (Erlangen, Germany). The diffusion imaging was done using a 2D spin-echo echo-planar imaging sequence with a total of 270 diffusion directions, each acquired once with both right-to-left and left-to-right phase encoding polarities, on three shells with three b-values 1,000, 2,000, and 3,000 s/mm$^{2}$. In addition, a total of 18 non-diffusion weighted images were also obtained.  The T1 images were acquired with the 3D magnetization prepared rapid gradient echo sequence with a slice acceleration factor of 2 using 0.7 mm isotropic resolution. The T1 images were registered to the dMRI using volumetric registration in ANTs \citep{avants2009advanced}. The cortical white surfaces $S_1$ (left) and $S_2$ (right) were extracted using Freesurfer and their geometry represented using a surface triangulation with $\approx 64,000$ vertices.
\par 
To estimate the SC, we first estimate the local models of diffusion from the data using the approach from \cite{tournier2007} and then apply the surface enhanced tractography (SET) algorithm \citep{st2018surface} to estimate the underlying white matter fiber tracts connecting different brain regions. The output of the tractography contains millions of streamlines in the form of 3D curves. An important feature of SET is that it ensures the ending points of streamlines are on $S_1\cup S_2$, facilitating our modeling of the SC as a point pattern on the cortical surface. 
\par 
For the joint analysis of imaging data from multiple subjects, an additional source of unwanted variability comes from misalignment due to different shapes and sizes of the brain.  Failure to account for misalignment can lead to an artificial inflation in the variability of the inferred connectivity pattern. To alleviate this issue, we parameterize each of the white surfaces using spherical coordinates via the surface inflation techniques from \cite{fischl1999}, and then apply a warping function estimated from geometric features on the surface using Freesurfer to bring the WM streamline endpoints to a common template space.
\par 
The final surface endpoint connectivity data consists of counts of connections between $\approx 64,000^2$ pairs of points. Conventional array-based representations require $ > 16$Gb  storage space per subject. To alleviate the disk space burden, we downsampled the registered surfaces to a resolution of 4,121 vertices using a procedure which minimizes the local metric distortion. More details about the surface alignment in Freesurfer and downsampling technique can be found in \cite{fischl1999high} and \cite{cole2021}.

\section{Statistical Framework for Continuous Connectivity}\label{sec:statistical_framework}
\subsection{Modeling Continuous Connectivity using Doubly Stochastic Point Processes}\label{ssec:statistical_model}
For a single subject, let $\tilde{O}=\{ (\tilde{ p}^1_1,\tilde{ p}^1_2), \cdots, (\tilde{ p}^q_{1},\tilde{ p}^q_2) \}$ denote the endpoints of $q$ streamlines connecting cortical white surfaces $\Omega = S_1 \cup S_2$ (see Figure~\ref{fig:t1_and_surface}). Since $S_i$ ($i\in \{1,2\}$) is homeomorphic to $\mathbb{S}^2$, we parameterize it using spherical coordinates.  Let $({ p}_1,{ p}_2)$ be the image of $(\tilde{ p}_1,\tilde{ p}_2)$ on $\mathbb{S}^2_1 \cup \mathbb{S}^2_2$ under the homeomorphism; we define  ${O}=\{ ({p}^1_1,{ p}^1_2), \cdots, ({ p}^q_{1},{ p}^q_2) \}$, and with some abuse of notation we let $\Omega= \mathbb{S}^2_1 \cup \mathbb{S}^2_2$, and hence $O \subset \Omega \times \Omega$. For a single subject, we can model the streamline endpoints $O$ as a realization of an underlying point process on $\Omega \times \Omega$ with an unknown integrable intensity function $u: \Omega \times \Omega \mapsto [0,\infty)$ defined as follows. For any two measurable regions $E_1 \subset \Omega$ and $E_2 \subset \Omega$, denote $\#(E_1,E_2)$ as the counting process of the number of streamlines ending in $(E_1,E_2)$. Then $u$ satisfies
\begin{equation}\label{eqn:first_moment_assumption}
    \mathbb{E}\left[\#(E_1,E_2)\right]=\int_{E_1} \int_{E_2} u(\omega_1,\omega_2)d\omega_1d\omega_2 < \infty
\end{equation}
\par 
In this work, we are interested in the analysis of a random sample of the structural connectivity data from $N$ subjects: $O_1,...,O_N$. Modeling the replicated point processes with a single deterministic intensity function is likely insufficient to properly accommodate the population variability in connectivity patterns. It is reasonable to assume that the intensity function governing $O$ is itself a realization of an underlying random process, which we denote as $U$. That is, conditional on $U_i\sim U$, the first order moment of the point set $O_i$ satisfies Equation~\eqref{eqn:first_moment_assumption} with intensity function $U_i$. 
%Hence, the object of interest is not a single unknown deterministic function, but rather a distribution over functions.
\par 
Denote $\mathcal{H}$ as the space of symmetric $L^2$ functions over $\Omega\times\Omega$, i.e., for $u \in \mathcal{H}$, $u(\omega_1,\omega_2) = u(\omega_2,\omega_1)$ and $\int_\Omega\int_\Omega u^2(\omega_1,\omega_2)d\omega_1d\omega_2<\infty$. We assume that $U$ has an associated measure $\mathbb{P}$ such that i) the mean function $\mathbb{E}_{\mathbb{P}}[U] = \mu\in \mathcal{H}$, ii) the process has finite second order moment $\mathbb{E}_{\mathbb{P}}[\|U\|_{L^{2}(\Omega\times\Omega)}^2]<\infty$, iii) the covariance function $C\left( (\omega_1,\omega_2), (\omega_1^{\prime},\omega_2^{\prime}) \right) := \text{Cov}\{U(\omega_1,\omega_2),U(\omega_1^{\prime},\omega_2^{\prime})\}$ is mean-square integrable and iv) $U$ is integrable almost surely. Under these conditions, $U$ is associated with a random density function, denoted $F_U(\omega_1, \omega_2) = U(\omega_1, \omega_2)/\int_{\Omega\times\Omega}U$. Define $Q$ as a distribution on $\mathbb{N}$ with finite moments modeling the total number of streamlines. $Q$ is related to the seeding procedure in fiber tracking \citep{girard2014towards,ambrosen2020validation}: in this study, we seeded 3 million points for each subject, and the resulting sample mean of the $q_i\sim Q$ was $\approx 1$ million. Conditional on $U_i$ and $q_i$, we assume that the $i$'th subject's observed streamline endpoints $O_i\overset{i.i.d.}{\sim} F_{U_{i}}$ and that $Q$ and $F_{U}$ are independent. Statistical models with similar independence assumptions have previously been made in context of functional data analysis for replicated point processes in 1-D \citep{muller2013}.

%We assume the following generative model for the structural connectivity of the $i$th-subject:
%\begin{equation}\label{eqn:generative_model}
%    \begin{aligned}
%    &U_i \sim U, \quad q_i \sim Q, \quad Q\indep F_{U} \\
%    & O_i | U_i,q_i \overset{i.i.d.}{\sim} F_{U_{i}}
%    \end{aligned}
%\end{equation}
%where $Q$ is a distribution on $\mathbb{N}$ with finite moments describing the distribution of the total number of streamlines and is related to the seeding procedure in fiber tracking \citep{girard2014towards,ambrosen2020validation}. In this study, we seeded 3 million points for each subject, and obtained $q_i$ with a mean of $\sim 1$ million. The model assumption $Q \indep F_{U}$ can be understood as an independence between the ``scale'' and ``shape'' of the structural connectivity pattern. This assumption has previously been made in context of functional data analysis for replicated point processes in 1-D \citep{muller2013, panaretos2016}.


\subsection{Subject-Level Estimate of Continuous Connectivity}
Under the model described in Section~\ref{ssec:statistical_model}, conditional on $O_i$, we can form $\widehat{F_{U_{i}}}$, and hence $\widehat{U}_i$, using kernel density estimation. Specifically, let $H_{h}:\Omega\times\Omega\mapsto \mathbb{R}^{+} \cup \{0\}$ be the kernel function with bandwidth $h > 0$ defined by $H_h((\omega_1,\omega_2)|(p_1,p_2)) = \kappa_h(\omega_1, p_1)\kappa_h(\omega_2, p_2)$, where $\kappa_h$ is the spherical heat kernel \citep{chung2006} trivially extended to $\Omega$ by setting $\kappa_h(\omega_1,p_1) = 0$ if $\omega_1$ and $p_1$ are not on the same copy of $\mathbb{S}^2$. A point-wise estimate of $F_{U_i}$ and $U_i$ for the $i$-th subject is given by:
\begin{equation}\label{eqn:KDE_cc}
    \widehat{F_{U_{i}}}(\omega_1,\omega_2) = \sum_{j=1}^{q_i} H_{h}((\omega_1,\omega_2)|(p^{j}_{i1}, p^{j}_{i2}))/q_i, \quad \widehat{U_i} = q_i 
    \widehat{F}_i(\omega_1,\omega_2)
\end{equation}
%Using the assumption of shape-scale independence, $U_i$ will be (asymptotically) unbiased as long as the kernel estimator ${F_{U_{i}}}$ in~\eqref{eqn:KDE_cc} is (asymptotically) unbiased. 
Given the number of streamlines we considered, i.e. $q_i$ is on the order of $10^6$, we can be confident in these point-wise estimates. Note, this estimator was first proposed in \cite{moyer2017} for the rate parameter of an inhomogenous Poisson process model for a single continuous connectome. Automated selection of the bandwidth $h$ can be performed using the cross-validation procedure described in the same reference. 

\section{Reduced-Rank Modeling of Continuous Connectivity}\label{sec:reduced_rank_model}
In Section~\ref{sec:statistical_framework}, we describe a statistical model linking the streamline endpoints with the underlying continuous connectivity and provide a subject-level point-wise estimate for this latent quantity using the observed data. In this section, we propose a framework to construct efficient representations of a sample of continuous connectivity objects using a novel data-driven reduced-rank modeling approach and then illustrate how this representation facilitates downstream statistical analyses such as prediction and hypothesis testing. Proofs of all the results in this section are provided in the Supplemental Materials.
%The local estimator  \eqref{eqn:KDE_cc} is infinite dimensional and therefore requires some simplification for efficient computation. Previous approaches have applied discretization techniques to study the continuous connectivity using extremely high-dimensional matrix representations \citep{moyer2017,cole2021,mansour2022}. This approach prohibits anything beyond simple joint analysis due to computational limitations in the storage and processing of the enormous connectivity matrices. In this section, we propose a framework to construct efficient representations of a sample of continuous connectivity objects using a novel data-driven reduced-rank modeling approach and then illustrate how this representation facilitates downstream statistical analyses such as prediction and hypothesis testing. Proofs of all the results in this section are provided in the Supplemental Materials.
%The section is organized as follows. In \ref{ssec:fpca}, we present the traditional approach to low-rank modeling for functional data and discuss its infeasibility in our situation due to the curse of dimensionality. In \ref{ssec:reduced_rank_model}, we develop our alternative reduced-rank approach and establish relevant theoretical properties. In \ref{ssec:inference}, we demonstrate how to use the proposed models to facilitate efficient downstream statistical analysis.  Proofs of all the results in this section are provided in the Supplemental Materials.

\subsection{Functional Principal Components Analysis}\label{ssec:fpca}
Optimal reduced-rank modeling for functional data has largely focused on the eigenfunctions of the covariance function $C$. Under the mean-square integrability assumption on $C$, Mercer's theorem guarantees the existence of a set of non-negative eigenvalues $\{\rho_k\}$ and associated orthonormal eigenfunctions $\{\psi_k\}$ such that 
$
C\left( (\omega_1,\omega_2), (\omega_1^{\prime},\omega_2^{\prime}) \right) = \overset{\infty}{\underset{k=1}{\sum}}\rho_k \psi_k(\omega_1,\omega_2)\psi_k(\omega_1^{\prime},\omega_2^{\prime}).
$
 By the Karhunen-Lo\`{e}ve theorem, the random function can be represented as
$
U(\omega_1, \omega_2) = \mu(\omega_1,\omega_2) + \sum_{k=1}^\infty Z_k\psi_k(\omega_1, \omega_2),
$ where $Z_k = \langle U - \mu, \psi_k\rangle_{L^2(\Omega\times\Omega)}$ are independent, mean zero random variables with $\mathbb{E}_{\mathbb{P}}[Z_k^2] = \rho_k$. 
\par 
The first $K$ $\psi_k$'s form an optimal (according to the mean integrated squared error) rank $K$ basis for representing realizations of $U$. This makes them very appealing for forming parsimonious finite rank approximations. Of course, the eigenfunctions are unknown and must be estimated from the data, i.e., by FPCA \citep{ramsay2005}. A common approach is to form a smoothed estimate $\widehat{C}$ and then perform a spectral decomposition over some finite dimensional basis system or discretization of the domain \citep{silverman1996,yao2005}. However, this approach is infeasible in the current situation due to the curse of dimensionality, as $C$ is a symmetric positive semi-definite (PSD) function defined over an $8$-D manifold domain, i.e., $(\Omega \times \Omega) \times (\Omega \times \Omega)$.
\par 
Approaches to FPCA for data on complicated non-Euclidean multidimensional domains are limited. \cite{lila2016} use finite elements to solve the best rank $K$ optimization problem, while \cite{muller2017} and \cite{lynch2018} assume a separable structure on $C$ to promote tractable estimation of the marginal eigenfunctions. The former still requires solving an optimization problem over $\mathcal{H}$, the space of symmetric functions on the product space of two 2-D submanifolds of $\mathbb{R}^3$, hence the curse of dimensionality is still problematic. The latter introduces assumptions that are hard to verify in practice, and can be inefficient when the true covariance is not separable \citep{consagra2021}. Instead, we propose an alternative data-driven procedure to create a reduced-rank function space, adapted to the distribution of $U$, that is both highly flexible and avoids the curse of dimensionality. 

\subsection{Data-Driven Reduced-Rank Function Spaces}\label{ssec:reduced_rank_model}
We begin with defining relevant notation. Without loss of generality, assume that $U$ has been centered, i.e., we consider the zero-mean process $\mathbb{E}_{\mathbb{P}}[U]=0$. Denote the set of unit $L^2(\Omega)$-norm functions, called the Hilbert sphere, $\mathbb{S}^{\infty}(\Omega) :=  \{\xi \in L^2(\Omega) : \left\| \xi \right\|_{L^{2}(\Omega)} = 1\}$.  Define the symmetric separable orthogonal function set of rank $K$ as
$$
\mathcal{V}_{K} = \{\xi_k\otimes\xi_k: \xi_k \in \mathbb{S}^{\infty}(\Omega), \langle \xi_k, \xi_j\rangle_{L^{2}(\Omega)} = \delta_{kj},\text{ for }k = 1,2,...,K\},
$$
where $\xi\otimes\xi(\omega_1,\omega_2) := \xi(\omega_1)\xi(\omega_2)$ and $\delta_{ik}$ is the Kronecker delta. 
\par 
For any $K$, there are an infinite number of such sets. We propose to construct a $\mathcal{V}_{K}$ adapted to the distribution of $U$ utilizing a greedy learning procedure. Specifically, given a sample of $N$ independent realizations of $U_i \sim U$, we iteratively construct $\mathcal{V}_K$ by repeating the following steps: 
\begin{equation}\label{eqn:empirical_greedy_algorithm}
\begin{aligned}
        \xi_k &= \sup_{\xi\in\mathbb{S}^{\infty}(\Omega)}N^{-1}\sum_{i=1}^N\left[|\left\langle R_{k-1,i}, \xi\otimes\xi\right\rangle_{L^2(\Omega\times\Omega)}|^2\right] \\
        \quad \mathcal{V}_k &= \mathcal{V}_{k-1} \cup \{\xi_k \otimes \xi_k\}\\
        \quad R_{k,i} &= U_i - P_{\mathcal{V}_k}(U_i), \\ 
\end{aligned}
\end{equation}
for $k=1,...,K$, where $P_{\mathcal{V}_k}$ is the orthogonal projection operator onto $\text{span}\left(\mathcal{V}_k\right)$ and the process is initialized with $R_{0,i} = U_i$ and $\mathcal{V}_0=\emptyset$.
\par 
We would like to characterize the theoretical performance of the resulting approximation space, $\text{span}\left(\mathcal{V}_k\right)$, for representing the continuous connectivity $U_i$. In order to proceed, we make the following assumptions on $U$.
\begin{definition}\label{defn:smoothness_class}
Let $K\in\mathbb{N}_{\infty}$ and $0 < B < \infty$. Define $L_{1,B}$ as the class of functions
$$
L_{1,B}(\mathcal{V}_K) := \{u \in \mathcal{H}: u = \sum_{k=1}^K s_k\xi_k\otimes\xi_k, \sum_{k=1}^K |s_k| < B\}.
$$ 
where $s_{k} := \langle u, \xi_k\otimes \xi_k\rangle_{L^2(\Omega\times\Omega)}$, for $\xi_k\otimes\xi_k \in \mathcal{V}_K$.
\end{definition}
\begin{assumption}[Eigenfunction Smoothness]\label{assm:smoothness_class}
There exists some $\mathcal{V}_K^{*}$ for $K\in\mathbb{N}_{\infty}$ and 
$0 < B_1 < \infty$, such that $\psi_k \in L_{1,B_{1}}(\mathcal{V}_K^{*})$ for all $k=1,2,...$.
\end{assumption}
\begin{assumption}[Moment Bound]\label{assm:moment_bound}
For some $0 < B_2 < \infty$, $\sum_{k=1}^\infty |Z_k| < B_2$, holds with probability 1. 
\end{assumption}
\begin{assumption}[Tail Decay]\label{assm:decay_rate}
$\sum_{k=1}^\infty \sqrt{\rho_k} < \infty$
\end{assumption}
The function class in Assumption~\ref{defn:smoothness_class} has been used in the literature for establishing error convergence rates for deterministic function approximation algorithms \citep{Temlyakov2003NonlinearMO,barron2008}. This assumption is closely related to the smoothness of the $\psi_k$'s, see the Supplemental Materials for more details. Assumptions~\ref{assm:moment_bound} and \ref{assm:decay_rate} control the tail behavior of $U$. Note that Assumption~\ref{assm:decay_rate} introduces a slightly stronger condition on the decay rate of the spectrum than the one guaranteed by the mean square integrability of $C$, i.e. $\sum_{k=1}^\infty \rho_k <\infty$, though it is satisfied for many commonly used covariance kernels. The following theorem bounds the asymptotic mean $L^2$ representation error of the approximation space constructed from the greedy updates in \eqref{eqn:empirical_greedy_algorithm} as a function of $K$.
\begin{theorem}\label{thrm:sample_convergence_rate}
Let $U_1, ..., U_N$ be i.i.d. samples from $U$. Under Assumptions~\ref{assm:smoothness_class}, \ref{assm:moment_bound} and \ref{assm:decay_rate}, with probability 1:
$$
N^{-1}\sum_{i=1}^N \left\|R_{K,i}\right\|_{L^2(\Omega\times\Omega)}^2 \le   \frac{B_1^2\left(\sum_{k=1}^\infty\sqrt{\rho_k}\right)^2}{K+1}\quad\text{as}\quad N\rightarrow\infty
$$
\end{theorem}
In general, $\xi_k\otimes\xi_k\neq\psi_k$, so $\text{span}\left(\mathcal{V}_K\right)$ is not the optimal rank $K$ space for representing realizations of $U$. 
However, $\mathcal{V}_K$ offers a desirable trade-off between flexibility and computational complexity. More specifically, notice that \eqref{eqn:empirical_greedy_algorithm} requires solving an optimization problem over $L^2(\Omega)$, while estimating the eigenfunctions requires an optimization problem over $\mathcal{H}\subset L^{2}(\Omega\times\Omega)$. This simplification is critical in practice. For real data analysis, we must impose some finite dimensional discretization to represent and estimate the infinite dimensional functional parameters. This can be done by either imposing a dense grid on $\Omega$ or by using basis expansion. In any case, optimization for functions directly in $L^{2}(\Omega\times\Omega)$  squares the number of unknown parameters, resulting in enormous computational difficulties.
The flexibility of $\mathcal{V}_K$ is demonstrated in Theorem~\ref{thrm:sample_convergence_rate}, which establishes both asymptotic completeness and error bounds as a function of the rank. 

\subsection{Statistical Analysis of Reduced-Rank Continuous Connectivity}\label{ssec:inference}
We can approximate any function in $\mathcal{H}$ as a linear combination of basis functions in $\mathcal{V}_K$, thereby mapping the infinite dimensional continuous connectivity $U_i$ to a low-dimensional vector consisting of the coefficients of the basis expansion. As such, any continuous connectivity $U_i \in \mathcal{H}$ can be identified with a $K$-dimensional Euclidean vector $\boldsymbol{s}_i := [S_{i1},...,S_{iK}]^T$, with $P_{\mathcal{V}_K}(U_i) = \sum_{k=1}^K S_{ik}\xi_k\otimes\xi_k$. Owing to the orthonormality of the basis functions in $\mathcal{V}_K$, the mapping $U_i\mapsto \boldsymbol{s}_i$ is an isometry between $\left(\text{span}(\mathcal{V}_K), \langle\cdot,\cdot\rangle_{L^{2}(\Omega\times\Omega)}\right)$ and $\left(\mathbb{R}^K, \langle\cdot,\cdot\rangle_2\right)$, where $\langle\cdot,\cdot\rangle_2$ is the standard Euclidean metric. Therefore, we can properly embed the continuous connectivity into a $K$-dimensional Euclidean vector space and utilize a multitude of existing tools from multivariate statistics for analysis of $U_i$. For the remainder of this section, we discuss how to perform several canonical tasks of interest in computational neuroscience under our continuous connectivity data representation. 
\par
\noindent{\textit{Trait Prediction}: It is often of interest to use the structural connectivity to predict some trait of interest. This can be accommodated under our framework simply by using the embedding vectors $\boldsymbol{s}_i$ as features in an appropriate predictive model.}
\par
\noindent{\textit{Global Hypothesis Testing}: Another important application is the assessment of differences in structural connectivity between two groups. Given two samples of continuous connectivity: $\{U_{11}, ..., U_{1N_{1}}\},$ and $\{U_{21}, ..., U_{2N_{2}}\}$, we are interested in testing $U_1 \overset{\text{dist}}{=} U_2$, where $U_{li}\sim U_l$, and $l=1,2$ denotes the group membership. Using the continuous connectivity embedding, this testing problem is translated into a two-group test on the coefficients $\mathcal{S}_1:=\{\boldsymbol{s}_{11}, ..., \boldsymbol{s}_{1N_{1}}\}$ v.s. $\mathcal{S}_2:=\{\boldsymbol{s}_{21},...,\boldsymbol{s}_{2N_{2}}\}$. A non-parametric test to assess whether $\mathcal{S}_1$ and $\mathcal{S}_2$ are independent samples from the same distribution can be performed using the Maximum Mean
Discrepancy (MMD) test statistic \citep{gretton2012}.}
\par
\noindent{\textit{Identifying Local Subnetwork Differences Between Groups}: In addition to testing global connectivity difference, it is often of interest to identify where this difference manifests in the brain. In the atlas-based approaches, this problem corresponds to the identification of brain subnetworks related to phenotypic traits of interest and is of substantial interest in modern structural connectome analysis \citep{chung2021}. The natural solution under our framework is the identification of regions of the domain $\Omega\times\Omega$ where the continuous connectivity is different between groups. This is known as local inference in the FDA literature. A common approach is to represent the functional data using some basis system with local support, e.g., splines or wavelets, and then perform testing on the coefficients of the expansion \citep{pini2016}. The local support property is critical as it allows the effects of the coefficients to be localized on the domain. To perform local inference for the continuous connectivity, we must be able to construct locally supported $\xi_k$. We augment our greedy learning procedure to include a tunable constraint to promote basis functions with sparse support (more details are presented in Section~\ref{sec:methods}).}
\par 
Let $U_l\approx P_{\mathcal{V}_{K}}(U_{l}) = \sum_{k=1}^K S_{lk}\xi_k\otimes\xi_k$, with $l=1,2$ being the group label. The following theorem shows how we may relate hypothesis tests on the coefficient differences to the identification of subnetworks that are different between groups.
\begin{theorem}\label{thrm:continuous_subnetwork_discovery}
Define a collection of $K$ testing problems on the coefficients
\begin{equation}\label{eqn:testing_problem}
    H_{k}^0: S_{1k} \overset{\text{dist}}{=} S_{2k} \qquad H_{k}^a: S_{1k} \overset{\text{dist}}{\neq} S_{2k}, \qquad \text{for } k = 1,...,K.
\end{equation}
Denote the index set $I=\{k\in\{1,...,K\}:H_{k}^a\text{ is true}\}$, and define
$$
\text{Supp}(\xi_k) := \{ \omega_1 \in \Omega:\xi_k(\omega_1) \neq 0\},\quad\text{Supp}(\xi_k\otimes\xi_k) := \{ (\omega_1,\omega_2) \in \Omega\times\Omega:\xi_k(\omega_1)\xi_k(\omega_2) \neq 0\}
$$
and $\mathcal{C} := \bigcup_{k\in I}\text{Supp}\left(\xi_k\otimes\xi_k\right) \subset\Omega\times\Omega$.
A non-empty $I$ implies the following point-wise condition: 
$
\exists (\omega_1,\omega_2) \in \mathcal{C} \text{ such that } U_1(\omega_1,\omega_2) \overset{\text{dist}}{\neq} U_2(\omega_1,\omega_2).
$
\end{theorem}
The point-wise conclusion $U_1(\omega_1,\omega_2) \overset{\text{dist}}{\neq} U_2(\omega_1,\omega_2)$ is the infinite dimensional analog of a significant edge in the discrete network based approaches and therefore the set $\mathcal{C}$ can be considered a \textit{continuous subnetwork cover}. Since the group labels are exchangeable under $H_{k}^{0}$, the set of $K$ tests in Equation~\eqref{eqn:testing_problem} used to construct $\mathcal{C}$ can be performed using simple permutations and the resulting p-values corrected using \cite{holm1979} to control the family wise error rate (FWER). 

\section{Estimation and Implementation Details}\label{sec:methods}



%\begin{remark}
%The number of unknown parameters to estimate in a rank $K$ separable basis under the marginal representation \eqref{eqn:basis_expansion} is given by $K(M+N)$, compared to $NM^2/2$ in the corresponding (symmetric) tensor product basis. Since the global rank $K$ can typically be made much smaller than either of the marginal ranks $M_1,M_2$, this can amount to a dramatic reduction in the number of unknown parameters.
%\end{remark}
\subsection{Deriving the Optimization Problem}
Using the orthogonal constraint for elements in $\mathcal{V}_K$, the $k$-th greedy search of $\xi_k$ in \eqref{eqn:empirical_greedy_algorithm} can be equivalently formulated as:
\begin{equation}\label{eqn:empirical_optm_reformulated}
\begin{aligned}
    \hat{\xi}_k = &\sup_{\xi \in L^2(\Omega)}\frac{1}{N}\sum_{i=1}^N\left\langle R_{k-1,i}, \xi\otimes\xi\right\rangle_{L^2(\Omega\times\Omega)}^2 \\
    \textrm{s.t.} \quad & \langle \xi, \xi_j \rangle_{L^{2}(\Omega)} = 0 \text{ for }j=1,2,...,k-1, \quad \left\|\xi\right\|_{L^2(\Omega)} = 1 \\
\end{aligned}
\end{equation}
Unfortunately, problem \eqref{eqn:empirical_optm_reformulated} is intractable due to the infinite-dimensional search space $L^{2}(\Omega)$. In this section, we derive a discrete approximation of problem \eqref{eqn:empirical_optm_reformulated} that facilities efficient computation by the algorithm proposed in Section~\ref{ssec:algorithm}.
\par 
For tractable computation of the $L^2(\Omega\times\Omega)$ inner product, we impose a mesh grid on $\Omega\times\Omega$. Let $\boldsymbol{X} = (\boldsymbol{x}_{11}, ..., \boldsymbol{x}_{1n_{1}}, \boldsymbol{x}_{22}, ..., \boldsymbol{x}_{2n_{2}})^\intercal \in \mathbb{R}^{(n_1+n_2)\times 3}$ be the vertices on the grid. Note that since $\Omega$ is a union of two 2-spheres, $\{ \boldsymbol{x}_{11}, ..., \boldsymbol{x}_{1n_{1}}\}$ are points on $\mathbb{S}_1^2$ and $\{\boldsymbol{x}_{22}, ..., \boldsymbol{x}_{2n_{2}}\}$ are points on $\mathbb{S}_2^2$.  For subject $i$, denote the high-resolution symmetric continuous connectivity matrix:
$\boldsymbol{Y}_{i} =\begin{bmatrix}
                            \boldsymbol{Y}_{i,11} & \boldsymbol{Y}_{i,12}  \\
                            \boldsymbol{Y}_{i,12}^{\intercal}& \boldsymbol{Y}_{i,22}
                        \end{bmatrix}$,
where $\boldsymbol{Y}_{i,d_{1}d_{2}} \in \mathbb{R}^{n_{d_{1}}\times n_{d_{2}}}$ contains elements $\widehat{U}_i(\boldsymbol{x}_{d_{1}\cdot}, \boldsymbol{x}_{d_{2}\cdot})$. The inner product in \eqref{eqn:empirical_optm_reformulated} can now be approximated as 
\begin{equation}\label{eqn:discrete_l2_norm}
    \left\langle \widehat{R}_{k,i}, \xi\otimes\xi\right\rangle_{L^{2}(\Omega\times\Omega)}^2 \approx (n_1n_2)^{-1}\left\langle \boldsymbol{R}_{k,i}, \boldsymbol{\xi}\otimes\boldsymbol{\xi}\right\rangle_{F}^2,
\end{equation}
where $\langle,\rangle_{F}$ is the Frobenius inner product, $\boldsymbol{\xi}_j\in\mathbb{R}^{n_1+n_2}$ are the vectors of evaluations of $\xi_j$ on $\boldsymbol{X}$, $\boldsymbol{R}_{k,i} = \boldsymbol{Y}_i - \bar{\boldsymbol{Y}}  - \sum_{j=1}^k s_{ij}\boldsymbol{\xi}_j\otimes\boldsymbol{\xi}_j$, with 
\begin{equation}\label{eqn:coef_rewrite}
    s_{ij} = (n_1n_2)^{-1}\left\langle\boldsymbol{R}_{j-1,i},\boldsymbol{\xi}_j\otimes\boldsymbol{\xi}_j\right\rangle_{F}, 
    %\approx \langle \widehat{U}_i, \xi_j\otimes\xi_j\rangle_{L^{2}(\Omega\times\Omega)},
\end{equation}
and $\bar{\boldsymbol{Y}}$ is the mean of the $\boldsymbol{Y}_i$'s.

We now handle the infinite dimensional search space of $\xi_k\in L^2(\Omega)$ through basis expansion. Note that $\Omega$ is a union of two 2-spheres. We can trivially extend any complete basis system for $L^2(\mathbb{S}^2)$, denoted $\{\phi_{j}\}_{j=1}^\infty$, to $L^2(\Omega)$, since $L^2(\Omega) = L^2(\mathbb{S}^2)\cup L^2(\mathbb{S}^2) = \text{span}(\{\phi_{j}\}_{j=1}^\infty)\cup \text{span}(\{\phi_{j}\}_{j=1}^\infty)$.  Denoting the $M_d$-dimensional truncation $\boldsymbol{\phi}_{M_{d}} = (\phi_1, ..., \phi_{M_{d}})^\intercal$ (where $d \in \{1,2\}$ indexes the two spheres in $\Omega$), $\xi_k$ is approximated as 
\begin{equation}\label{eqn:basis_expansion}
 \xi_{k}(\omega) = \boldsymbol{c}_{1,k}^\intercal\boldsymbol{\phi}_{M_{1}}(\omega)\mathbb{I}\{\omega\in\mathbb{S}^2_1\} + \boldsymbol{c}_{2,k}^\intercal\boldsymbol{\phi}_{M_{2}}(\omega)\mathbb{I}\{\omega\in\mathbb{S}^2_2\},
\end{equation}
where the $\boldsymbol{c}_{d,k} \in \mathbb{R}^{M_{d}}$ are the vectors of coefficients with respect to the basis $\boldsymbol{\phi}_{M_{d}}$. Hence, an element in $L^2(\Omega)$ can be represented as $\boldsymbol{c}_k = (\boldsymbol{c}_{1,k}^\intercal,\boldsymbol{c}_{2,k}^\intercal)^\intercal$ with basis functions $\boldsymbol{\phi}_M = (\boldsymbol{\phi}_{M_{1}}^\intercal,\boldsymbol{\phi}_{M_{2}}^\intercal)^\intercal$, where $M = M_{1}+M_{2}$. In theory, $\{\phi_{j}\}_{j=1}^\infty$ can be taken as any complete basis system for $L^2(\mathbb{S}^2)$. In practice, we use spherical splines of degree 1, due to their appealing properties. For an overview on the construction of spherical splines, please visit the Supplemental Materials, or \cite{lai2007}.
\par 
In applications, it may be desirable to incorporate some constraints on the learned basis functions $\{\xi_k\}$. For example, we want to promote smoothness in the $\xi_k$ to ameliorate the effect of discretization. We may also want locally supported $\xi_k$ to facilitate the local inference/continuous subnetwork detection problem discussed in Section~\ref{ssec:inference}. Smoothness can be achieved through a regularization term that penalizes the candidate solution's ``roughness'', measured using the integrated quadratic variation: $\text{Pen}_{QV}(\xi_k) = \int_{\Omega}\|\nabla_{\Omega}\xi_k(\omega)\|^2d\omega$. Owing to the local support of the spherical spline basis functions, locally supported $\xi_k$ can be achieved by encouraging sparsity in the $\boldsymbol{c}_k$'s. In particular, our estimation procedure incorporates an optional constraint set: $\{\boldsymbol{c}\in\mathbb{R}^{M}:\|\boldsymbol{c}\|_0\le n_{\alpha_{2}}\}$, where $n_{\alpha_{2}}$ is a tuning parameter controlling the level of localization of the basis functions. 
\par 
Define $\boldsymbol{\Phi}_d\in\mathbb{R}^{n_d \times M_{d}}$ to be the matrix of evaluations of $\boldsymbol{\phi}_{M_{d}}$ over $\{ \boldsymbol{x}_{d1}, ..., \boldsymbol{x}_{dn_{1}}\}$ and denote the matrix of inner products $\boldsymbol{J}_{d} = \int_{\mathbb{S}^2}\boldsymbol{\phi}_{M_{d}}\boldsymbol{\phi}_{M_{d}}^\intercal$. Define the block matrices 
$$
\boldsymbol{\Phi} = \begin{bmatrix} 
                       \boldsymbol{\Phi}_1 & \boldsymbol{0} \\
                        \boldsymbol{0} &\boldsymbol{\Phi}_2
                \end{bmatrix}, \quad \boldsymbol{J}_{\phi} = \begin{bmatrix} 
\boldsymbol{J}_{1} & \boldsymbol{0} \\
\boldsymbol{0} &  \boldsymbol{J}_{2}
\end{bmatrix}.
$$
After incorporating the smoothness and local support constraint, the final formulation of \eqref{eqn:empirical_optm_reformulated}
is given by 
\begin{equation}\label{eqn:empirical_optm_reformulated_discretized}
\begin{aligned}
    \hat{\boldsymbol{c}}_k = &\underset{\boldsymbol{c} \in \mathbb{R}^{M}}{\text{ argmax }}\frac{1}{Nn_1n_2}\sum_{i=1}^N\left\langle \boldsymbol{R}_{k-1,i}, (\boldsymbol{\Phi}\boldsymbol{c})\otimes (\boldsymbol{\Phi}\boldsymbol{c})\right\rangle_{F}^2 -  \alpha_1 \boldsymbol{c}^\intercal\boldsymbol{Q}_{\boldsymbol{\phi}}\boldsymbol{c} \\
    \textrm{s.t.} \quad & \boldsymbol{c}^\intercal\boldsymbol{J}_{\phi}\boldsymbol{c} = 1, \quad \boldsymbol{c}^\intercal\boldsymbol{J}_{\phi}\boldsymbol{c}_j  = 0 \text{ for }j=1,2,...,k-1, \quad \left\|\boldsymbol{c}\right\|_{0} \le n_{\alpha_{2}} \\
\end{aligned}
\end{equation}
where $\alpha_1, n_{\alpha_{2}} > 0$ are hyperparameters used to control the smoothness and local support size, respectively, and $ \boldsymbol{c}^\intercal\boldsymbol{Q}_{\boldsymbol{\phi}}\boldsymbol{c}$ encodes $\text{Pen}_{QV}(\xi_k)$ after basis expansion (see the Supplemental Materials for more details).  Efficient algorithms exist for evaluating spherical splines, computing their directional derivatives as well as performing integration. As a result, the matrices $\boldsymbol{J}_{\boldsymbol{\phi}}$ and $\boldsymbol{Q}_{\boldsymbol{\phi}}$ can be constructed cheaply (see the Supplementary Materials or \cite{schumaker2015}). 

\subsection{Algorithm}\label{ssec:algorithm} 
Denote $\mathcal{Y}$ as the $(n_1 + n_2) \times (n_1 + n_2) \times N$-dimensional semi-symmetric tensor obtained from a mode-3 stacking of the $\boldsymbol{Y}_i-\bar{\boldsymbol{Y}}$. 
The computational grid $\boldsymbol{X}$ can be made arbitrarily dense, rendering $\mathcal{Y}$ an enormously high dimensional ``functional tensor'' object. This prohibits a standard tensor decomposition applied to $\mathcal{Y}$ and necessitates the development of our efficient algorithm discussed below. 
\par 
The optimization problem \eqref{eqn:empirical_optm_reformulated_discretized} is a constrained maximization of a degree 4 polynomial with $M \ge 3$ variables and thus is NP-hard \citep{hou2014}. To derive a computationally tractable algorithm, we first notice that by combing Equations~\eqref{eqn:coef_rewrite} and \eqref{eqn:basis_expansion}, we have that 
\begin{equation}\label{eqn:coef_rewrite_basis}
    s_{ik} \approx (n_1n_2)^{-1}\langle \boldsymbol{R}_{k-1,i}, \left(\boldsymbol{\Phi}\boldsymbol{c}_k\right)\otimes\left(\boldsymbol{\Phi}\boldsymbol{c}_k\right)\rangle_{F}.  \\
\end{equation}
Using approximation \eqref{eqn:coef_rewrite_basis} and introducing the associated auxiliary variable $\boldsymbol{s}=(s_1,...,s_{N})^\intercal\in\mathbb{R}^{N}$, \eqref{eqn:empirical_optm_reformulated_discretized} can be equivalently defined as 
\begin{equation}\label{eqn:empirical_optm_reformulated_discretized_AO}
\begin{aligned}
    \hat{\boldsymbol{c}}_k = &\underset{\boldsymbol{c} \in \mathbb{R}^{M}}{\text{ argmax }}\sum_{i=1}^Ns_i\left\langle\boldsymbol{R}_{k-1,i}, \left(\boldsymbol{\Phi}\boldsymbol{c}\right)\otimes\left(\boldsymbol{\Phi}\boldsymbol{c}\right)\right\rangle_{F} -  \alpha_1 \boldsymbol{c}^\intercal\boldsymbol{Q}_{\boldsymbol{\phi}}\boldsymbol{c} \\
    \textrm{s.t.} \quad & \boldsymbol{c}^\intercal\boldsymbol{J}_{\phi}\boldsymbol{c} = 1, \boldsymbol{c}^\intercal\boldsymbol{J}_{\phi}\boldsymbol{c}_j  = 0 \text{ for }j=1,2,...,k-1,\\
    \quad & \left\|\boldsymbol{c}\right\|_{0} \le n_{\alpha_{2}}  , \quad s_i = \langle \boldsymbol{R}_{k-1,i}, \left(\boldsymbol{\Phi}\boldsymbol{c}\right)\otimes\left(\boldsymbol{\Phi}\boldsymbol{c}\right)\rangle_{F}, \text{ for } i=1,...,N.
\end{aligned}
\end{equation}
\par 
We apply an alternating optimization (AO) scheme to \eqref{eqn:empirical_optm_reformulated_discretized_AO}, iteratively maximizing $\boldsymbol{c}$ given $\boldsymbol{s}$ and vice versa. A data-reduction transformation based on the singular value decomposition $\boldsymbol{\Phi}_d = \boldsymbol{U}_d\boldsymbol{D}_d\boldsymbol{V}_d^\intercal$ is utilized in order to avoid computations that scale with the number of grid points (the dimension of $\boldsymbol{Y}$). Define the block matrices 
$$
\boldsymbol{V} = \begin{bmatrix} 
                        \boldsymbol{V}_1 & \boldsymbol{0} \\
                        \boldsymbol{0} & \boldsymbol{V}_2
                \end{bmatrix}, \qquad 
                 \boldsymbol{D} = \begin{bmatrix} 
                        \boldsymbol{D}_1 & \boldsymbol{0} \\
                        \boldsymbol{0} & \boldsymbol{D}_2
                \end{bmatrix}, \qquad \boldsymbol{U} = \begin{bmatrix} 
                        \boldsymbol{U}_1 & \boldsymbol{0} \\
                        \boldsymbol{0} & \boldsymbol{U}_2
                \end{bmatrix},
$$
and define $\boldsymbol{G}_{k,i} := \boldsymbol{U}^\intercal\boldsymbol{R}_{k,i}\boldsymbol{U}\in\mathbb{R}^{M\times M}$, which is the transformed residual of $\boldsymbol{R}_{k,i}$ for the $i$'th subject . Note that the columns of $\boldsymbol{U}$ form an orthonormal basis for the $M$-dimensional regression subspace of $\boldsymbol{\Phi}$ and therefore this transformation can be understood as mapping the rows and columns of $\boldsymbol{R}_{k,i}$ into the span of this subspace. By the properties of the Frobenius inner product, we have $\left\langle\boldsymbol{R}_{k-1,i}, \boldsymbol{\Phi}\boldsymbol{c}\otimes\boldsymbol{\Phi}\boldsymbol{c}\right\rangle_{F}=\left\langle\boldsymbol{G}_{k-1,i}, \boldsymbol{D}\boldsymbol{V}^\intercal\boldsymbol{c}\otimes\boldsymbol{D}\boldsymbol{V}^\intercal\boldsymbol{c}\right\rangle_{F}$. Crucially, this identity can be used in problem \eqref{eqn:empirical_optm_reformulated_discretized_AO} to avoid the computational burden of storing and computing with matrices of dimension $(n_1+n_2)\times(n_1+n_2)$.
\par 
Define the $M\times M \times N$-dimensional tensor $\mathcal{G}_{k}$ to be the mode-3 stacking of the $\boldsymbol{G}_{k,i}$. Then, by definition of the $d$-mode tensor-matrix multiplication (denoted $\times_{d}$), $\mathcal{G}_{0} := \mathcal{Y}\times_1\boldsymbol{U}^\intercal\times_2\boldsymbol{U}^\intercal$. Under the AO scheme, the update for the block variable $\boldsymbol{c}_k$ at the $t+1$ iteration is given by 
\begin{equation}\label{eqn:ctilde_update}
\begin{aligned}
    \boldsymbol{c}^{(t+1)} = \underset{\boldsymbol{b}\in\mathbb{R}^{M}}{\text{max}} &\quad \boldsymbol{b}^\intercal\left[\boldsymbol{V}\boldsymbol{D}\left(\boldsymbol{I} - \boldsymbol{P}_{k-1}\right)\left[\mathcal{G}_{k-1}\times_3\boldsymbol{s}^{(t)} - \alpha_1\boldsymbol{D}^{-1}\boldsymbol{V}^\intercal\boldsymbol{Q}_{\boldsymbol{\phi}}\boldsymbol{V}\boldsymbol{D}^{-1}\right]\left(\boldsymbol{I} - \boldsymbol{P}_{k-1}^{\intercal}\right)\boldsymbol{D}\boldsymbol{V}^\intercal\right]\boldsymbol{b} \\
    & \textrm{s.t.} \quad \boldsymbol{b}^\intercal\boldsymbol{J}_{\boldsymbol{\phi}}\boldsymbol{b} = 1, \quad \left\|\boldsymbol{b}\right\|_{0} \le n_{\alpha_{2}} , \\
\end{aligned}
\end{equation}
where 
\begin{equation}\label{eqn:update_P}
        \boldsymbol{P}_{k-1} = \boldsymbol{D}\boldsymbol{V}^\intercal\boldsymbol{C}_{k-1}\left[\boldsymbol{C}_{k-1}^{\intercal}\boldsymbol{J}_{\boldsymbol{\phi}}\boldsymbol{C}_{k-1}\right]^{-1}\boldsymbol{C}_{k-1}^{\intercal}\boldsymbol{J}_{\boldsymbol{\phi}}\boldsymbol{V}\boldsymbol{D}^{-1},  \quad \boldsymbol{C}_{k-1} := \left[\boldsymbol{c}_1, ..., \boldsymbol{c}_{k-1}\right],
\end{equation}
and the $\boldsymbol{c}_{j}$'s are from the previous $k-1$ selections. For $\boldsymbol{s}$, the update at the $t+1$ iteration is given in closed form by
\begin{equation}\label{eqn:s_update}
    \boldsymbol{s}^{(t+1)} = \mathcal{G}_{k-1} \times_1 (\boldsymbol{D}\boldsymbol{V}^\intercal\boldsymbol{c}_k^{(t+1)})\times_2 (\boldsymbol{D}\boldsymbol{V}^\intercal\boldsymbol{c}_k^{(t+1)}).
\end{equation}
For a detailed derivation of \eqref{eqn:ctilde_update} and \eqref{eqn:s_update}, please visit the Supplementary Materials.
\par 
If no sparsity constraint is employed, \eqref{eqn:ctilde_update} reduces to finding the leading generalized eigenvector of a symmetric matrix. Since $\boldsymbol{J}_{\boldsymbol{\phi}}$ is symmetric and positive definite, this problem has a unique solution. Since \eqref{eqn:s_update} is trivially unique, the AO scheme of Algorithm~\ref{alg:rank_1_ssb} is guaranteed to converge to a stationary point of the objective by the existence and uniqueness property \citep{bezdek2003}.
\par 
Alternatively, with the sparsity constraint active, \eqref{eqn:ctilde_update} is recognized as a sparse generalized eigenvalue problem (SGEP), for which several recent methods could be applied to obtain a solution \citep{tan2018,jung2019,cai2021}. 
%To establish existence and uniqueness of SGEP, additional assumptions on the problem structure are required \citep{cai2021}. Even so, solution algorithms can typically be shown to converge to a local optimum. 
Due to computational efficiency considerations, in this work we opt to relax the
constraint $\boldsymbol{b}^\intercal\boldsymbol{J}_{\boldsymbol{\phi}}\boldsymbol{b} =1\mapsto\boldsymbol{b}^\intercal\boldsymbol{b}=1$ and then apply the fast truncated power iterations method from \cite{yuan2011}. Since $\boldsymbol{J}_{\boldsymbol{\phi}}$ is positive definite, this relaxation simply corresponds to looking for an orthogonal solution, rather than an orthonormal one. Orthonormality can be enforced by post-hoc normalization. 
\par 
Algorithm~\ref{alg:rank_1_ssb} provides pseudocode for the proposed AO scheme. Notice that the only computation that scales with the number of grid points is the transformation of the functional tensor $\mathcal{Y}$ into the tensor $\mathcal{G}$, which happens only once during the initialization of the procedure. Since typically $M \ll n_1+n_2$, this can amount to an enormous savings in computation when compared to an alternative approach of performing tensor decomposition directly on $\mathcal{Y}$. For instance, it is known that the tensor rank decomposition of a semi-symmetric mode-3 tensor can be obtained using simultaneous matrix diagonalization \citep{lathauwer2006}, the algorithms for which typically require on the order of $O((n_1 + n_2)^3)$ operations per iteration \citep{chabriel2014}. As $\boldsymbol{X}$ can be taken to arbitrarily high resolution, this underscores the practical computational importance of the reduction transformation utilized in our framework.
\par 
The block update \eqref{eqn:ctilde_update} requires an initialization for $\boldsymbol{c}^{(0)}$ and $\boldsymbol{s}^{(0)}$, reasonable values for which can be obtained using the leading left singular vectors of the mode-1 and mode-3 matricization of $\mathcal{G}_{k-1}$, respectively. For further justification of the chosen initialization procedure, see the Supplementary Materials. 


\begin{algorithm}
\caption{AO Algorithm to approximate \eqref{eqn:empirical_optm_reformulated_discretized_AO}}\label{alg:rank_1_ssb}
\begin{algorithmic}[1]
\State \textbf{Input}: $\text{Tensor }\mathcal{Y}; \text{ matrices }\boldsymbol{J}_{\boldsymbol{\phi}}, \boldsymbol{Q}_{\boldsymbol{\phi}}, \boldsymbol{U},\boldsymbol{V},\boldsymbol{D};  \text{ rank }K; \text{ hyperparameters } \alpha_1, n_{\alpha_{2}}$
\State \textbf{Output}: $\boldsymbol{C}, \boldsymbol{S}$
\State \textbf{Initialize}: $\mathcal{G}_{0} \gets  \mathcal{G} := \mathcal{Y}\times_1\boldsymbol{U}^\intercal\times_2\boldsymbol{U}^\intercal$; $\boldsymbol{C} \gets \emptyset$; $\boldsymbol{S}\gets \emptyset$; $\boldsymbol{P}_0\gets \boldsymbol{0}_{M\times M}$
\For{$k=1,...K$}
    \State \textbf{Initialize} $\boldsymbol{s}_k^{(0)}$  using the leading left singular vector of the mode-3 matricization of $\mathcal{G}_{k-1}$
    \State \textbf{Initialize} $\boldsymbol{c}_k^{(0)}$ using  $\boldsymbol{V}\boldsymbol{D}^{-1}$ product with the leading left singular vector of the mode-1 matricization of $\mathcal{G}_{k-1}$
    \While{\text{Not Converged}}
        \State 
        \State \textbf{Update} $\boldsymbol{c}_k^{(t+1)}$ according to \eqref{eqn:ctilde_update} using initial guess $\boldsymbol{c}_k^{(t)}$
        \State \textbf{Update} $\boldsymbol{s}_k^{(t+1)}$ according to \eqref{eqn:s_update}
    \EndWhile
    \State Compute $\boldsymbol{P}_k$ using \eqref{eqn:update_P}
    \State $\mathcal{G}_{k} \gets \mathcal{G}_{k-1}- \left(\boldsymbol{D}\boldsymbol{V}^\intercal\boldsymbol{c}_k^{(t+1)}\right) \otimes \left(\boldsymbol{D}\boldsymbol{V}^\intercal\boldsymbol{c}_k^{(t+1)}\right) \otimes  \boldsymbol{s}_k^{(t+1)}$
    \State $\boldsymbol{C} \gets \left[\boldsymbol{C};\boldsymbol{c}_k^{(t+1)}\right]$
    \State $\boldsymbol{S} \gets \left[\boldsymbol{S}; \boldsymbol{s}_k^{(t+1)}\right]$
\EndFor

\end{algorithmic}
\end{algorithm}


\subsection{Hyperparameter Selection}\label{ssec:hyper_param_select}

\noindent{\textit{Smoothness and Sparsity}: Algorithm~\ref{alg:rank_1_ssb} requires specifying the penalty parameters $\alpha_1$ (dictating the degree of smoothness of the solution), and $n_{\alpha_{2}}$ (determining the size of the support of $\xi_k$). In practice, $\alpha_1$ can be selected through cross validation on the rank-1 approximation. In our real data analysis, we found small values were preferable, likely due to the fact that the functional data has already been smoothed via KDE over a dense grid. The local support parameter $ n_{\alpha_{2}}$ can be used if locally supported basis functions are desirable, e.g., for identifying local subnetworks that are different between groups, and can be tuned according to the desired sparsity level.  
\par 
\noindent{\textit{Rank Selection}: It is also important to select both the marginal ranks ($M_1$ and $M_2$ to represent $\xi_k$) and the global rank $K$. The global rank can be selected using a threshold criteria on the proportion of variance explained, estimated using the transformed tensor by $\left\|\mathcal{G}_{K}\right\|_{F}^2/\left\|\mathcal{G}\right\|_{F}^2$. Similarly, selecting the marginal ranks can be accomplished using a threshold criteria on $\|\mathcal{Y}\times_1\boldsymbol{U}^\intercal\times_2\boldsymbol{U}^\intercal\|_{F}^2/\|\mathcal{Y}\|_{F}^2$, where $\boldsymbol{U}$ are obtained from the SVD of basis evaluation matrices $\boldsymbol{\Phi}=\boldsymbol{U}\boldsymbol{D}\boldsymbol{V}^{\intercal}$ for a set of increasing $M_1,M_2$. This quantity can be considered as an estimate of the proportion of variance explained by $\text{span}(\boldsymbol{\phi}_{M}\otimes\boldsymbol{\phi}_{M})$.}
\par 
\noindent{\textit{Spherical Triangulation}: The optimization problem \eqref{eqn:empirical_optm_reformulated_discretized_AO} is dependent on the underlying spherical triangulation, denoted $\mathcal{T}_d$, used to define the spherical spline basis. For example, the geometric properties of the spherical triangles in $\mathcal{T}_{d}$ and the spatial distribution of vertices can heavily affect the approximation power of $\boldsymbol{\phi}_{M_{d}}$ \citep{shewchuk2002}. It is therefore important to have a procedure to construct $\mathcal{T}_d$. As a result of the surface inflation based spherical parameterization of the cortical white surfaces, the grid points $\boldsymbol{X}$ will be irregularly spaced over $\Omega$. Therefore, we use a simple pruning heuristic to design $\mathcal{T}_d$, independently for each copy of $\mathbb{S}^2_d$, such that the local density of basis functions is aligned to the spatial distribution of $\boldsymbol{X}$. In particular, our approach consists of the following steps: i) initiate a dense set of (nearly) equispaced vertices over $\mathbb{S}^2$, ii) compute the pairwise distances between this vertex set and the grid $\boldsymbol{X}$ iii) sequentially prune vertices that have the largest minimum distance to the grid points until $M_d$ vertices are left, iv) define $\mathcal{T}_d$ to be the spherical Delaunay tessellation \citep{lai2007} over this refined vertex set. This simple heuristic was observed to consistently result in better $L^2$ reconstruction performance than the (nearly) equispaced vertex strategy for the same $M_d$. 

\section{Simulation Study}\label{sec:simulation}
 
In this section, we investigate the performance of our algorithm on simulated data. We study the convergence for both the in-sample (residual) error, as well as the generalization error on an independent test set, as a function of rank $K$ and sample size $N$. We also consider the computational performance of our algorithm in a variety of settings.
\par 
We simulated continuous connectivity according to:
$U(\omega_1, \omega_2) = \sum_{k=1}^{K_{true}} S_k\xi_k(\omega_1)\xi_k(\omega_2) $
where $\xi_k(\omega) = \boldsymbol{c}_{k}^\intercal \boldsymbol{\phi}_{M}(\omega)$, for $\boldsymbol{\phi}_{M}(\omega) = (\boldsymbol{\phi}_{M_{1}}^\intercal(\omega), \boldsymbol{\phi}_{M_{2}}^\intercal(\omega))^\intercal$ and $\boldsymbol{\phi}_{M_{d}}$ is the linear spherical spline basis formed by the Delaunay  triangulation of $M_1=M_2=410$ vertices. To generate the $\xi_k$, we independently sampled $\boldsymbol{c}_{k}\sim\mathcal{N}(\boldsymbol{0},0.2^2\boldsymbol{I})$. 
The random coefficients $S_{k}$ were drawn independently from $\mathcal{N}(0, k^{-1})$. The true rank was fixed to $K_{true}=20$. The $U$ were evaluated at all pairs of $n_1 + n_2 = 4,121$ points in the grid $\boldsymbol{X}$ over $\Omega$ discussed in Section~\ref{sec:data}. All experiments were performed using MATLAB/2020 on a Linux machine with a 2.4 GHz Intel Xeon CPU E5-2695 and 32GB of RAM. 

\subsection{Reconstruction Error Analysis}

We study the connectivity reconstruction error as a function of $K$ for training sample sizes $N\in\{10,50,100\}$. For each sample size, in addition to the training data, we independently sampled  $100$ $U_i$'s to serve as a test set for estimating the generalization error of $P_{\mathcal{V}_{K}}$, for $\mathcal{V}_{K}$ constructed from the training set. For each setting, 100 replicated experiments were performed and the mean integrated square error (MSE) of the reconstructed connectivity was estimated for both training and testing data.  We used the marginal spline basis system for approximation and fixed a small roughness penalty parameter. The sparsity constraint was not active.
\par 
Figure~\ref{fig:simulation_analysis}a shows the MSE as a function of $K$ for different choices of $N$. As $N$ increases, we observe the in-sample (training) and out-sample (testing) error curves converge to one another. The black curve is $\propto(K+1)^{-1}$, in accord with the asymptotic error bound for the global optimum derived in Theorem~\ref{thrm:sample_convergence_rate}, with constant multiple defined by averaging the errors computed for the rank 1 case. We see that for all $K$ and $N$, on average, the errors obey the theory. Recall that the convergence of the proposed AO procedure is to a stationary point, which may not be the global solution. These simulation results indicate that the proposed AO procedure can still construct solutions which exhibit the established convergence properties.
%\begin{figure}[t]
%    \centering
    %\includegraphics[scale=0.6]]{Figures/train_test_error_analysis.pdf}
    %\caption{Average sample (solid-lines) and generalization (dashed-lines) error as a function of model rank $K$ for several $N$. The black line is $\propto(K+1)^{-1}$, in accord with the theoretical asymptotic bound from Theorem~\ref{thrm:sample_convergence_rate}.}
    %\label{fig:convergence_analysis}
%\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.5]{Figures/simulation_results_CC_collected.pdf}
    \caption{(a) Average sample (solid-lines) and generalization (dashed-lines) error as a function of model rank $K$ for several $N$. The black line is $\propto(K+1)^{-1}$. (b) Average per-iteration computational time for the updates \eqref{eqn:ctilde_update} and \eqref{eqn:s_update} as a function of sample size $N$ (top) and marginal rank $M$ (bottom).}
    \label{fig:simulation_analysis}
\end{figure} 

\subsection{Computational Performance}
We now investigate the computational performance of the rank-1 updates in Algorithm~\ref{alg:rank_1_ssb}, which require iteratively solving \eqref{eqn:s_update} and \eqref{eqn:ctilde_update}. We consider all combinations of sample sizes $N\in\{10,50,100,200\}$ and marginal ranks $M\in\{36, 132, 516, 2052\}$. For each configuration, Algorithm~\ref{alg:rank_1_ssb} was run 10-times and the mean per-update computational time was recorded along with the number of iterations required for convergence. Convergence was assessed by computing the relative change in the objective function between iterations of the inner loop in Algorithm~\ref{alg:rank_1_ssb}, terminating when a sufficiently small value ($10^{-6}$) was reached. The median number of iterations to convergence was $4$, with the minimum and maximum being $3$ and $14$, respectively, indicating that our algorithm converges quickly under a variety of settings.
\par 
Figure~\ref{fig:simulation_analysis}b displays the average computational time per update of both  $\boldsymbol{c}_k$ and $\boldsymbol{s}_k$. For updating $\boldsymbol{s}_k$, the computational time has an approximately linear relationship with the sample size $N$ (left panel) and approximately quadratic relationship with spline rank $M$ (right panel). This is predicted by the theoretical complexity analysis: update  \eqref{eqn:s_update} can be computed at a computational cost of $O\left(N\left(M + M^2\right) + M^2\right)$. Updating  $\boldsymbol{c}_k$ is quite fast, on the order of $0.1$ seconds or less, for all the settings considered. 
%\begin{figure}
%    \centering
%    \includegraphics[scale=0.5]{Figures/computational_comparison_cc-1.pdf}
%    \caption{Average per-iteration computational time for the updates \eqref{eqn:ctilde_update} and \eqref{eqn:s_update} for as a function of sample size $N$ (left), sparsity constraint $\alpha_2$ (center) and marginal rank $M$ (right).}
%    \label{fig:computational_analysis}
%\end{figure} 
 
\section{Real Data Applications}\label{sec:real_data_experiments}
In this section, we demonstrate our continuous connectivity framework, denoted CC, on several statistical tasks of interest for neuroscience applications. We used the computation grid $\boldsymbol{X}$ on $\Omega$ with $n_1+n_2 = 4,121$, as outline in Section~\ref{sec:data}. To form $\widehat{U}_i$ from the streamline endpoints of subject $i$ at all points on $\boldsymbol{X}$, the KDE bandwidth was set to be $h=0.005$ in Equation~\eqref{eqn:KDE_cc}, in accordance with the experiments in \cite{cole2021}. For all models considered in this section, we used a spherical spline basis with $M_1=M_2=410$, selected using an $85\%$ threshold on the criteria described in Section~\ref{ssec:hyper_param_select}. See the Supplemental Materials for a figure displaying the grid and spherical triangulations for both copies of $\mathbb{S}^2$. The roughness penalty parameter was selected to be $\alpha_1=10^{-8}$. The sparsity constraint was not active in the analysis in Sections \ref{ssec:reproducibility} and \ref{ssec:compare_network_embed},  while in the analysis in Section \ref{ssec:network_discovery} we selected $n_{\alpha_{2}}=50$ to produce in $\approx 95\%$ sparsity in the rank-1 coefficient vector.  

\subsection{CC Reproducibility Analysis}\label{ssec:reproducibility}
We are interested in studying the reproducibility of the proposed reduced-rank representation on real data. More specifically, we want to understand how well the reduced-rank function space, $\text{span}\left(\mathcal{V}_K\right)$, estimated from one population can represent the re-scanned data from the same population. In absence of disease, we expect the brain organization of a healthy adult to be relatively constant over the span of several months and therefore the HCP scan-rescan data can be considered as independent noisy samples of the same connectome, making it appealing for evaluating reproducibility. In particular, we used the subjects scan-1 data to form estimates $\hat{\xi}_k$ according to the procedure in Section~\ref{sec:methods}. For several $K$, the estimated $\mathcal{V}_K = \{\hat{\xi}_1, ...,\hat{\xi}_K\}$ were used to represent the scan-2 data by standard basis expansion under the least squares principle. In Figure~\ref{fig:reproducibility_analysis}a, we show the first three coefficients corresponding to $\{\hat{\xi}_1,\hat{\xi}_2,\hat{\xi}_3\}$ for a random collection of 10 test-retest subjects. The unique markers identify multiple scans from the same individual. One can see that a within-subject clustering pattern is already present using only $K=3$ basis functions. 
\par
The pairwise $L^2(\Omega\times\Omega)$ distances between the basis expansion representations of all the scan-1 and scan-2 data were computed. Figure~\ref{fig:reproducibility_analysis}b displays the pairwise distance matrices for several different $K$'s. Each matrix is $74 \times 74$, giving the pairwise distances between the $74$ scans from $37$ subjects. Scans from the same subject are put next to each other, generating small $2\times2$ blocks along the diagonal. A quantitative assessment of the reproducibility was obtained using the leave-one-out cross validated (LOOCV) accuracy of the nearest neighbor classifier applied to the distances: for each representation $i$, we compute $j = \text{argmin}_{l\neq i} \text{dist}(i,l)$, where $\text{dist}(i,l)$ is shorthand for the distance between scans $i$ and $l$. The LOOCV accuracy is computed as the fraction of examples where $i$ and $j$ are two scans corresponding to the same individual. At the bottom of Figure~\ref{fig:reproducibility_analysis}b  we show the LOOCV accuracy results. With $K=22$, we achieved a $100\%$ classification accuracy. 

\begin{figure}
    \centering
   \includegraphics[scale=0.43]{Figures/reproducibility_alt.pdf}
    \caption{(a) The low-rank embeddings for 10 randomly selected HCP test-retest subjects using $K=3$. Each subject is identified by a unique marker. (b) Pairwise distance matrices for $74$ scans from $37$ subjects under several $K$'s. The LOOCV accuracy of the nearest neighbor classier applied to the distances is also recorded.}
    \label{fig:reproducibility_analysis}
\end{figure}


\subsection{Relating Brain Networks to Traits}\label{ssec:compare_network_embed}

We compare the embeddings produced by our continuous approach to those constructed from atlas-based networks using several state-of-the-art joint network embedding methods, namely, Tensor-Network PCA (TN-PCA) \citep{zhang2019}, Multiple Random Dot-Product Graph model (MRDPG) \citep{nielsen2018} and Multiple Adjacency Spectral Embedding method (MASE) \citep{arroyo2021b}, on both hypothesis testing and prediction tasks. For evaluation, we used the sample of 437 female HCP subjects and their corresponding traits. 
\par 
Streamline count-based connectome matrices were formed from each subject's tractography result using both the Desikan (with 68 cortical parcels) and Destriex (with 148 cortical parcels) atlases. MRDPG and MASE require a binary adjacency matrix representation of the connectivity, which was obtained by thresholding the count-based connectome matrices, while TN-PCA was applied directly to the count matrices. To facilitate fair comparison, $K=100$ embedding dimensions were used for all methods, except MRDPG applied to the Desikan atlas, since this method requires $K\le V$, and hence we let $K=68$. The K-dimensional embeddings  were used as representations of the SC in subsequent analysis tasks. All of the analysis was performed using R/4.0.2 and MATLAB/2020b on a  Linux cluster equipped with 120GB of RAM.  %Note that TN-PCA can be applied to interval data, in theory it is possible to utilize this method directly on the sample of high-resolution connectivity matrices. In practice, this failed due to memory error, even with the large RAM allocation used for this study. This again underscores the importance of the ability of Algorithm~\ref{alg:rank_1_ssb} to control the dimensionality of the problem by transforming the observed high resolution connectivity tensor $\mathcal{Y}$ to the reduced data tensor $\mathcal{G}$.

\subsubsection{Hypothesis Testing}\label{sssec:hypothesis_testing}
We first compare the power of the embeddings produced by different methods for identifying group differences. The groups are defined as follows: for each of the 80 measured traits in the categories \textit{cognition}, \textit{emotion}, and \textit{sensory}, two groups were created by selecting the top 100 and bottom 100 of the 437 HCP females, in terms of their measured trait score. For each trait, we use the MMD test to test the null hypothesis that the groups of embedding vectors were drawn from the same distribution. The corresponding p-values were computed using 10,000 Monte-Carlo resampling iterations and corrected for false discovery rate (FDR) control using \cite{benjamini1995}.
\par 
The fours panels in Figure~\ref{fig:global_inference} show the p-value results for different embedding methods. The discrete network-based analysis was performed using the Destriex atlas. The y-axis gives the negative log transformed p-values and the colors indicate significant discoveries under a couple FDR control levels. With a threshold of $\text{FDR}\le 0.05$, the embeddings produced by our method are able to identify 22 significant discoveries, compared to 7 or less for the competitors. \par 
Figure~\ref{fig:global_inference_Desikan} in the Supplemental Materials shows the corresponding results for the network-based approaches using the Desikan atlas. The results indicate both fewer and, perhaps more saliently, different discoveries than using the Destriex. The sensitivity of the analysis to the choice of atlas can be a major drawback to the network-based approaches. Not only does our continuous framework produce uniformly more powerful embeddings, i.e., by modeling the SC data at much higher resolutions, but the inherent atlas-independence reduces the contingency of the reported results. 

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.45]{Figures/significant_embeddings_reformatted.pdf}
    \caption{Results from the global hypothesis testing task. The y-axis gives the $-\text{log}_{10}$-transformed p-values from the MMD test. Network-based analyses (TN-PCA, MASE, and MRDPG) were performed using the Destriex Atlas.}
    \label{fig:global_inference}
\end{figure}

\subsubsection{Trait Prediction}\label{sssec:trait_prediction}
We now compare the performance of the different methods for the task of predicting various trait measurements from the SC. Many of the trait measurements in HCP are under the same category (e.g., fluid intelligence, executive function and emotion recognition) and can be highly correlated with one another. Therefore, we constructed a set of composite measures using principal component analysis (PCA). In particular, we first grouped these measurements, discarding any that were binary or categorical. The categories considered were: fluid intelligence, processing speed, self regulation and impulse control, sustained attention, executive function, psychiatric, taste, emotional recognition, anger and hostility and finally BMI and weight. A PCA was performed for each category and the first $n$ PCs that explain $\ge 90\%$ of the variance were selected. Each subject's measurements were then projected onto each of the principal directions to get PC scores, which were used as outcomes for the trait prediction task. In all, there were 31 of these.
\par 
The embeddings were used as features in a LASSO regression model for the various outcomes of interest. For each outcome of interest, we performed 100 random 80-20 train-test splits of the data. The LASSO regularization parameter was selected with cross validation using the training data. The trained model was then applied to the test set and the Pearson correlation ($\rho$) between the predicted and observed values was recorded. Any outcome whose predictions were not deemed significantly associated (random train-test split average $\rho > 0.1$) with \textit{any} of the embedding frameworks was discarded from analysis. In all, 15 out of the original 31 outcomes met this criteria. 
\par 
Table~\ref{tab:concon_vs_atlas} records the Pearson correlation averaged over the random train-test splits for the significant outcomes for each method. The outcomes are labeled with the convention \textit{assessment}-\textit{PC number}. The discrete networks used by the competitor methods were formed with the Destriex atlas.  Our method outperforms all other methods for 12 out of the 15 outcomes. In several cases, the improvement is dramatic, e.g. Anger and Hostility-2, Emotion Recognition-4,  Executive Function-2. This suggests potentially large gains in predictive capability when analyzing connectivity data at very high resolutions. Table~\ref{tab:desikan_prediction_results} in the Supplemental Materials gives the corresponding results for the networks formed using the Desikan atlas. Echoing the results of Section~\ref{sssec:hypothesis_testing}, for many cases, we note the predictions using the discrete network embedding techniques are highly sensitive to the choice of atlas.

\begin{table}
\centering
\small
\begin{tabular}{r|rrrrr}
\toprule
 &  \multicolumn{4}{c}{\textbf{SC analysis methods}} \\
 Outcome & CC & TN-PCA & MASE & MRDPG \\
\midrule
Fluid Intelligence-1  &   \textbf{0.1530} (0.0853) &      0.1122 (0.0692) &     0.1321 (0.0765) &     0.1235 (0.0839) \\
Self Regulation-1     &   \textbf{0.2079} (0.0932) &     -0.0460 (0.0902) &     0.1280 (0.0810) &     0.1410 (0.0856) \\
Self Regulation-3     &   0.0329 (0.0838) &      0.0464 (0.1026) &    -0.0117 (0.0811) &     \textbf{0.1289} (0.0966) \\
Sustained Attention-2 &   \textbf{0.1228} (0.0922) &     -0.0412 (0.0844) &    -0.0343 (0.0830) &    -0.0031 (0.0924) \\
Executive Function-1  &   \textbf{0.1085} (0.1033) &      0.1072 (0.0790) &     0.0415  (0.0788) &     0.0881 (0.0753) \\
Executive Function-2  &   \textbf{0.1441} (0.0757) &     -0.0116 (0.0918) &    -0.0631 (0.0859) &     0.0521 (0.1016) \\
Psychiatric-3         &   \textbf{0.1128} (0.0884) &     -0.0470 (0.0797) &    -0.0107 (0.1025) &    -0.0274 (0.0791) \\
Psychiatric-6         &  -0.0376 (0.0872) &      \textbf{0.1277} (0.0862) &     0.1001 (0.0852) &     0.1239 (0.0957) \\
Taste-1               &   \textbf{0.1236} (0.0815) &      0.0164 (0.0873) &     0.0466 (0.0800) &     0.0214 (0.0868) \\
Emotion Recognition-1 &   \textbf{0.1058} (0.0834) &      0.0895 (0.0910) &     0.0896 (0.0802) &     0.0160 (0.0826) \\
Emotion Recognition-2 &   0.0100 (0.0880) &      0.0489 (0.0887) &     \textbf{0.1145} (0.0827) &    -0.0436 (0.0921) \\
Emotion Recognition-4 &   \textbf{0.1591} (0.0873) &     -0.0329 (0.0840) &    -0.0659 (0.0895) &    -0.0349 (0.1017) \\
Anger and Hostility-2 &   \textbf{0.2216} (0.0871) &      0.0011 (0.0957) &    -0.0369 (0.0950) &    -0.0379 (0.0809) \\
Anger and Hostility-3 &   \textbf{0.2190} (0.0898) &     -0.0078 (0.0918) &     0.1850 (0.0904) &     0.0576 (0.0815) \\
BMI and Weight-1      &   \textbf{0.3046} (0.0858) &      0.2365 (0.0899) &     0.0866 (0.0855) &     0.1519 (0.0922) \\
\bottomrule
\end{tabular}
\caption{Trait prediction results for our continuous embeddings, denoted CC, along with TN-PCA, MASE, and MRDPG using the Destriex atlas. The Pearson correlation between the true and predicted outcomes was averaged over the 100 random train-test splits. Standard deviations are shown in parentheses. The best prediction result for each outcome is embolden.}
\label{tab:concon_vs_atlas}
\end{table}

\subsection{Continuous Subnetwork Discovery}\label{ssec:network_discovery}
Finally, we illustrate how to identify connections that are different between groups using our continuous framework.  In order to focus the analysis, we consider the cognitive trait impulsivity, as measured by \textit{delay discounting}. Delay discounting measures the tendency for people to prefer smaller, immediate rewards over larger, but delayed rewards. It is known that steep discounting is associated with a variety of psychiatric conditions, including antisocial personality disorders, drug abuse and pathological gambling \citep{odum2011}. The HCP collects several measures of delay discounting on each participant as a part of a self-regulation/impulsivity assessment. In this study we focus on one of the measures, namely, the subjective value of $\$200$ at 6 months. For this measure, a series of trials are performed in which the subjects are made to choose between two alternatives: $\$200$ in 6 months or a smaller amount today. For each trial, reward amounts are adjusted based on the subject's choices to iteratively determine an indifference amount that identifies the participants subjective value of $\$200$ at 6 months. For more information on how this measurement is collected, we refer the interested reader to \cite{estle2006}.
\par 
From the sample of 437 female HCP subjects, we sub-selected and classified them to have high or low discounting, according to their subjective value of $\$200$ at 6 months. In particular, the subject was classified to the high discounting group if his/her subjective value $\le \$40$, and to the low discounting group if it was  $\ge\$160$. This resulted in a total sample size of 142: 64 in the high discounting group and 78 in the low discounting group. We apply the local inference procedure formulated in Section~\ref{ssec:inference}. The basis functions $\mathcal{V}_{K}$ were estimated from the full set of 437 HCP female subjects, with $K=100$. In order to facilitate the estimation of locally supported basis functions, we use $n_{\alpha_{2}}=50$  which produces $\approx 95\%$ sparse entries in $\boldsymbol{c}_k$'s. 10,000 permutations were used to construct the null distribution for each univariate test and compute the empirical p-values. A Bonferroni-Holm correction was applied to the p-values to ensure FWER$\le 0.10$.   
\par 
The coefficients associated with basis functions $\xi_{33}$ and $\xi_{55}$ were identified to be significantly different between high and low discounting groups. Figure~\ref{fig:subnet_select}a shows the support sets of these selected basis functions (yellow regions) plotted on the cortical surface. Figure~\ref{fig:subnet_select}b  displays the p-values from point-wise two group t-tests on $\boldsymbol{X}\times\boldsymbol{X}$ (left and center) along with the corresponding plot of the observed vs. the expected p-values under $H_0$ (right), for both $(\omega_1,\omega_2)\in\mathcal{C}$ and $(\omega_1,\omega_2)\notin\mathcal{C}$.  The skew of the -log$_{10}$-transformed p-values of the former indicates the presence of sub-regions of $\mathcal{C}$ where the continuous connectivity differs between groups. 
\par 
The support sets show significant coverage of regions and connections in the prefrontal cortex; including in the left and right middle frontal gyrus, and the right frontal pole, orbitofrontal cortex and rostral anterior cingulate cortex. These results are strongly supported by the literature. Generally, areas in the prefrontal cortex are known to be critical for advanced decisions involving reward \citep{rogers1999}. In particular, previous studies have shown delay discounting to be associated with the grey matter volume in the frontal pole, middle frontal gyrus \citep{wang2016_neuro} and the orbitofrontal cortex \citep{owens2017}. fMRI meta-analysis have identified the anterior cingulate cortex to be active during delay discounting tasks \citep{wesley2014}. Additional regions of substantial coverage include the left precentral and postcentral gyrus, along with the right postcentral and supramarginal gyrus. \cite{olson2009} found differences in delay discounting to be associated with mean diffusivity in white matter regions near the supramarginal gyrus, while \cite{wang2016_neuro} found resting state functional connectivity in the precentral and postcentral gyrus to predictive of delay discounting. 

\begin{figure}
    \centering
    %\includegraphics[scale=0.45]{Figures/local_inference_dd_vis.pdf}
    %\caption{A: The support sets (yellow) of the two basis functions found to be significantly associated with connectivity differences in the high vs. low delay discounting groups. B: Point-wise absolute differences in the mean continuous connectivity over the continuous subnetwork cover $\mathcal{C}$.}
    \includegraphics[scale=0.63]{Figures/continuous_delay_discounting_analysis.pdf}
    \caption{(a) The support sets (yellow) of the two basis functions found to be significantly associated with connectivity differences in the high vs. low delay discounting groups. (b) P-values from t-tests at all points $\omega_1,\omega_2\in \boldsymbol{X}\times\boldsymbol{X}$ and associated qq-plot.}
    \label{fig:subnet_select}
\end{figure}


\section{Conclusion and Future Directions}\label{sec:conclusion}
%This work improves the existing structural connectivity analysis framework by replacing the discrete network representation with a continuous one. We define the continuous structural connectivity as a latent random function on the product space of the cortical surface that governs the distribution of tractography streamlines' endpoints. This continuous representation allows us to bypass issues that plague the traditional discrete network based approaches but also poses new challenges for computation and modeling due to the super-high dimensionalities of the data. To facilitate tractable representation and analysis, we formulate a data-adaptive reduced-rank function space that avoids the curse of dimensionality. To construct a set of basis functions that span this space, we derive a penalized optimization problem and propose a novel computationally efficient algorithm for estimation. The proposed method was applied to several critical neuroscience applications, including group difference hypothesis testing and trait prediction. Through comparison with the state-of-the-art atlas-based network analysis methods, we demonstrated the superior performance of the proposed framework in real data analysis of the HCP data.  
This work introduces a novel modeling framework for the analysis of structural connectivity. We define the continuous structural connectivity as a latent random function on the symmetric product space of the cortical surface that governs the distribution of white matter fiber tract endpoints. This continuous representation allows us to bypass issues that plague the traditional discrete network based approaches but also poses new challenges for computation and modeling due to the super-high dimensionalities of the data. To facilitate tractable representation and analysis, we formulate a data-adaptive reduced-rank function space that avoids the curse of dimensionality. To construct a set of basis functions that span this space, we derive a penalized optimization problem and propose a novel computationally efficient algorithm for estimation. The proposed method was applied to several critical neuroscience applications, including hypothesis testing and trait prediction. Through comparison with state-of-the-art atlas-based network analysis methods, we demonstrated the superior performance of the proposed framework in real data analysis of the HCP data. Implementation of our method along with code for processing the SC data has been made publicly available in the github repository \textbf{sbci-brain}: \url{https://github.com/sbci-brain}.
\par 
There are several interesting possible extensions of the proposed framework. First, a principled way of adapting the spherical tessellation, and hence the spline approximation space, to the properties of the distribution of $U$, would likely result in more parsimonious  representation of the data. 
%It can be shown that the optimal tessellation for piecewise linear spline approximation of realizations from a random function is governed by the variance of the Hessian, denoted $\text{Var}\left(\text{Hess}\right)$. In particular, the optimal tessellation elements should have vertices distributed according to a density function proportional to the determinant of $\text{Var}\left(\text{Hess}\right)$ and be equilateral under the Riemannian metric induced by $\text{Var}\left(\text{Hess}\right)$. We notice that this is closely related to the optimal meshing techniques found in the numerical partial differential equations literature, where  meshes are adapted to the properties of certain dynamical systems to produce solvers with greatly reduced approximation error \citep{du2003,du2005,xu2006}. Repurposing these procedures for our case is therefore a direction of interest. 
Second, a unified method that is able to estimate $\mathcal{V}_K$ directly from the streamline endpoints without the need for the intermediate KDE smoothing step is desirable. Third, the registration between the continuous connectivity functions can be improved. Currently, we rely on Freesurfer's registration which only uses structural features on the cortical surface. A future direction is to directly register the continuous connectivity data. Finally, recall that the FWER control for the continuous subnetwork discovery is for the existence of a difference at some $(\omega_1,\omega_2)\in\mathcal{C}$ and thus this procedure is extremely conservative. A more powerful inference procedure is an important direction for future work.
 

\iffalse 

\pagebreak
\begin{center}
\textbf{\LARGE Supplemental Materials}
\end{center}
\setcounter{equation}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{section}{0}
%\setcounter{page}{1}
\makeatletter
\renewcommand{\theequation}{S\arabic{equation}}
\renewcommand{\thefigure}{S\arabic{figure}}
\renewcommand{\thetable}{S\arabic{table}}
\renewcommand{\thesection}{S\arabic{section}}
\renewcommand{\bibnumfmt}[1]{[S#1]}
\renewcommand{\citenumfont}[1]{S#1}

\section{Theory}

\subsection{Functional Greedy Algorithm}\label{ssec:ff_greedy}

\noindent{\textbf{Proof of Proposition~\ref{prop:uap}}
\begin{proof}
Let $\Gamma := \{\gamma_j: j=1,2,...\}$ be a complete orthogonal basis system for $L^2(\Omega)$. For instance, $\Gamma$ may be constructed using the spherical wavelet basis functions defined in \cite{lessig2008}, which form a complete orthogonal basis for $L^2(\mathbb{S}^2)$, and then trivially be extended to a basis for $L^2(\Omega)$ using the technique discussed previously. Then by definition, for $u \in \mathcal{H}\subset L^2(\Omega\times\Omega)$, we have that $u(\omega_1, \omega_2) = \sum_{j=1}^\infty\sum_{l=1}^\infty a_{jl}\gamma_{j}(\omega_1)\gamma_{l}(\omega_2)$, where $a_{jl} = a_{lj}$, due to symmetry. Denote the infinite symmetric matrix 
$$
A = \begin{bmatrix} a_{11} & a_{12} & a_{13} & \cdots \\
a_{21} & a_{22} &  a_{23} & \cdots\\
a_{31} & a_{32} &  a_{33} & \cdots\\
\vdots & \vdots &  \vdots & \vdots\\
\end{bmatrix}.
$$
Since $u \in L^2(\Omega\times\Omega)$, it follows that $\sum_{j=1}^\infty\sum_{l=1}^\infty a_{jl}^2 < \infty$ and therefore $A$ is a Hilbert–Schmidt operator on the space $l^2(\mathbb{N})$ and thus is compact. Then by the spectral theorem, there exists real eigenvalues $\{\lambda_k\}_{k=1}^\infty$ and orthogonal eigenvectors $\{e_k\}_{k=1}^\infty$ such that 
$$
A = \sum_{k=1}^\infty \lambda_ke_k\otimes e_k,
$$
\citep{Hsing2015TheoreticalFO}. Let $\xi_k = \sum_{j=1}^\infty e_{kj}\gamma_j(\omega)$, it follows that both 
$$
\begin{aligned}
    u(\omega_1, \omega_2) &= \sum_{j=1}^\infty\sum_{l=1}^\infty a_{jl}\gamma_{j}(\omega_1)\gamma_{l}(\omega_2) \\
    &= \sum_{j=1}^\infty\sum_{l=1}^\infty\sum_{k=1}^\infty \lambda_ke_{kj} e_{kl}\gamma_{j}(\omega_1)\gamma_{l}(\omega_2) \\ 
    &= \sum_{k=1}^\infty\lambda_k\left(\sum_{j=1}^\infty e_{kj}\gamma_{j}(\omega_1)\right)\left(\sum_{l=l}^\infty e_{kl}\gamma_{l}(\omega_1)\right) \\ 
    &= \sum_{k=1}^\infty \lambda_k \xi_k(\omega_1)\xi_k(\omega_2)
\end{aligned}
$$
and 
$$
\begin{aligned}
\langle\xi_k,\xi_m\rangle_{L^{2}} &= \int_{\Omega}\left(\sum_{j=1}^\infty e_{kj}\gamma_{j}(\omega)\right)\left(\sum_{l=l}^\infty e_{jl}\gamma_{l}(\omega)\right)d\omega \\
&= \sum_{j=1}^\infty\sum_{l=l}^\infty e_{kj}e_{jl}\int_{\Omega}\gamma_{j}(\omega)\gamma_{l}(\omega)d\omega \\
&= \sum_{j=1}^\infty e_{kj}e_{mj} = \delta_{km},
\end{aligned}
$$
completing the proof. 
\end{proof}
\noindent{We provide a result on the convergence rate of the fully functional greedy algorithm that will be useful in proving Theorem~\ref{thrm:sample_convergence_rate}.}
\begin{lemma}\label{lem:population_convergence_rate}
Under Assumption~\ref{assm:smoothness_class}, we have the following expected approximation error rate resulting from the greedy algorithm defined in equation~\eqref{eqn:greedy_algorithm}
$$
\mathbb{E}\left[\left\|R_{k}\right\|_{L^{2}}^2\right] \le  \frac{B^2}{k+1} 
$$
\end{lemma}
\begin{proof}
Notice that we can write
\begin{equation}\label{eqn:reccurence}
\begin{aligned}
    \left\|R_{k}\right\|_{L^{2}}^2 &= \left\| U^c - P_{k}(U^c)\right\|_{L^{2}}^2 \\
    &= \left\| U^c - P_{k-1}(U^c) - \langle U^c - P_{k-1}(U^c), \xi_k\cdot\xi_k\rangle \xi_k\cdot\xi_k\right\|_{L^{2}}^2  \\
    &= \left\| U^c - P_{k-1}(U^c)\right\|_{L^{2}}^2 - |\left\langle U^c - P_{k-1}(U^c), \xi_k\cdot\xi_k\right\rangle_{L^{2}}|^2 \\
    & \equiv \left\| R_{k-1}\right\|_{L^{2}}^2 - |\left\langle R_{k-1}, \xi_k\cdot\xi_k\right\rangle_{L^{2}}|^2 
\end{aligned}
\end{equation}
Furthermore,  
\begin{equation}\label{eqn:bound_prev_reccurence}
\begin{aligned}
    \left\| R_{k-1}\right\|_{L^{2}}^2 &=  \left\langle R_{k-1}, R_{k-1}\right\rangle_{L^{2}} \\ 
    &= \left\langle R_{k-1}, U^{c}\right\rangle_{L^{2}} \\
    &= \left\langle R_{k-1}, \sum_{j \in I} S_{\xi_{j}}\xi_{j}\cdot\xi_{j}\right\rangle_{L^{2}} \\
    &= \sum_{j \in I}S_{\xi_{j}}\left\langle R_{k-1},  \xi_{j}\cdot\xi_{j}\right\rangle_{L^{2}}\\ 
    &\le \sum_{j \in I}|S_{\xi_{j}}||\left\langle R_{k-1},  \xi_{j}\cdot\xi_{j}\right\rangle_{L^{2}}|\\
    &\le \sum_{j \in I}|S_{\xi_{j}}|\sup_{\xi\in\mathcal{V}}|\left\langle R_{k-1},  \xi\cdot\xi\right\rangle_{L^{2}}|
\end{aligned}
\end{equation}
Now, taking the expected value of \eqref{eqn:bound_prev_reccurence} and using Cauchy-Schwarz, we have that 
$$
\begin{aligned}
     \mathbb{E}\left[\sum_{j \in I}|S_{\xi_{j}}|\sup_{\xi\in\mathcal{V}}|\left\langle R_{k-1},  \xi\cdot\xi\right\rangle_{L^{2}}|\right] \le  \mathbb{E}\left[\left(\sum_{j \in I}|S_{\xi_{j}}|\right)^2\right]^{1/2}\mathbb{E}\left[\sup_{\xi\in\mathcal{V}}|\left\langle R_{k-1},  \xi\cdot\xi\right\rangle_{L^{2}}|^2\right]^{1/2} \\ 
\end{aligned}
$$
which gives the bound 
$$
 \mathbb{E}\left[ \left\| R_{k-1}\right\|_{L^{2}}^2\right]^2 \le \mathbb{E}\left[\left(\sum_{j \in I}|S_{\xi_{j}}|\right)^2\right]\mathbb{E}\left[\sup_{\xi\in\mathcal{V}}|\left\langle R_{k-1},  \xi\cdot\xi\right\rangle_{L^{2}}|^2\right].
$$
By the definition of our greedy selection algorithm, we have that
$$
\mathbb{E}\left[\sup_{\xi\in\mathcal{V}}|\left\langle R_{k-1},  \xi\cdot\xi\right\rangle_{L^{2}}|^2\right] = \mathbb{E}\left[|\left\langle R_{k-1},  \xi_k\cdot\xi_k\right\rangle_{L^{2}}|^2\right].
$$
Taking the expectation of \eqref{eqn:reccurence} and plugging in our results, we have that 
$$
\begin{aligned}
\mathbb{E}\left[\left\|R_{k}\right\|_{L^{2}}^2\right] &=  \mathbb{E}\left[\left\| R_{k-1}\right\|_{L^{2}}^2\right] - \mathbb{E}\left[|\left\langle R_{k-1}, \xi_k\cdot\xi_k\right\rangle_{L^{2}}|^2\right] \\
&\le \mathbb{E}\left[\left\| R_{k-1}\right\|_{L^{2}}^2\right]\left(1 - \frac{\mathbb{E}\left[\left\| R_{k-1}\right\|_{L^{2}}^2\right]}{\mathbb{E}\left[\left(\sum_{j \in I}|S_{\xi_{j}}|\right)^2\right]}\right) \\
& \le \mathbb{E}\left[\left\| R_{k-1}\right\|_{L^{2}}^2\right]\left(1 - \frac{\mathbb{E}\left[\left\| R_{k-1}\right\|_{L^{2}}^2\right]}{B^2}\right),
\end{aligned}
$$
where the final inequality comes from the fact that, under Assumption~\ref{assm:smoothness_class},
$$
\mathbb{E}\left[\left(\sum_{j \in I}|S_{\xi_{j}}|\right)^2\right] = \mathbb{E}\left[\left\|U\right\|_{L_{1,B}}^2 \right] \le B^2
$$
Furthermore, we have that 
$$
\begin{aligned}
    \mathbb{E}\left[\left\|R_{0}\right\|_{L^{2}}^2\right] &= \sum_{k=1}^\infty\mathbb{E}\left[Z_k^2\right] = \mathbb{E}\left[\sum_{j\in I}|S_{\xi_{j}}||S_{\xi_{j}}|\right] \\
    &\le \mathbb{E}\left[\left(\sum_{j\in I}|S_{\xi_{j}}|\right)\left(\sum_{k\in I}|S_{\xi_{k}}|\right)\right] \\
    &= \mathbb{E}\left[\left\|U\right\|_{L_{1,B}}^2 \right] \le B^2
\end{aligned}
$$
Hence the sequence $\{\mathbb{E}\left[\left\|R_{k}\right\|_{L^{2}}^2\right]\}_{k}$ is decreasing.
\par 
For clarity, denote $r_k := \mathbb{E}\left[\left\|R_{k}\right\|_{L^{2}}^2\right]$. Assume that $r_{k-1}\le \frac{B^2}{k}$ for any $k$. Then if $r_{k-1} \le \frac{B^2}{k+1}$, clearly $r_{k} \le \frac{B^2}{k+1}$ since it is a decreasing sequence. If $r_{k-1} \ge \frac{B^2}{k+1}$, then 
$r_k \le \frac{B^2}{k}\left(1 - B^{-2}\frac{B^2}{k+1}\right)= \frac{B^2}{k+1}$. Hence, by induction we have established that 
$$
\mathbb{E}\left[\left\|R_{k}\right\|_{L^{2}}^2\right] \le \frac{B^2}{k+1}.
$$
\end{proof}
\noindent{\textbf{Proof of Theorem~\ref{thrm:sample_convergence_rate}}}
\begin{proof} 
For clarity, denote $S_{i,\xi_{j}} = \langle U^{c}_i, \xi_j\cdot\xi_j\rangle_{L^{2}}$. Using the same logic as \eqref{eqn:reccurence} and \eqref{eqn:bound_prev_reccurence} we have that 
$$
\left\|R_{k,i}\right\|_{L^{2}}^2 = \left\|R_{k-1,i}\right\|_{L^{2}}^2 -  |\left\langle R_{k-1,i}, \xi_k\cdot\xi_k\right\rangle_{L^{2}}|^2 
$$
and 
$$
\left\|R_{k-1,i}\right\|_{L^{2}}^2 \le \sum_{j \in I}|S_{i,\xi_{j}}|\sup_{\xi\in\mathcal{V}}|\left\langle R_{k-1,i},  \xi\cdot\xi\right\rangle_{L^{2}}|.
$$
Furthermore, applying Cauchy-Schwarz to the empirical inner product, we have that 
$$
\begin{aligned}
N^{-1}\sum_{i=1}^N\sum_{j \in I}|S_{i,\xi_{j}}|\sup_{\xi\in\mathcal{V}}|\left\langle R_{k-1,i},  \xi\cdot\xi\right\rangle_{L^{2}}| &\le \left(N^{-1}\sum_{i=1}^N\left(\sum_{j \in I}|S_{i,\xi_{j}}|\right)^2\right)^{1/2}\times \\
&\left(N^{-1}\sum_{i=1}^N\sup_{\xi\in\mathcal{V}}|\left\langle R_{k-1,i},  \xi\cdot\xi\right\rangle_{L^{2}}|^2\right)^{1/2}.
\end{aligned}
$$
Combining these results, we obtain the relation 
\begin{equation}\label{eqn:empirical_recurrence}
    R^{(N)}_k \le R^{(N)}_{k-1}\left(1 - \frac{R^{(N)}_{k-1}}{U^{(N)}_{L_{1}}}\right).
\end{equation}
where
$$
    R^{(N)}_k := N^{-1}\sum_{i=1}^N\left\|R_{k,i}\right\|_{L^{2}}^2 \text{ and } U^{(N)}_{L_{1}} := N^{-1}\sum_{i=1}^N\left\|U_i\right\|_{L_{1,B}}^2
$$
for clarity. 
\par 
By Hoeffding's Inequality, for any $t>0$ we have that 
$$
\mathbb{P}\left(|N^{-1}\sum_{i=1}^N\left\|U_i\right\|_{L_{1,B}}^2 - \mathbb{E}\left[\left\|U\right\|_{L_{1,B}}^2\right]| \ge t\right)\le 2\text{exp}(-\frac{2Nt^2}{B^4}). 
$$
So with probability at least  $1 - 2\text{exp}(-\frac{2Nt^2}{B^4})$, we have 
$$
\begin{aligned}
N^{-1}\sum_{i=1}^N\left\|U_i\right\|_{L_{1,B}}^2 &= |N^{-1}\sum_{i=1}^N\left\|U_i\right\|_{L_{1,B}}^2 - \mathbb{E}\left[\left\|U\right\|_{L_{1,B}}^2\right] + \mathbb{E}\left[\left\|U\right\|_{L_{1,B}}^2\right]| \\ 
&\le |N^{-1}\sum_{i=1}^N\left\|U_i\right\|_{L_{1,B}}^2 - \mathbb{E}\left[\left\|U\right\|_{L_{1,B}}^2\right]| + \mathbb{E}\left[\left\|U\right\|_{L_{1,B}}^2\right] \\
&\le t + B^2.
\end{aligned}
$$
and 
\begin{equation}\label{eqn:empirical_recurrence_prop_bound}
    R^{(N)}_k \le R^{(N)}_{k-1} \left(1 - \frac{R^{(N)}_{k-1}}{t + B^2}\right).
\end{equation}
Finally we note that, with probability 1, $R^{(N)}_k\le B^2 + t$. The final result can be obtained by applying the same recursion argument as in the proof to Lemma~\ref{lem:population_convergence_rate}.
\end{proof}

\section{Marginal Basis System}\label{sec:marg_splines}

\subsection{Spherical Splines}
Define a spherical triangle $T$ with vertices $\boldsymbol{v}_1, \boldsymbol{v}_2, \boldsymbol{v}_3$, as the set of points in $\mathbb{S}^2$ that are bounded by the great circle arcs connecting $(\boldsymbol{v}_{i}, \boldsymbol{v}_{i+1})$, $i=1,2,3$ and $\boldsymbol{v}_4\equiv \boldsymbol{v}_1$. A collection of spherical triangles $\mathcal{T} = \{T_j\}_{j=1}^J$ is a spherical triangulation of $\mathbb{S}^2$, provided that the intersection between any two elements in $\mathcal{T}$ is empty, a common vertex or a common edge and $\mathbb{S}^2 = \bigcup_{T_j\in\mathcal{T}} T_j$. The \textit{spherical Delaunay triangulation} is the unique triangulation over a set of points $\{\boldsymbol{v}_m\}_{m=1}^M$ such that the minimum angle in the triangulation is as large as possible.
\par 
For each spherical triangle $T_j$, we can define a local coordinate system called the \textit{spherical barycentric coordinates}, defined for $\boldsymbol{v}\in T_i$ to be the nonnegative real numbers satisfying 
$$
    \boldsymbol{v} = b_1(\boldsymbol{v})\boldsymbol{v}_1 + b_2(\boldsymbol{v})\boldsymbol{v}_3 + b_3(\boldsymbol{v})\boldsymbol{v}_3.
$$
We can define the linear spherical Bernstein basis on $T_j$ as the span of the three nodal basis functions $\mathcal{B} := \text{span}\left(\{b_1(\boldsymbol{v}), b_2(\boldsymbol{v}), b_3(\boldsymbol{v})\}\right)$. That is, for any $s(\boldsymbol{v}) \in \mathcal{B}$, there exists coefficients $c_1,c_2,c_3$ such that $s(\boldsymbol{v}) = \sum_{j=1}^3c_jb_j(\boldsymbol{v})$.
The local basis functions defined for each spherical triangle can be ``glued together'' to form a piecewise continuous linear spline space over $\mathbb{S}^2$. Following \cite{lai2007}, we define 
$$
    \mathcal{S}_1^0(\mathcal{T}) = \{s\in C^0(\mathbb{S}^2):s|_{T_{j}}\in \mathcal{B},\quad\text{for}\quad j=1,...,J\}.
$$
An explicit basis for $ \mathcal{S}_1^0(\mathcal{T})$ can be constructed as follows: for each vertices $\boldsymbol{v}_m$ in tessellation $\mathcal{T}$, let $\phi_j\in\mathcal{S}_1^0(\mathcal{T})$ such that
$$
    \phi_j(\boldsymbol{v}_m) = \begin{cases}
      1 & \text{ if } j=m\\
      0 & \text{ otherwise}
    \end{cases}.
$$
It can be shown that $\phi_j$ is unique and that $\{\phi_j\}_{j=1}^M$ forms a basis for $\mathcal{S}_1^0(\mathcal{T})$ \citep{lai2007}.
\par 
The $\phi_j$ have several attractive properties. Efficient algorithms exist for evaluating and computing their directional derivative using the local basis functions \citep{schumaker2015}. For scattered data approximation, the $L^2$ rate of convergence of the least squares minimizer in $\mathcal{S}_d^0(\mathcal{T})$ for $g$ with $\beta+1$ continuous derivatives is $\mathcal{O}(|\mathcal{T}|^{\beta})$, where $|\mathcal{T}| = \max_{T\in\mathcal{T}}|T|$ with $|T|$ being the length of the longest arc in $T$ and any degree $d$. Although the rate depends on the smoothness of the unknown function, it is independent of the degree $d$ and hence in the ``fine grid'' regime, we do not gain approximation power by considering any spline basis of order larger than 1. 

\subsection{Penalty Matrix Computation}

Define  $\gamma:\Theta\subset\mathbb{R}^2\rightarrow\mathbb{R}^3$ to be a local parameterization around $\boldsymbol{x}\in\mathbb{S}^2$ that is smooth and bijective. The following choice of local parameterization 
$$
    \gamma(\theta_1, \theta_2) = (\text{sin}(\theta_1)\text{cos}(\theta_2), \text{sin}(\theta_1)\text{sin}(\theta_2), \text{cos}(\theta_1))^\intercal := \boldsymbol{x}^\intercal
$$
is valid (invertible) for all points on $\mathbb{S}^2$ except $(0,0,\pm 1)$, i.e. outside of the poles. By definition, the vectors 
$$
    \{\frac{\partial \gamma}{\partial\theta_1}(\theta_1,\theta_2), \frac{\partial \gamma}{\partial\theta_2}(\theta_1,\theta_2)\}
$$
form a basis for the tangent space $T_{\boldsymbol{x}}(\mathbb{S}^2)$. We may equip $T_{\boldsymbol{x}}(\mathbb{S}^2)$ with an inner product defined by matrix $\boldsymbol{\Gamma}\in\mathbb{R}^{2\times 2}$
where 
$$
\langle \boldsymbol{u}, \boldsymbol{v} \rangle_{T_{\omega}(\mathbb{S}^2)} = \boldsymbol{u}^\intercal\boldsymbol{\Gamma}\boldsymbol{v}
$$
where $\boldsymbol{u},\boldsymbol{v}\in\mathbb{R}^2$ are coordinates w.r.t. to basis vectors of $T_{\omega}(\mathbb{S}^2)$. We let $\boldsymbol{\Gamma}$ be the first fundamental form, i.e. the inner product induced by the Euclidean embedding space $\mathbb{R}^3$, that is for $\theta = \gamma^{-1}(\omega)$, we have the element-wise definition 
$$
    \boldsymbol{\Gamma}_{ij}(\theta) = \langle\frac{\partial \gamma}{\partial\theta_i}(\theta_1,\theta_2), \frac{\partial \gamma}{\partial\theta_j}(\theta_1,\theta_2)\rangle_{\mathbb{R}^3}.
$$
We can now define the gradient for $\phi_k:\mathbb{S}^2\rightarrow\mathbb{R}$ 
$$
    \nabla_{\mathbb{S}^2}\phi_k(\boldsymbol{x}) = \sum_{i,j}^2 [\boldsymbol{\Gamma}(\boldsymbol{\theta})]^{-1}_{ij}\frac{\partial (\phi_k\circ\gamma)}{\partial \theta_j}(\boldsymbol{\theta})\frac{\partial \gamma}{\partial \theta_j}(\boldsymbol{\theta}).   
$$
Using basic trigonometric identities it easy to show
$$
\boldsymbol{\Gamma}^{-1}(\boldsymbol{\theta}) = \begin{pmatrix}  
            1 & 0 \\
            0 & 1/\text{sin}^2(\theta_1)  
\end{pmatrix}.
$$
The basis vectors are 
$$
   \frac{\partial \gamma}{\partial\theta_1}(\theta_1,\theta_2) = (\text{cos}(\theta_1)\text{cos}(\theta_2), \text{cos}(\theta_1)\text{sin}(\theta_2), -\text{sin}(\theta_1))^\intercal
$$
and 
$$
    \frac{\partial \gamma}{\partial\theta_2}(\theta_1,\theta_2) = (-\text{sin}(\theta_1)\text{sin}(\theta_2), \text{sin}(\theta_1)\text{cos}(\theta_2), 0)^\intercal
$$
Finally, we must compute the partial derivative of the basis $\phi_k$ with respect to the local coordinates. We have 
$$
\begin{aligned}
    \frac{\partial \phi_k \circ \psi}{\partial \theta_j}(\theta) &= \sum_{l=1}^3 \frac{\partial\phi_k}{\partial x_l}\frac{\partial x_l}{\partial\theta_j} \\
\end{aligned}
$$
Now, we have already computed $\frac{\partial x_l}{\partial\theta_j}$ and thus we must find  $\frac{\partial\phi_k}{\partial x_l}$ to complete the computation, for which fast algorithms exists \citep{lai2007}. The final form of the penalty matrix is given in the following proposition. 
\begin{proposition}\label{prop:penalty_formulation}
Under the basis expansion in Equation~\eqref{eqn:basis_expansion}, the quadratic variation penalty has the representation 
$$
\begin{pmatrix} \boldsymbol{c}_{1} \\ \boldsymbol{c}_{2}  \end{pmatrix}^\intercal \begin{bmatrix} \int_{\mathbb{S}^2}\boldsymbol{F}_{1}\boldsymbol{F}^\intercal_{1} & \boldsymbol{0} \\ \boldsymbol{0} & \int_{\mathbb{S}^2}\boldsymbol{F}_{2}\boldsymbol{F}^\intercal_{2} \end{bmatrix} \begin{pmatrix} \boldsymbol{c}_{1} \\ \boldsymbol{c}_{2}  \end{pmatrix},
$$
where $\boldsymbol{F}_d(\boldsymbol{x})\in\mathbb{R}^{M_{d}\times 3}$ is the Jacobian of $\boldsymbol{\phi}_{M_{d}}$.
\end{proposition}
\begin{proof}
Since $\Omega = \mathbb{S}_1^2 \cup \mathbb{S}_2^2$, the gradient separates as 
$$
    \nabla_{\Omega}(\xi_k(\boldsymbol{x})) = \nabla_{\mathbb{S}^2}(\boldsymbol{c}^\intercal_{1,k}\boldsymbol{\phi}_{M_{1}}(\boldsymbol{x}))\mathbb{I}\{\boldsymbol{x}\in\mathbb{S}_1^2\} + \nabla_{\mathbb{S}^2}(\boldsymbol{c}^\intercal_{2,k}\boldsymbol{\phi}_{M_{2}}(\boldsymbol{x}))\mathbb{I}\{\boldsymbol{x}\in\mathbb{S}_2^2\}.
$$
We have 
$$
\begin{aligned}
    \text{Pen}(\xi_k) &=  \int_{\Omega}\left[ \boldsymbol{c}^\intercal_{1,k}\boldsymbol{F}_{1}(\boldsymbol{x})\boldsymbol{F}^\intercal_{1}(\boldsymbol{x})\boldsymbol{c}_{1,k}1\{\boldsymbol{x}\in\mathbb{S}_1^2\} + \boldsymbol{c}^\intercal_{2,k}\boldsymbol{F}_{2}(\boldsymbol{x})\boldsymbol{F}^\intercal_{2}(\boldsymbol{x})\boldsymbol{c}_{2,k}1\{\boldsymbol{x}\in\mathbb{S}_2^2\}\right] d\boldsymbol{x} \\
    &=  \begin{pmatrix} \boldsymbol{c}_{1,k} \\ \boldsymbol{c}_{2,k} \end{pmatrix}^\intercal \begin{bmatrix} \int_{\mathbb{S}^2}\boldsymbol{F}_{1}\boldsymbol{F}^\intercal_{1} & \boldsymbol{0} \\ \boldsymbol{0} & \int_{\mathbb{S}^2}\boldsymbol{F}_{2}\boldsymbol{F}^\intercal_{2} \end{bmatrix} \begin{pmatrix} \boldsymbol{c}_{1,k} \\ \boldsymbol{c}_{2,k} \end{pmatrix} \\ 
\end{aligned}
$$
\end{proof}
The required integrals can be computed using Lebedev quadrature rules or using exact rules for the local planar triangle approximation to the spherical triangle. The latter of these is of course faster and preferable when the spherical triangles are small enough.

\section{Algorithm}\label{ssec:algoImp}

\subsection{Derivation of Block Update}
We first state and prove two results that will be useful for our derivation.
\begin{proposition}\label{prop:isometric_mapping}
Define the reparameterization $\tilde{\boldsymbol{c}} = \boldsymbol{D}\boldsymbol{V}^\intercal\boldsymbol{c}$. Then 
\begin{equation}
\sum_{i=1}^N\left\langle \boldsymbol{R}_{k-1,i}, \boldsymbol{\Phi}\boldsymbol{c}\otimes\boldsymbol{\Phi}\boldsymbol{c}\right\rangle_{F}^2 \propto \sum_{i=1}^N\left(\tilde{\boldsymbol{c}}^\intercal s_{i}(\tilde{\boldsymbol{c}})\boldsymbol{G}_{k-1,i}\tilde{\boldsymbol{c}}\right)
\end{equation}
where $\boldsymbol{G}_{k-1,i} = \boldsymbol{U}^\intercal\boldsymbol{R}_{k-1,i}\boldsymbol{U}$ and $s_i(\tilde{\boldsymbol{c}}) = \tilde{\boldsymbol{c}}^\intercal\boldsymbol{G}_{k-1,i}\tilde{\boldsymbol{c}}$. 
\end{proposition}
\begin{proof}
Notice that
$$
\begin{aligned}
\left\langle \boldsymbol{R}_{k-1,i}, \boldsymbol{\Phi}\boldsymbol{c}\otimes\boldsymbol{\Phi}\boldsymbol{c}\right\rangle_{F} &= \text{trace}\left( \boldsymbol{R}_{k-1,i}^\intercal, \right[\boldsymbol{\Phi}\boldsymbol{c}\left]\right[\boldsymbol{\Phi}\boldsymbol{c}\left]^\intercal\right)\\ 
&= \text{trace}\left( \boldsymbol{R}_{k-1,i}^\intercal, \boldsymbol{U}\boldsymbol{D}\boldsymbol{V}^\intercal\boldsymbol{c}\boldsymbol{c}^\intercal\boldsymbol{V}\boldsymbol{D}\boldsymbol{U}^\intercal\right) \\
&= \tilde{\boldsymbol{c}}^\intercal\boldsymbol{G}_{k-1,i}\tilde{\boldsymbol{c}}.
\end{aligned}
$$
Coupled with Equation~\eqref{eqn:coef_rewrite}, the result follows directly. 
\end{proof}
For clarity, in the following derivation we work mainly in the transformed parameter $\boldsymbol{\tilde{c}}$. For notational convenience, we define the quantities 
 $$
 \boldsymbol{\tilde{J}}_{\boldsymbol{\phi}} = \boldsymbol{D}^{-1}\boldsymbol{V}^\intercal\boldsymbol{J}_{\boldsymbol{\phi}}\boldsymbol{V}\boldsymbol{D}^{-1}, \qquad \boldsymbol{\tilde{R}}_{\boldsymbol{\phi}} = \boldsymbol{D}^{-1}\boldsymbol{V}^\intercal\boldsymbol{Q}_{\boldsymbol{\phi}}\boldsymbol{V}\boldsymbol{D}^{-1},
$$ 
so
$$
    \boldsymbol{c}^\intercal\boldsymbol{J}_{\boldsymbol{\phi}}\boldsymbol{c} = \boldsymbol{\tilde{c}}^\intercal\boldsymbol{\tilde{J}}_{\boldsymbol{\phi}}\boldsymbol{\tilde{c}}, \qquad
    \boldsymbol{c}^\intercal\boldsymbol{Q}_{\boldsymbol{\phi}}\boldsymbol{c} = \boldsymbol{\tilde{c}}^\intercal\boldsymbol{\tilde{R}}_{\boldsymbol{\phi}}\boldsymbol{\tilde{c}}.
$$

\begin{proposition}\label{prop:orthogonal_constraint}
Let $\boldsymbol{\tilde{C}}_{k-1} = [\boldsymbol{\tilde{c}}_1, ..., \boldsymbol{\tilde{c}}_{k-1}]$. Then the orthogonality constraint $\boldsymbol{c}^\intercal\boldsymbol{J}_{\boldsymbol{\phi}}\boldsymbol{c}_j = \boldsymbol{\tilde{c}}^\intercal\boldsymbol{\tilde{J}}_{\boldsymbol{\phi}}\boldsymbol{\tilde{c}_j} = 0\text{ for }j=1,...,k-1$ is equivalent the condition that 
$$
    (\boldsymbol{I} - \boldsymbol{\tilde{P}}_{k-1})\boldsymbol{\tilde{c}} = \boldsymbol{\tilde{c}}
$$
where 
$$
\begin{aligned}
    \boldsymbol{\tilde{P}}_{k-1} &= \boldsymbol{\tilde{C}}_{k-1}[\boldsymbol{\tilde{C}}_{k-1}^\intercal\boldsymbol{\tilde{J}}_{\boldsymbol{\phi}}\boldsymbol{\tilde{C}}_{k-1}]^{-1}\boldsymbol{\tilde{C}}_{k-1}^\intercal\boldsymbol{\tilde{J}}_{\boldsymbol{\phi}} \\
    &= \boldsymbol{D}\boldsymbol{V}^\intercal\boldsymbol{C}_{k-1}\left[\boldsymbol{C}_{k-1}^{\intercal}\boldsymbol{J}_{\boldsymbol{\phi}}\boldsymbol{C}_{k-1}\right]^{-1}\boldsymbol{C}_{k-1}^{\intercal}\boldsymbol{J}_{\boldsymbol{\phi}}\boldsymbol{V}\boldsymbol{D}^{-1} \\
    &= \boldsymbol{P}_{k-1} 
\end{aligned}
$$
\end{proposition}
\begin{proof}
Note that the matrix $\boldsymbol{\tilde{J}}$ is symmetric and positive definite and therefore defines an inner product on $\mathbb{R}^{M_{1}+M_{2}}$. The result then follows trivially from standard results in linear algebra. 
\end{proof}

Using Proposition~\ref{prop:isometric_mapping}, we can reparamterized problem \eqref{eqn:empirical_optm_reformulated_discretized_AO} as 
\begin{equation}\label{eqn:empirical_optm_reformulated_discretized_reparam} 
\begin{aligned}
    \hat{\tilde{\boldsymbol{c}}}_k = &\underset{\tilde{\boldsymbol{c}} \in \mathbb{R}^{M}}{\text{ argmax }} \sum_{i=1}^N\left(\tilde{\boldsymbol{c}}^\intercal \boldsymbol{s}_{i}\boldsymbol{G}_{k-1,i}\tilde{\boldsymbol{c}}\right) - \alpha_1\boldsymbol{\tilde{c}}^\intercal\boldsymbol{\tilde{R}}_{\boldsymbol{\phi}}\boldsymbol{\tilde{c}}\\
    \textrm{s.t.} \quad & \boldsymbol{\tilde{c}}^\intercal\boldsymbol{\tilde{J}}_{\boldsymbol{\phi}}\boldsymbol{\tilde{c}} = 1,  \quad \boldsymbol{\tilde{c}}^\intercal\boldsymbol{\tilde{J}}_{\boldsymbol{\phi}}\boldsymbol{\tilde{c}}_j  = 0 \text{ for }j=1,2,...,k-1\\
    \quad & \left\|\boldsymbol{V}\boldsymbol{D}^{-1}\tilde{\boldsymbol{c}}\right\|_{0} \le \alpha_{2} \\
    \quad & \boldsymbol{s} = \mathcal{G}_{k-1}\times_1 \boldsymbol{\tilde{c}} \times_2 \boldsymbol{\tilde{c}},
\end{aligned}
\end{equation}
where the rewritten constraint $\boldsymbol{s} = \mathcal{G}_{k-1}\times_1 \boldsymbol{\tilde{c}} \times_2 \boldsymbol{\tilde{c}}$ follows from the element-wise definition of $\boldsymbol{s}_i(\boldsymbol{\tilde{c}})$ in Proposition~\ref{prop:isometric_mapping} coupled with the definition of $d$-mode multiplication. Noting that we have $\mathcal{G}_{k-1}\times_3\boldsymbol{s} = \sum_{i=1}^N\boldsymbol{s}_{i}\boldsymbol{G}_{k-1,i}$, \eqref{eqn:empirical_optm_reformulated_discretized_reparam} becomes 
$$
\begin{aligned}
    \hat{\tilde{\boldsymbol{c}}}_k = &\underset{\tilde{\boldsymbol{c}} \in \mathbb{R}^{M}}{\text{ argmax }} \tilde{\boldsymbol{c}}^\intercal\left[\mathcal{G}_{k-1}\times_3\boldsymbol{s} - \alpha_1{\boldsymbol{\tilde{R}}}_{\boldsymbol{\phi}}\right]\boldsymbol{\tilde{c}}\\
    \textrm{s.t.} \quad & \boldsymbol{\tilde{c}}^\intercal\boldsymbol{\tilde{J}}_{\boldsymbol{\phi}}\boldsymbol{\tilde{c}} = 1,  \quad \boldsymbol{\tilde{c}}^\intercal\boldsymbol{\tilde{J}}_{\boldsymbol{\phi}}\boldsymbol{\tilde{c}}_j  = 0 \text{ for }j=1,2,...,k-1\\
    \quad & \left\|\boldsymbol{V}\boldsymbol{D}^{-1}\tilde{\boldsymbol{c}}\right\|_{0} \le \alpha_{2} \\
    \quad & \boldsymbol{s} = \mathcal{G}_{k-1}\times_1 \boldsymbol{\tilde{c}} \times_2 \boldsymbol{\tilde{c}} 
\end{aligned}
$$
Apply Proposition~\ref{prop:orthogonal_constraint}, the orthogonality constraint can be absorbed into the objective function, resulting in 
$$
\begin{aligned}
    \hat{\tilde{\boldsymbol{c}}}_k = &\underset{\tilde{\boldsymbol{c}} \in \mathbb{R}^{M}}{\text{ argmax }} \tilde{\boldsymbol{c}}^\intercal\left(\boldsymbol{I} - \boldsymbol{\tilde{P}}_{k-1}\right)\left[\mathcal{G}_{k-1}\times_3\boldsymbol{s} - \alpha_1{\boldsymbol{\tilde{R}}}_{\boldsymbol{\phi}}\right]\left(\boldsymbol{I} - \boldsymbol{\tilde{P}}_{k-1}\right)\boldsymbol{\tilde{c}}\\
    \textrm{s.t.} \quad & \boldsymbol{\tilde{c}}^\intercal\boldsymbol{\tilde{J}}_{\boldsymbol{\phi}}\boldsymbol{\tilde{c}} = 1 \\
    \quad & \left\|\boldsymbol{V}\boldsymbol{D}^{-1}\tilde{\boldsymbol{c}}\right\|_{0} \le \alpha_{2} \\
    \quad & \boldsymbol{s} = \mathcal{G}_{k-1}\times_1 \boldsymbol{\tilde{c}} \times_2 \boldsymbol{\tilde{c}}. 
\end{aligned}
$$
Transforming back to the original coordinates using $\boldsymbol{c} = \boldsymbol{V}\boldsymbol{D}^{-1}\tilde{\boldsymbol{c}}$ and invoking the relaxed norm constraint, 
$$
\begin{aligned}
     \hat{\boldsymbol{c}}_k  = \underset{\boldsymbol{c} \in \mathbb{R}^{M}}{\text{ argmax }} &\quad \boldsymbol{c}^\intercal\left[\boldsymbol{V}\boldsymbol{D}\left(\boldsymbol{I} - \boldsymbol{P}_{k-1}\right)\left[\mathcal{G}_{k-1}\times_3\boldsymbol{s} - \alpha_1\boldsymbol{D}^{-1}\boldsymbol{V}^\intercal\boldsymbol{Q}_{\boldsymbol{\phi}}\boldsymbol{V}\boldsymbol{D}^{-1}\right]\left(\boldsymbol{I} - \boldsymbol{P}_{k-1}^{\intercal}\right)\boldsymbol{D}\boldsymbol{V}^\intercal\right]\boldsymbol{c} \\
    & \textrm{s.t.} \quad \boldsymbol{c}^\intercal\boldsymbol{c} = 1, \quad \left\|\boldsymbol{c}\right\|_{0} \le \alpha_{2}, \\
     \quad & \boldsymbol{s} = \mathcal{G}_{k-1}\times_1 \left(\boldsymbol{D}\boldsymbol{V}^\intercal\boldsymbol{c}\right) \times_2 \left(\boldsymbol{D}\boldsymbol{V}^\intercal\boldsymbol{c}\right), 
\end{aligned} 
$$
and the updates \eqref{eqn:ctilde_update} and \eqref{eqn:s_update} follow trivially by applying block coordinate ascent to the above. 

\fi 
